Constraints on the structure of hot exozodiacal dust belts

Recent interferometric surveys of nearby main-sequence stars show a faint but significant near-infrared excess in roughly two dozen systems, i.$\,$e. around $10\,\%$ to $30\,\%$ of stars surveyed. This excess is attributed to dust located in the immediate vicinity of the star, the origin of which is highly debated. We used previously published interferometric observations to constrain the properties and distribution of this hot dust. Considering both scattered radiation and thermal reemission, we modelled the observed excess in nine of these systems. We find that grains have to be sufficiently absorbing to be consistent with the observed excess, while dielectric grains with pure silicate compositions fail to reproduce the observations. The dust should be located within $\sim\,0.01-1\,au$ from the star depending on its luminosity. Furthermore, we find a significant trend for the disc radius to increase with the stellar luminosity. The dust grains are determined to be below $0.2-0.5\,\mu\textrm{m}$, but above $0.02-0.15\,\mu\textrm{m}$ in radius. The dust masses amount to $(0.2-3.5)\times10^{-9}\,M_\oplus$. The near-infrared excess is probably dominated by thermal reemission, though a contribution of scattered light up to $35\,\%$ cannot be completely excluded. The polarisation degree predicted by our models is always below $5\,\%$, and for grains smaller than $\sim0.2\,\mu\textrm{m}$ even below $1\,\%$. We also modelled the observed near-infrared excess of another ten systems with poorer data in the mid-infrared. The basic results for these systems appear qualitatively similar, yet the constraints on the dust location and the grain sizes are weaker.

==> Literature <==
@ARTICLE{Abe2006,
   author = {{Abe}, M. and {Takagi}, Y. and {Kitazato}, K. and {Abe}, S. and 
	{Hiroi}, T. and {Vilas}, F. and {Clark}, B.~E. and {Abell}, P.~A. and 
	{Lederer}, S.~M. and {Jarvis}, K.~S. and {Nimura}, T. and {Ueda}, Y. and 
	{Fujiwara}, A.},
    title = "{Near-Infrared Spectral Results of Asteroid Itokawa from the Hayabusa Spacecraft}",
  journal = {Science},
     year = 2006,
    month = jun,
   volume = 312,
    pages = {1334-1338},
      doi = {10.1126/science.1125718},
   adsurl = {http://adsabs.harvard.edu/abs/2006Sci...312.1334A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 

@BOOK{AbramowitzStegun,
   author = {{Abramowitz}, M. and {Stegun}, I.~A.},
    title = "{Handbook of mathematical functions with formulas, graphs, and mathematical tables}",
booktitle = {Dover Books on Advanced Mathematics, New York: Dover, |c1965, Corrected edition, edited by Abramowitz, Milton; Stegun, Irene A.},
     year = 1965,
   editor = "{Abramowitz, M.~{\&} Stegun, I.~A.}",
}

@ARTICLE{Absil2006,
   author = {{Absil}, O. and {di Folco}, E. and {M{\'e}rand}, A. and {Augereau}, J.-C. and 
	{Coud{\'e} du Foresto}, V. and {Aufdenberg}, J.~P. and {Kervella}, P. and 
	{Ridgway}, S.~T. and {Berger}, D.~H. and {ten Brummelaar}, T.~A. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N.~H. and {McAlister}, H.~A.
	},
    title = "{Circumstellar material in the <ASTROBJ>Vega</ASTROBJ> inner system revealed by CHARA/FLUOR}",
  journal = {\aap},
   eprint = {astro-ph/0604260},
 keywords = {stars: individual: Vega, circumstellar matter, techniques: interferometric},
     year = 2006,
    month = jun,
   volume = 452,
    pages = {237-244},
      doi = {10.1051/0004-6361:20054522},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...452..237A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Absil2008,
   author = {{Absil}, O. and {di Folco}, E. and {M{\'e}rand}, A. and {Augereau}, J.-C. and 
	{Coud{\'e} du Foresto}, V. and {Defr{\`e}re}, D. and {Kervella}, P. and 
	{Aufdenberg}, J.~P. and {Desort}, M. and {Ehrenreich}, D. and 
	{Lagrange}, A.-M. and {Montagnier}, G. and {Olofsson}, J. and 
	{ten Brummelaar}, T.~A. and {McAlister}, H.~A. and {Sturmann}, J. and 
	{Sturmann}, L. and {Turner}, N.~H.},
    title = "{A near-infrared interferometric survey of debris disc stars. II. CHARA/FLUOR observations of six early-type dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0806.4936},
 keywords = {stars: fundamental parameters, circumstellar matter, binaries: close, methods: observational, techniques: interferometric},
     year = 2008,
    month = sep,
   volume = 487,
    pages = {1041-1054},
      doi = {10.1051/0004-6361:200810008},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487.1041A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 
@ARTICLE{Absil2009,
   author = {{Absil}, O. and {Mennesson}, B. and {Le Bouquin}, J.-B. and 
	{Di Folco}, E. and {Kervella}, P. and {Augereau}, J.-C.},
    title = "{An Interferometric Study of the Fomalhaut Inner Debris Disk. I. Near-Infrared Detection of Hot Dust with VLTI/VINCI}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.3133},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: Fomalhaut, techniques: interferometric},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {150-160},
      doi = {10.1088/0004-637X/704/1/150},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..150A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Absil2013,
   author = {{Absil}, O. and {Defr{\`e}re}, D. and {Coud{\'e} du Foresto}, V. and 
	{Di Folco}, E. and {M{\'e}rand}, A. and {Augereau}, J.-C. and 
	{Ertel}, S. and {Hanot}, C. and {Kervella}, P. and {Mollier}, B. and 
	{Scott}, N. and {Che}, X. and {Monnier}, J.~D. and {Thureau}, N. and 
	{Tuthill}, P.~G. and {ten Brummelaar}, T.~A. and {McAlister}, H.~A. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N.},
    title = "{A near-infrared interferometric survey of debris-disc stars. III. First statistics based on 42 stars observed with CHARA/FLUOR}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.2488},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, planetary systems, binaries: close, stars: fundamental parameters, techniques: interferometric},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A104},
    pages = {A104},
      doi = {10.1051/0004-6361/201321673},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A.104A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Acke2012,
   author = {{Acke}, B. and {Min}, M. and {Dominik}, C. and {Vandenbussche}, B. and 
	{Sibthorpe}, B. and {Waelkens}, C. and {Olofsson}, G. and {Degroote}, P. and 
	{Smolders}, K. and {Pantin}, E. and {Barlow}, M.~J. and {Blommaert}, J.~A.~D.~L. and 
	{Brandeker}, A. and {De Meester}, W. and {Dent}, W.~R.~F. and 
	{Exter}, K. and {Di Francesco}, J. and {Fridlund}, M. and {Gear}, W.~K. and 
	{Glauser}, A.~M. and {Greaves}, J.~S. and {Harvey}, P.~M. and 
	{Henning}, T. and {Hogerheijde}, M.~R. and {Holland}, W.~S. and 
	{Huygen}, R. and {Ivison}, R.~J. and {Jean}, C. and {Liseau}, R. and 
	{Naylor}, D.~A. and {Pilbratt}, G.~L. and {Polehampton}, E.~T. and 
	{Regibo}, S. and {Royer}, P. and {Sicilia-Aguilar}, A. and {Swinyard}, B.~M.
	},
    title = "{Herschel images of Fomalhaut. An extrasolar Kuiper belt at the height of its dynamical activity}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1204.5037},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: Fomalhaut, circumstellar matter, planetary systems, radiative transfer, zodiacal dust},
     year = 2012,
    month = apr,
   volume = 540,
      eid = {A125},
    pages = {A125},
      doi = {10.1051/0004-6361/201118581},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540A.125A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Agol2007,
   author = {{Agol}, E.},
    title = "{Rounding up the wanderers: optimizing coronagraphic searches for extrasolar planets}",
  journal = {\mnras},
   eprint = {astro-ph/0610697},
 keywords = {surveys, planetary systems},
     year = 2007,
    month = feb,
   volume = 374,
    pages = {1271-1289},
      doi = {10.1111/j.1365-2966.2006.11232.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.374.1271A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AHearn2005,
   author = {{A'Hearn}, M.~F. and {Belton}, M.~J.~S. and {Delamere}, W.~A. and 
	{Kissel}, J. and {Klaasen}, K.~P. and {McFadden}, L.~A. and 
	{Meech}, K.~J. and {Melosh}, H.~J. and {Schultz}, P.~H. and 
	{Sunshine}, J.~M. and {Thomas}, P.~C. and {Veverka}, J. and 
	{Yeomans}, D.~K. and {Baca}, M.~W. and {Busko}, I. and {Crockett}, C.~J. and 
	{Collins}, S.~M. and {Desnoyer}, M. and {Eberhardy}, C.~A. and 
	{Ernst}, C.~M. and {Farnham}, T.~L. and {Feaga}, L. and {Groussin}, O. and 
	{Hampton}, D. and {Ipatov}, S.~I. and {Li}, J.-Y. and {Lindler}, D. and 
	{Lisse}, C.~M. and {Mastrodemos}, N. and {Owen}, W.~M. and {Richardson}, J.~E. and 
	{Wellnitz}, D.~D. and {White}, R.~L.},
    title = "{Deep Impact: Excavating Comet Tempel 1}",
  journal = {Science},
     year = 2005,
    month = oct,
   volume = 310,
    pages = {258-264},
      doi = {10.1126/science.1118923},
   adsurl = {http://adsabs.harvard.edu/abs/2005Sci...310..258A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Aitken1986,
   author = {{Aitken}, D.~K. and {Briggs}, G.~P. and {Roche}, P.~F. and {Bailey}, J.~A. and 
	{Hough}, J.~H.},
    title = "{Infrared spectropolarimetry of the Galactic Centre - Magnetic alignment in the discrete sources}",
  journal = {\mnras},
 keywords = {Galactic Nuclei, Infrared Astronomy, Interstellar Magnetic Fields, Interstellar Matter, Milky Way Galaxy, Polarimetry, Infrared Spectra, Interstellar Extinction, Magnetically Trapped Particles, Silicates},
     year = 1986,
    month = jan,
   volume = 218,
    pages = {363-384},
   adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.218..363A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Aitken1989,
   author = {{Aitken}, D.~K. and {Smith}, C.~H. and {Roche}, P.~F.},
    title = "{10 and 20-micron spectropolarimetry of the BN object}",
  journal = {\mnras},
 keywords = {Infrared Astronomy, Orion Nebula, Polarimetry, Interstellar Matter, Silicates},
     year = 1989,
    month = feb,
   volume = 236,
    pages = {919-927},
   adsurl = {http://adsabs.harvard.edu/abs/1989MNRAS.236..919A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Akeson2009,
   author = {{Akeson}, R.~L. and {Ciardi}, D.~R. and {Millan-Gabet}, R. and 
	{Merand}, A. and {Folco}, E.~D. and {Monnier}, J.~D. and {Beichman}, C.~A. and 
	{Absil}, O. and {Aufdenberg}, J. and {McAlister}, H. and {ten Brummelaar}, T. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N.},
    title = "{Dust in the inner regions of debris disks around a stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0810.3701},
 keywords = {circumstellar matter, stars: individual: {$\beta$} Leo {$\zeta$} Lep},
     year = 2009,
    month = feb,
   volume = 691,
    pages = {1896-1908},
      doi = {10.1088/0004-637X/691/2/1896},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691.1896A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alexander2009,
   author = {{Alexander}, R.~D. and {Armitage}, P.~J.},
    title = "{Giant Planet Migration, Disk Evolution, and the Origin of Transitional Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.0004},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, planetary systems: formation, planetary systems: protoplanetary disks},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {989-1001},
      doi = {10.1088/0004-637X/704/2/989},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..989A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Allen2000,
   author = {{Cox}, A.~N.},
    title = "{Allen's astrophysical quantities}",
 keywords = {ASTROPHYSICS, ASTRONOMICAL CONSTANTS, TABLES, HANDBOOKS},
booktitle = {Allen's Astrophysical Quantities},
     year = 2000,
   adsurl = {http://adsabs.harvard.edu/abs/2000asqu.book.....C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andrews2005,
   author = {{Andrews}, S.~M. and {Williams}, J.~P.},
    title = "{Circumstellar Dust Disks in Taurus-Auriga: The Submillimeter Perspective}",
  journal = {\apj},
   eprint = {astro-ph/0506187},
 keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems: Protoplanetary Disks, Solar System: Formation, Stars: Pre-Main-Sequence},
     year = 2005,
    month = oct,
   volume = 631,
    pages = {1134-1160},
      doi = {10.1086/432712},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...631.1134A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andrews2007,
   author = {{Andrews}, S.~M. and {Williams}, J.~P.},
    title = "{High-Resolution Submillimeter Constraints on Circumstellar Disk Structure}",
  journal = {\apj},
   eprint = {astro-ph/0610813},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Planetary Systems: Protoplanetary Disks, Solar System: Formation, Stars: Pre-Main-Sequence},
     year = 2007,
    month = apr,
   volume = 659,
    pages = {705-728},
      doi = {10.1086/511741},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...659..705A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Andrews2011,
   author = {{Andrews}, S.~M. and {Wilner}, D.~J. and {Espaillat}, C. and 
	{Hughes}, A.~M. and {Dullemond}, C.~P. and {McClure}, M.~K. and 
	{Qi}, C. and {Brown}, J.~M.},
    title = "{Resolved Images of Large Cavities in Protoplanetary Transition Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1103.0284},
 primaryClass = "astro-ph.GA",
 keywords = {circumstellar matter, planet-disk interactions, planets and satellites: formation, protoplanetary disks, submillimeter: planetary systems},
     year = 2011,
    month = may,
   volume = 732,
      eid = {42},
    pages = {42},
      doi = {10.1088/0004-637X/732/1/42},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732...42A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ardila2004,
   author = {{Ardila}, D.~R. and {Golimowski}, D.~A. and {Krist}, J.~E. and 
	{Clampin}, M. and {Williams}, J.~P. and {Blakeslee}, J.~P. and 
	{Ford}, H.~C. and {Hartig}, G.~F. and {Illingworth}, G.~D.},
    title = "{A Resolved Debris Disk around the G2 V Star HD 107146}",
  journal = {\apj},
    year = 2004,
    month = dec,
   volume = 617,
    pages = {L147-L150}
}

@BOOK{Armitage2010,
   author = {{Armitage}, P.~J.},
    title = "{Astrophysics of Planet Formation}",
 keywords = {planets and satellites: formation, solar system: formation, protoplanetary disks, planets and satellites: dynamical evolution and stability},
booktitle = {Astrophysics of Planet Formation, by Philip J.~Armitage, pp.~294.~ISBN 978-0-521-88745-8 (hardback).~Cambridge, UK: Cambridge University Press, 2010.},
     year = 2010,
   adsurl = {http://adsabs.harvard.edu/abs/2010apf..book.....A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Artymowicz,
   author = {{Artymowicz}, P.},
    title = "{Radiation pressure forces on particles in the Beta Pictoris system}",
  journal = {\apj},,
     year = 1988,
    month = dec,
   volume = 335,
    pages = {L79-L82},
}

@INPROCEEDINGS{Asplund2005,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J.},
    title = "{The Solar Chemical Composition}",
booktitle = {Cosmic Abundances as Records of Stellar Evolution and Nucleosynthesis},
     year = 2005,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 336,
   editor = "{T.~G.~Barnes III {\&} F.~N.~Bash}",
    month = sep,
    pages = {25-38},
}

@ARTICLE{Aufdenberg2006,
   author = {{Aufdenberg}, J.~P. and {M{\'e}rand}, A. and {Coud{\'e} du Foresto}, V. and 
	{Absil}, O. and {Di Folco}, E. and {Kervella}, P. and {Ridgway}, S.~T. and 
	{Berger}, D.~H. and {ten Brummelaar}, T.~A. and {McAlister}, H.~A. and 
	{Sturmann}, J. and {Sturmann}, L. and {Turner}, N.~H.},
    title = "{First Results from the CHARA Array. VII. Long-Baseline Interferometric Measurements of Vega Consistent with a Pole-On, Rapidly Rotating Star}",
  journal = {\apj},
   eprint = {astro-ph/0603327},
 keywords = {Methods: Numerical, Stars: Atmospheres, stars: fundamental parameters (radii), stars: fundamental parameters (temperature), Stars: Individual: Name: Vega, Stars: Rotation, Techniques: Interferometric},
     year = 2006,
    month = jul,
   volume = 645,
    pages = {664-675},
      doi = {10.1086/504149},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645..664A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Augereau1999,
   author = {{Augereau}, J.~C. and {Lagrange}, A.~M. and {Mouillet}, D. and 
	{Papaloizou}, J.~C.~B. and {Grorod}, P.~A.},
    title = "{On the HR 4796 A circumstellar disk}",
  journal = {\aap},
     year = 1999,
    month = aug,
   volume = 348,
    pages = {557-569},
}

@ARTICLE{Augereau2001,
   author = {{Augereau}, J.~C. and {Nelson}, R.~P. and {Lagrange}, A.~M. and 
	{Papaloizou}, J.~C.~B. and {Mouillet}, D.},
    title = "{Dynamical modeling of large scale asymmetries in the beta Pictoris dust disk}",
  journal = {\aap},
     year = 2001,
    month = may,
   volume = 370,
    pages = {447-455},
}

@ARTICLE{Aumann1984,
   author = {{Aumann}, H.~H. and {Beichman}, C.~A. and {Gillett}, F.~C. and 
	{de Jong}, T. and {Houck}, J.~R. and {Low}, F.~J. and {Neugebauer}, G. and 
	{Walker}, R.~G. and {Wesselius}, P.~R.},
    title = "{Discovery of a shell around Alpha Lyrae}",
  journal = {\apj},
     year = 1984,
    month = mar,
   volume = 278,
    pages = {L23-L27}
}

@INPROCEEDINGS{Backman1993,
   author = {{Backman}, D.~E. and {Paresce}, F.},
    title = "{Main-sequence stars with circumstellar solid material - The VEGA phenomenon}",
 keywords = {Infrared Astronomy, Main Sequence Stars, Stellar Composition, Stellar Envelopes, Stellar Evolution, Emission Spectra, Infrared Astronomy Satellite, Photosphere},
booktitle = {Protostars and Planets III},
     year = 1993,
   editor = {{Levy}, E.~H. and {Lunine}, J.~I.},
    pages = {1253-1304},
   adsurl = {http://adsabs.harvard.edu/abs/1993prpl.conf.1253B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Backman2004,
   author = {{Backman}, D.},
    title = "{Debris Disks: An Overview}",
booktitle = {Debris Disks and the Formation of Planets},
     year = 2004,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 324,
   editor = "{L.~Caroff, L.~J.~Moon, D.~Backman, {\&} E.~Praton}",
    month = dec,
    pages = {9-19}
}

@ARTICLE{Balbus1991,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{A powerful local shear instability in weakly magnetized disks. I - Linear analysis. II - Nonlinear evolution}",
  journal = {\apj},
 keywords = {Accretion Disks, Magnetohydrodynamic Stability, Stellar Magnetic Fields, Stellar Mass Accretion, Boussinesq Approximation, Computational Astrophysics, Linear Systems},
     year = 1991,
    month = jul,
   volume = 376,
    pages = {214-233},
      doi = {10.1086/170270},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...376..214B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baliunas1983,
   author = {{Baliunas}, S.~L. and {Hartmann}, L. and {Noyes}, R.~W. and 
	{Vaughan}, H. and {Preston}, G.~W. and {Frazer}, J. and {Lanning}, H. and 
	{Middelkoop}, F. and {Mihalas}, D.},
    title = "{Stellar rotation in lower main-sequence stars measured from time variations in H and K emission-line fluxes. II - Detailed analysis of the 1980 observing season data}",
  journal = {\apj},
 keywords = {Calcium, Chromosphere, Late Stars, Main Sequence Stars, Stellar Rotation, Stellar Spectrophotometry, Autocorrelation, Giant Stars, Light Curve, Secular Variations, Stellar Radiation, Stellar Spectra, Time Series Analysis},
     year = 1983,
    month = dec,
   volume = 275,
    pages = {752-772},
      doi = {10.1086/161572},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...275..752B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Baliunas1996,
   author = {{Baliunas}, S. and {Sokoloff}, D. and {Soon}, W.},
    title = "{Magnetic Field and Rotation in Lower Main-Sequence Stars: an Empirical Time-dependent Magnetic Bode's Relation?}",
  journal = {Astrophysical Journal Letters},
 keywords = {STARS: MAGNETIC FIELDS, STARS: ROTATION},
     year = 1996,
    month = feb,
   volume = 457,
    pages = {L99},
      doi = {10.1086/309891},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...457L..99B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Banzatti2011,
   author = {{Banzatti}, A. and {Testi}, L. and {Isella}, A. and {Natta}, A. and 
	{Neri}, R. and {Wilner}, D.~J.},
    title = "{New constraints on dust grain size and distribution in CQ Tauri}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1009.2697},
 primaryClass = "astro-ph.GA",
 keywords = {protoplanetary disks, dust, extinction, circumstellar matter, stars: individual: CQ Tauri},
     year = 2011,
    month = jan,
   volume = 525,
      eid = {A12},
    pages = {A12},
      doi = {10.1051/0004-6361/201015206},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525A..12B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barabascheff1923,
   author = {{Barabascheff}, N.},
    title = "{Bestimmung der Erdalbedo und des Reflexionsgesetzes f{\"u}r die Oberfl{\"a}che der Mondmeere. Theorie der Rillen}",
  journal = {Astronomische Nachrichten},
     year = 1923,
    month = jan,
   volume = 217,
    pages = {445},
   adsurl = {http://adsabs.harvard.edu/abs/1923AN....217..445B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Barber1990,
   author = {{Barber}, P.~W. and {Hill}, S.~C.},
    title = "{Light Scattering By Particles: Computational Methods}",
  journal = {Light Scattering By Particles: Computational Methods.~Series: Advanced Series in Applied Physics},
     year = 1990,
    month = jul,
   volume = 2,
      doi = {10.1142/0784},
   adsurl = {http://adsabs.harvard.edu/abs/1990AdSAP...2.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Barrado1999,
   author = {{Barrado y Navascu{\'e}s}, D. and {Stauffer}, J.~R. and {Song}, I. and 
	{Caillault}, J.-P.},
    title = "{The Age of {$\beta$} Pictoris}",
  journal = {\apj},
   eprint = {astro-ph/9905242},
 keywords = {STARS: CIRCUMSTELLAR MATTER, STARS: INDIVIDUAL: CONSTELLATION NAME: BETA PICTORIS, STARS: KINEMATICS, Stars: Circumstellar Matter, Stars: Individual: Constellation Name: {$\beta$} Pictoris, Stars: Kinematics},
     year = 1999,
    month = aug,
   volume = 520,
    pages = {L123-L126},
      doi = {10.1086/312162},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...520L.123B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bauer1997,
   author = {{Bauer}, I. and {Finocchi}, F. and {Duschl}, W.~J. and {Gail}, H.-P. and 
	{Schloeder}, J.~P.},
    title = "{Simulation of chemical reactions and dust destruction in protoplanetary accretion disks.}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, MOLECULAR PROCESSES, SOLAR SYSTEM: FORMATION, METHODS: NUMERICAL, DUST},
     year = 1997,
    month = jan,
   volume = 317,
    pages = {273-289},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...317..273B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bastien1987,
   author = {{Bastien}, P.},
    title = "{Polarization, jets, and the distribution of circumstellar dust around T Tauri stars and other young infrared sources}",
  journal = {\apj},
 keywords = {INFRARED SOURCES (ASTRONOMY), LINEAR POLARIZATION, PRE-MAIN SEQUENCE STARS, RADIO JETS (ASTRONOMY), STELLAR ENVELOPES, T TAURI STARS, COSMIC DUST, STELLAR WINDS},
     year = 1987,
    month = jun,
   volume = 317,
    pages = {231-240},
      doi = {10.1086/165271},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...317..231B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bastien1988,
   author = {{Bastien}, P. and {Menard}, F.},
    title = "{On the interpretation of polarization maps of young stellar objects}",
  journal = {\apj},
 keywords = {EARLY STARS, POLARIZATION (WAVES), PRE-MAIN SEQUENCE STARS, STELLAR ENVELOPES, ASTRONOMICAL MAPS, WAVE SCATTERING},
     year = 1988,
    month = mar,
   volume = 326,
    pages = {334-338},
      doi = {10.1086/166095},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...326..334B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bazell1990,
   author = {{Bazell}, D. and {Dwek}, E.},
    title = "{The effects of compositional inhomogeneities and fractal dimension on the optical properties of astrophysical dust}",
  journal = {\apj},
 keywords = {COSMIC DUST, FRACTALS, INTERSTELLAR MATTER, OPTICAL PROPERTIES, ABUNDANCE, SPATIAL DISTRIBUTION},
     year = 1990,
    month = sep,
   volume = 360,
    pages = {142-150},
}


@ARTICLE{Beckwith1990,
   author = {{Beckwith}, S.~V.~W. and {Sargent}, A.~I. and {Chini}, R.~S. and 
	{Guesten}, R.},
    title = "{A survey for circumstellar disks around young stellar objects}",
  journal = {Astronomical Journal},
 keywords = {MOLECULAR CLOUDS, PRE-MAIN SEQUENCE STARS, SKY SURVEYS (ASTRONOMY), STELLAR ENVELOPES, T TAURI STARS, AURIGA CONSTELLATION, COMPUTATIONAL ASTROPHYSICS, EMISSION SPECTRA, H ALPHA LINE, MILKY WAY GALAXY, STELLAR EVOLUTION, TAURUS CONSTELLATION},
     year = 1990,
    month = mar,
   volume = 99,
    pages = {924-945},
      doi = {10.1086/115385},
   adsurl = {http://adsabs.harvard.edu/abs/1990AJ.....99..924B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beckwith1991,
   author = {{Beckwith}, S.~V.~W. and {Sargent}, A.~I.},
    title = "{Particle emissivity in circumstellar disks}",
  journal = {Astronomical Journal},
 keywords = {Particle Emission, Shell Stars, Stellar Mass Ejection, Millimeter Waves, Pre-Main Sequence Stars, Radio Stars, T Tauri Stars},
     year = 1991,
    month = nov,
   volume = 381,
    pages = {250-258},
      doi = {10.1086/170646},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...381..250B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beckwith2008,
   author = {{Beckwith}, S.~V.~W.},
    title = "{Detecting Life-bearing Extrasolar Planets with Space Telescopes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.1444},
 keywords = {extraterrestrial intelligence, planetary systems, techniques: miscellaneous, telescopes },
     year = 2008,
    month = sep,
   volume = 684,
      eid = {1404-1415},
    pages = {1404-1415},
      doi = {10.1086/590466},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...684.1404B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@PROCEEDINGS{Beichman1988,
    title = "{Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 1: Explanatory supplement}",
 keywords = {All Sky Photography, Catalogs, Indexes (Documentation), Infrared Astronomy Satellite, Cosmology, Galaxies, Star Formation, Stellar Evolution},
booktitle = {Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 1: Explanatory supplement},
     year = 1988,
   volume = 1,
   editor = {{Beichman}, C.~A. and {Neugebauer}, G. and {Habing}, H.~J. and 
	{Clegg}, P.~E. and {Chester}, T.~J.},
   adsurl = {http://adsabs.harvard.edu/abs/1988iras....1.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beichman2005,
   author = {{Beichman}, C.~A. and {Bryden}, G. and {Gautier}, T.~N. and 
	{Stapelfeldt}, K.~R. and {Werner}, M.~W. and {Misselt}, K. and 
	{Rieke}, G. and {Stansberry}, J. and {Trilling}, D.},
    title = "{An Excess Due to Small Grains around the Nearby K0 V Star HD 69830: Asteroid or Cometary Debris?}",
  journal = {\apj},
   eprint = {astro-ph/0504491},
 keywords = {Stars: Circumstellar Matter, Comets: General, Infrared: Stars, Kuiper Belt, Stars: Planetary Systems},
     year = 2005,
    month = jun,
   volume = 626,
    pages = {1061-1069},
      doi = {10.1086/430059},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...626.1061B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Beichman2006,
author = {{Beichman}, C.~A. and {Bryden}, G. and {Stapelfeldt}, K.~R. and 
	{Gautier}, T.~N. and {Grogan}, K. and {Shao}, M. and {Velusamy}, T. and 
	{Lawler}, S.~M. and {Blaylock}, M. and {Rieke}, G.~H. and {Lunine}, J.~I. and 
	{Fischer}, D.~A. and {Marcy}, G.~W. and {Greaves}, J.~S. and 
	{Wyatt}, M.~C. and {Holland}, W.~S. and {Dent}, W.~R.~F.},
    title = "{New Debris Disks around Nearby Main-Sequence Stars: Impact on the Direct Detection of Planets}",
  journal = {\apj},
   eprint = {astro-ph/0611682},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Kuiper Belt},
     year = 2006,
    month = dec,
   volume = 652,
    pages = {1674-1693},
      doi = {10.1086/508449},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652.1674B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bell1997,
   author = {{Bell}, K.~R. and {Cassen}, P.~M. and {Klahr}, H.~H. and {Henning}, T.},
    title = "{The Structure and Appearance of Protostellar Accretion Disks: Limits on Disk Flaring}",
  journal = {\apj},
 keywords = {Accretion, Accretion Disks, Radiative Transfer, Stars: Pre-Main-Sequence},
     year = 1997,
    month = sep,
   volume = 486,
    pages = {372-387},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...486..372B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bernstein2004,
   author = {{Bernstein}, G.~M. and {Trilling}, D.~E. and {Allen}, R.~L. and 
	{Brown}, M.~E. and {Holman}, M. and {Malhotra}, R.},
    title = "{The Size Distribution of Trans-Neptunian Bodies}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/0308467},
 keywords = {Kuiper Belt, Solar System: Formation},
     year = 2004,
    month = sep,
   volume = 128,
    pages = {1364-1390},
      doi = {10.1086/422919},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128.1364B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bertone2004,
   author = {{Bertone}, E. and {Buzzoni}, A. and {Ch{\'a}vez}, M. and {Rodr{\'{\i}}guez-Merino}, L.~H.
	},
    title = "{ATLAS Versus NextGen Model Atmospheres: A Combined Analysis of Synthetic Spectral Energy Distributions}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/0406215},
 keywords = {Stars: Atmospheres, Stars: Fundamental Parameters},
     year = 2004,
    month = aug,
   volume = 128,
    pages = {829-841},
      doi = {10.1086/422486},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128..829B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bertrang2014,
   author = {{Bertrang}, G.~H.-M. and {Wolf}, S. and {Das}, H.~S.},
    title = "{Large-scale magnetic fields in Bok globules}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1404.5597},
 primaryClass = "astro-ph.SR",
 keywords = {magnetic fields, polarization, stars: formation, stars: low-mass, ISM: clouds, instrumentation: polarimeters},
     year = 2014,
    month = may,
   volume = 565,
      eid = {A94},
    pages = {A94},
      doi = {10.1051/0004-6361/201323091},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...565A..94B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertrang2015Dok,
   author = {{Bertrang}, G.~H.-M.},
    title = "{Polarized Radiation As Tracer Of Magnetic Fields In Star
      Formation}",
 journal = {Dissertation, in Vorbereitung},
     year = 2015,
}

@ARTICLE{Beuzit1997,
   author = {{Beuzit}, J.-L. and {Mouillet}, D. and {Lagrange}, A.-M. and 
	{Paufique}, J.},
    title = "{A stellar coronograph for the COME-ON-PLUS adaptive optics system}",
  journal = {\aap},
     year = 1997,
    month = oct,
   volume = 125,
    pages = {175-182},
}

@BOOK{BinneyMerrifield,
   author = {{Binney}, J. and {Merrifield}, M.},
    title = "{Galactic Astronomy, Princeton, NJ : Princeton University Press, (Princeton series in astrophysics)}",
     year = 1998,
}

@ARTICLE{Birnstiel2010,
   author = {{Birnstiel}, T. and {Ricci}, L. and {Trotta}, F. and {Dullemond}, C.~P. and 
	{Natta}, A. and {Testi}, L. and {Dominik}, C. and {Henning}, T. and 
	{Ormel}, C.~W. and {Zsom}, A.},
    title = "{Testing the theory of grain growth and fragmentation by millimeter observations of protoplanetary disks}",
    journal = {\aap},
     year = 2010,
    month = jun,
   volume = 516,
    pages = {L14},
}


@ARTICLE{BjorkmanWood2001,
   author = {{Bjorkman}, J.~E. and {Wood}, K.},
    title = "{Radiative Equilibrium and Temperature Correction in Monte Carlo Radiation Transfer}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0103249},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Radiative Transfer, Scattering},
     year = 2001,
    month = jun,
   volume = 554,
    pages = {615-623},
      doi = {10.1086/321336},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554..615B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Blum2000,
   author = {{Blum}, J. and {Wurm}, G. and {Kempf}, S. and {Poppe}, T. and 
	{Klahr}, H. and {Kozasa}, T. and {Rott}, M. and {Henning}, T. and 
	{Dorschner}, J. and {Schr{\"a}pler}, R. and {Keller}, H.~U. and 
	{Markiewicz}, W.~J. and {Mann}, I. and {Gustafson}, B.~A. and 
	{Giovane}, F. and {Neuhaus}, D. and {Fechtig}, H. and {Gr{\"u}n}, E. and 
	{Feuerbacher}, B. and {Kochan}, H. and {Ratke}, L. and {El Goresy}, A. and 
	{Morfill}, G. and {Weidenschilling}, S.~J. and {Schwehm}, G. and 
	{Metzler}, K. and {Ip}, W.-H.},
    title = "{Growth and Form of Planetary Seedlings: Results from a Microgravity Aggregation Experiment}",
  journal = {Physical Review Letters},
     year = 2000,
    month = sep,
   volume = 85,
    pages = {2426-2429},
      doi = {10.1103/PhysRevLett.85.2426},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhRvL..85.2426B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{BlumWurm2008,
   author = {{Blum}, J. and {Wurm}, G.},
    title = "{The Growth Mechanisms of Macroscopic Bodies in Protoplanetary Disks}",
  journal = {Annual Review of Astronomy {\&} Astrophysics},
     year = 2008,
    month = sep,
   volume = 46,
    pages = {21-56}
}

@BOOK{BohrenHuffman83,
   author = {{Bohren}, C.~F. and {Huffman}, D.~R.},
    title = "{Absorption and scattering of light by small particles}",
booktitle = {New York: Wiley, 1983},
     year = 1983,
   editor = "{Bohren, C.~F.~{\&} Huffman, D.~R.}",
}

@ARTICLE{Boyajian2013,
   author = {{Boyajian}, T.~S. and {von Braun}, K. and {van Belle}, G. and 
	{Farrington}, C. and {Schaefer}, G. and {Jones}, J. and {White}, R. and 
	{McAlister}, H.~A. and {ten Brummelaar}, T.~A. and {Ridgway}, S. and 
	{Gies}, D. and {Sturmann}, L. and {Sturmann}, J. and {Turner}, N.~H. and 
	{Goldfinger}, P.~J. and {Vargas}, N.},
    title = "{Stellar Diameters and Temperatures. III. Main-sequence A, F, G, and K Stars: Additional High-precision Measurements and Empirical Relations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.2974},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and C-M diagrams, infrared: stars, planetary systems, stars: atmospheres, stars: fundamental parameters, stars: general, stars: solar-type, techniques: high angular resolution, techniques: interferometric},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/771/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...40B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boley2012,
   author = {{Boley}, A.~C. and {Payne}, M.~J. and {Corder}, S. and {Dent}, W.~R.~F. and 
	{Ford}, E.~B. and {Shabram}, M.},
    title = "{Constraining the Planetary System of Fomalhaut Using High-resolution ALMA Observations}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1204.0007},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, planet-disk interactions, submillimeter: planetary systems},
     year = 2012,
    month = may,
   volume = 750,
      eid = {L21},
    pages = {L21},
      doi = {10.1088/2041-8205/750/1/L21},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750L..21B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonsor2012,
   author = {{Bonsor}, A. and {Augereau}, J.-C. and {Th{\'e}bault}, P.},
    title = "{Scattering of small bodies by planets: a potential origin for exozodiacal dust?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1209.6033},
 primaryClass = "astro-ph.EP",
 keywords = {methods: numerical, comets: general, planets and satellites: dynamical evolution and stability, zodiacal dust, planet-disk interactions, circumstellar matter},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A104},
    pages = {A104},
      doi = {10.1051/0004-6361/201220005},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A.104B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonsor2013,
   author = {{Bonsor}, A. and {Raymond}, S.~N. and {Augereau}, J.-C.},
    title = "{The short-lived production of exozodiacal dust in the aftermath of a dynamical instability in planetary systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1306.0592},
 primaryClass = "astro-ph.EP",
 keywords = {methods: numerical, planets and satellites: dynamical evolution and stability, planets and satellites: general, zodiacal dust, planetary systems},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {2938-2945},
      doi = {10.1093/mnras/stt933},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.2938B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonsor2013a,
   author = {{Bonsor}, A. and {Kennedy}, G.~M. and {Crepp}, J.~R. and {Johnson}, J.~A. and 
	{Wyatt}, M.~C. and {Sibthorpe}, B. and {Su}, K.~Y.~L.},
    title = "{Spatially resolved images of dust belt(s) around the planet-hosting subgiant {$\kappa$} CrB}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1302.7000},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: high angular resolution, techniques: radial velocities, planets and satellites: detection, planets and satellites: individual: {$\kappa$} CrB, planet-disc interactions, infrared: planetary systems},
     year = 2013,
    month = jun,
   volume = 431,
    pages = {3025-3035},
      doi = {10.1093/mnras/stt367},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.3025B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Booth2013,
   author = {{Booth}, M. and {Kennedy}, G. and {Sibthorpe}, B. and {Matthews}, B.~C. and 
	{Wyatt}, M.~C. and {Duch{\^e}ne}, G. and {Kavelaars}, J.~J. and 
	{Rodriguez}, D. and {Greaves}, J.~S. and {Koning}, A. and {Vican}, L. and 
	{Rieke}, G.~H. and {Su}, K.~Y.~L. and {Moro-Mart{\'{\i}}n}, A. and 
	{Kalas}, P.},
    title = "{Resolved debris discs around A stars in the Herschel DEBRIS survey}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1210.0547},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, stars: individual: {$\alpha$} CrB, {$\beta$} Uma, {$\lambda$} Boo, {$\epsilon$} Pav, {$\zeta$} Eri, {$\gamma$} Tri, {$\rho$} Vir, 30 Mon, {$\beta$} Tri, planetary systems, infrared: stars},
     year = 2013,
    month = jan,
   volume = 428,
    pages = {1263-1280},
      doi = {10.1093/mnras/sts117},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.1263B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bouwman2003,
   author = {{Bouwman}, J. and {de Koter}, A. and {Dominik}, C. and {Waters}, L.~B.~F.~M.
	},
    title = "{The origin of crystalline silicates in the Herbig Be star HD 100546 and in comet Hale-Bopp}",
   journal = {\aap},
   eprint = {astro-ph/0301254},
 keywords = {circumstellar matter, stars: formation, stars: pre-main-sequence},
     year = 2003,
    month = apr,
   volume = 401,
    pages = {577-592},
      doi = {10.1051/0004-6361:20030043},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...401..577B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Brandner2005,
      author        = "Brandner, Wolfgang and Kasper, Markus E",
      title         = "{Science with Adaptive Optics: Proceedings of the ESO
                       Workshop Held at Garching, Germany, 16-19 September 2003}",
      publisher     = "Springer",
      address       = "Berlin",
      series        = "ESO Astrophysics Symposia",
      year          = "2005",
}

@book{Bronstein,
  author = {Ilja N. Bronstein ,Konstantin A. Semendjajew , Gerhard Musiol},
  publisher = {Deutsch (Harri)},
  title = {Taschenbuch der Mathematik},
  year = 2006,
  isbn = {3817120062},
}

@INPROCEEDINGS{Brott2005,
   author = {{Brott}, I. and {Hauschildt}, P.~H.},
    title = "{A PHOENIX Model Atmosphere Grid for Gaia}",
 keywords = {Stars atmospheres, Stars late-type, Radiative transfer, Gaia},
booktitle = {The Three-Dimensional Universe with Gaia},
     year = 2005,
   series = {ESA Special Publication},
   volume = 576,
   eprint = {astro-ph/0503395},
   editor = {{Turon}, C. and {O'Flaherty}, K.~S. and {Perryman}, M.~A.~C.
	},
    month = jan,
    pages = {565},
   adsurl = {http://adsabs.harvard.edu/abs/2005ESASP.576..565B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Brown1986,
   author = {{Brown}, A. and {Drake}, S.~A. and {Mundt}, R.},
    title = "{Multifrequency VLA Observations of the Pre-Main Sequence Stars HL TAU, XZ TAU, FS TAU A and FS TAU B}",
booktitle = {Cool Stars, Stellar Systems and the Sun},
     year = 1986,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 254,
   editor = {{Zeilik}, M. and {Gibson}, D.~M.},
    pages = {451},
      doi = {10.1007/3-540-16763-3_236},
   adsurl = {http://adsabs.harvard.edu/abs/1986LNP...254..451B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Brownlee1977,
   author = {{Brownlee}, D.~E. and {Tomandl}, D.~A. and {Olszewski}, E.},
    title = "{Interplanetary dust - A new source of extraterrestrial material for laboratory studies}",
 keywords = {Comets, Extraterrestrial Matter, Interplanetary Dust, Meteoritic Composition, Micrometeoroids, Atmospheric Entry, Chondrites, Iron, Microparticles, Olivine, Particulate Sampling, Pyroxenes, Stratosphere},
booktitle = {Lunar and Planetary Science Conference Proceedings},
     year = 1977,
   series = {Lunar and Planetary Science Conference Proceedings},
   volume = 8,
   editor = {{Merril}, R.~B.},
    pages = {149-160},
   adsurl = {http://adsabs.harvard.edu/abs/1977LPSC....8..149B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brownlee1985,
   author = {{Brownlee}, D.~E.},
    title = "{Cosmic dust - Collection and research}",
  journal = {Annual Review of Earth and Planetary Sciences},
 keywords = {Cosmic Dust, Interplanetary Dust, Particles, Samples, Extraterrestrial, Sampling, Abundance, Analysis, Origin, Evolution, Laboratory Studies},
     year = 1985,
   volume = 13,
    pages = {147-173},
      doi = {10.1146/annurev.ea.13.050185.001051},
   adsurl = {http://adsabs.harvard.edu/abs/1985AREPS..13..147B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Bruggeman1935,
 author={{Bruggeman}, D.~A.~G.},
 title={Berechnung verschiedener physikalischer Konstanten von heterogenen Substanzen. I. Dielektrizitätskonstanten und Leitfähigkeiten der Mischkörper aus isotropen Substanzen},
 journal={Annalen der Physik},
 volume={416},
number={7},
 year={1935},
pages={636-664}
}

@ARTICLE{Bryden2006,
   author = {{Bryden}, G. and {Beichman}, C.~A. and {Trilling}, D.~E. and 
	{Rieke}, G.~H. and {Holmes}, E.~K. and {Lawler}, S.~M. and {Stapelfeldt}, K.~R. and 
	{Werner}, M.~W. and {Gautier}, T.~N. and {Blaylock}, M. and 
	{Gordon}, K.~D. and {Stansberry}, J.~A. and {Su}, K.~Y.~L.},
    title = "{Frequency of Debris Disks around Solar-Type Stars: First Results from a Spitzer MIPS Survey}",
   journal = {\apj},
   eprint = {astro-ph/0509199},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Kuiper Belt-planetary systems: formation},
     year = 2006,
    month = jan,
   volume = 636,
    pages = {1098-1113},
      doi = {10.1086/498093},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636.1098B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Burns1979,
   author = {{Burns}, J.~A. and {Lamy}, P.~L. and {Soter}, S.},
    title = "{Radiation forces on small particles in the solar system}",
  journal = {\icarus},
 keywords = {Interplanetary Dust, Particle Motion, Poynting-Robertson Effect, Radiation Pressure, Solar Radiation, Heuristic Methods, Pressure Effects, Relativity, Solar Rotation, Solar System, Solar Wind},
     year = 1979,
    month = oct,
   volume = 40,
    pages = {1-48},
      doi = {10.1016/0019-1035(79)90050-2},
   adsurl = {http://adsabs.harvard.edu/abs/1979Icar...40....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows1996,
   author = {{Burrows}, C.~J. and {Stapelfeldt}, K.~R. and {Watson}, A.~M. and 
	{Krist}, J.~E. and {Ballester}, G.~E. and {Clarke}, J.~T. and 
	{Crisp}, D. and {Gallagher}, III, J.~S. and {Griffiths}, R.~E. and 
	{Hester}, J.~J. and {Hoessel}, J.~G. and {Holtzman}, J.~A. and 
	{Mould}, J.~R. and {Scowen}, P.~A. and {Trauger}, J.~T. and 
	{Westphal}, J.~A.},
    title = "{Hubble Space Telescope Observations of the Disk and Jet of HH 30}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, ISM: DUST, EXTINCTION, ISM: JETS AND OUTFLOWS, STARS: PRE-MAIN-SEQUENCE, STARS: INDIVIDUAL ALPHANUMERIC: HH 30},
     year = 1996,
    month = dec,
   volume = 473,
    pages = {437},
      doi = {10.1086/178156},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...473..437B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cameron1962,
   author = {{Cameron}, A.~G.~W.},
    title = "{The formation of the sun and planets}",
  journal = {Icarus},
     year = 1962,
   volume = 1,
    pages = {13-69},
      doi = {10.1016/0019-1035(62)90005-2},
   adsurl = {http://adsabs.harvard.edu/abs/1962Icar....1...13C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cameron1973,
   author = {{Cameron}, A.~G.~W.},
    title = "{Accumulation processes in the primitive solar nebula}",
  journal = {Icarus},
     year = 1973,
    month = mar,
   volume = 18,
    pages = {407-450},
      doi = {10.1016/0019-1035(73)90153-X},
   adsurl = {http://adsabs.harvard.edu/abs/1973Icar...18..407C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@book{CashwellEverett1959,
  author={Cashwell, E.D. and Everett, C.J.},
  title={A practical manual on the Monte Carlo method for random walk problems},
  lccn={59010519},
  series={International tracts in computer science and technology and their application},
  url={http://books.google.de/books?id=-so-AAAAIAAJ},
  year={1959},
  publisher={Pergamon Press}
}

@ARTICLE{Chandrasekhar1946,
   author = {{Chandrasekhar}, S.},
    title = "{On the Radiative Equilibrium of a Stellar Atmosphere. XI.}",
  journal = {\apj},
     year = 1946,
    month = jul,
   volume = 104,
    pages = {110},
      doi = {10.1086/144837},
   adsurl = {http://adsabs.harvard.edu/abs/1946ApJ...104..110C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen2005,
   author = {{Chen}, C.~H. and {Patten}, B.~M. and {Werner}, M.~W. and {Dowell}, C.~D. and 
	{Stapelfeldt}, K.~R. and {Song}, I. and {Stauffer}, J.~R. and 
	{Blaylock}, M. and {Gordon}, K.~D. and {Krause}, V.},
    title = "{A Spitzer Study of Dusty Disks around Nearby, Young Stars}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems: Formation},
     year = 2005,
    month = dec,
   volume = 634,
    pages = {1372-1384},
      doi = {10.1086/497124},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1372C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chen2006,
   author = {{Chen}, C.~H. and {Sargent}, B.~A. and {Bohac}, C. and {Kim}, K.~H. and 
	{Leibensperger}, E. and {Jura}, M. and {Najita}, J. and {Forrest}, W.~J. and 
	{Watson}, D.~M. and {Sloan}, G.~C. and {Keller}, L.~D.},
    title = "{Spitzer IRS Spectroscopy of IRAS-discovered Debris Disks}",
  journal = {\apjs},
   eprint = {astro-ph/0605277},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Planetary Systems: Formation},
     year = 2006,
    month = sep,
   volume = 166,
    pages = {351-377},
      doi = {10.1086/505751},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..166..351C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen2014,
   author = {{Chen}, C.~H. and {Mittal}, T. and {Kuchner}, M. and {Forrest}, W.~J. and 
	{Lisse}, C.~M. and {Manoj}, P. and {Sargent}, B.~A. and {Watson}, D.~M.
	},
    title = "{The Spitzer Infrared Spectrograph Debris Disk Catalog. I. Continuum Analysis of Unresolved Targets}",
  journal = {\apjs},
 keywords = {catalogs, circumstellar matter, infrared: stars, zodiacal dust},
     year = 2014,
    month = apr,
   volume = 211,
      eid = {25},
    pages = {25},
      doi = {10.1088/0067-0049/211/2/25},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..211...25C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{ChiangGoldreich1997,
   author = {{Chiang}, E.~I. and {Goldreich}, P.},
    title = "{Spectral Energy Distributions of T Tauri Stars with Passive Circumstellar Disks}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9706042},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, INFRARED: STARS, RADIATIVE TRANSFER, STARS: PRE-MAIN-SEQUENCE},
     year = 1997,
    month = nov,
   volume = 490,
    pages = {368},
      doi = {10.1086/304869},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...490..368C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chiar2006,
   author = {{Chiar}, J.~E. and {Tielens}, A.~G.~G.~M.},
    title = "{Pixie Dust: The Silicate Features in the Diffuse Interstellar Medium}",
  journal = {\apj},
   eprint = {astro-ph/0510156},
 keywords = {ISM: Dust, Extinction, Infrared: ISM, ISM: Abundances, ISM: Lines and Bands, ISM: Molecules},
     year = 2006,
    month = feb,
   volume = 637,
    pages = {774-785},
      doi = {10.1086/498406},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...637..774C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cho2007,
   author = {{Cho}, J. and {Lazarian}, A.},
    title = "{Polarization of FIR Emission From T Tauri Disks}",
  journal = {Journal of Korean Astronomical Society},
 keywords = {accretion, accretion disks ---circumstellar matter, polarization, stars: pre-main-sequence, dust, extinctio},
     year = 2007,
   volume = 40,
    pages = {113-118},
      doi = {10.5303/JKAS.2007.40.4.113},
   adsurl = {http://adsabs.harvard.edu/abs/2007JKAS...40..113C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Churcher2011,
   author = {{Churcher}, L.~J. and {Wyatt}, M.~C. and {Duch{\^e}ne}, G. and 
	{Sibthorpe}, B. and {Kennedy}, G. and {Matthews}, B.~C. and 
	{Kalas}, P. and {Greaves}, J. and {Su}, K. and {Rieke}, G.},
    title = "{Multiwavelength modelling of the {$\beta$} Leo debris disc: one, two or three planetesimal populations?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1107.0316},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: {$\beta$} Leo, planetary systems},
     year = 2011,
    month = nov,
   volume = 417,
    pages = {1715-1734},
      doi = {10.1111/j.1365-2966.2011.19341.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.1715C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Chylek1983,
   author = {{Ch{\'y}lek}, P. and {Srivastava}, V.},
    title = "{Dielectric constant of a composite inhomogeneous medium}",
  journal = {Physical Review B (Condensed Matter)},
     year = 1983,
    month = apr,
   volume = 27,
    pages = {5098-5106},
      doi = {10.1103/PhysRevB.27.5098},
   adsurl = {http://adsabs.harvard.edu/abs/1983PhRvB..27.5098C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clayton2004,
   author = {{Clayton}, D.~D. and {Nittler}, L.~R.},
    title = "{Astrophysics with Presolar Stardust}",
  journal = {Annual Review of Astronomy {\&} Astrophysics},
     year = 2004,
    month = sep,
   volume = 42,
    pages = {39-78},
      doi = {10.1146/annurev.astro.42.053102.134022},
   adsurl = {http://adsabs.harvard.edu/abs/2004ARA%26A..42...39C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cohen1979,
   author = {{Cohen}, M. and {Kuhi}, L.~V.},
    title = "{Observational studies of pre-main-sequence evolution}",
  journal = {\apjs},
 keywords = {Main Sequence Stars, Stellar Evolution, Stellar Spectra, Stellar Spectrophotometry, Astronomical Catalogs, Binary Stars, Emission Spectra, Hertzsprung-Russell Diagram, Infrared Astronomy, Line Spectra, Optical Scanners, Stellar Luminosity, Stellar Temperature},
     year = 1979,
    month = dec,
   volume = 41,
    pages = {743-843},
      doi = {10.1086/190641},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJS...41..743C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Connelley2007,
   author = {{Connelley}, M.~S. and {Reipurth}, B. and {Tokunaga}, A.~T.},
    title = "{Infrared Nebulae around Young Stellar Objects}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/0611634},
 keywords = {atlases, infrared: ISM, reflection nebulae, stars: formation},
     year = 2007,
    month = apr,
   volume = 133,
    pages = {1528-1559},
      doi = {10.1086/511745},
   adsurl = {http://adsabs.harvard.edu/abs/2007AJ....133.1528C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Corder2009,
   author = {{Corder}, S. and {Carpenter}, J.~M. and {Sargent}, A.~I. and 
	{Zauderer}, B.~A. and {Wright}, M.~C.~H. and {White}, S.~M. and 
	{Woody}, D.~P. and {Teuben}, P. and {Scott}, S.~L. and {Pound}, M.~W. and 
	{Plambeck}, R.~L. and {Lamb}, J.~W. and {Koda}, J. and {Hodges}, M. and 
	{Hawkins}, D. and {Bock}, D.~C.-J.},
    title = "{A Resolved Ring of Debris Dust around the Solar Analog HD 107146}",
  journal = {\apj},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {L65-L68},
}


@ARTICLE{Cotera2001,
   author = {{Cotera}, A.~S. and {Whitney}, B.~A. and {Young}, E. and {Wolff}, M.~J. and 
	{Wood}, K. and {Povich}, M. and {Schneider}, G. and {Rieke}, M. and 
	{Thompson}, R.},
    title = "{High-Resolution Near-Infrared Images and Models of the Circumstellar Disk in HH 30}",
  journal = {\apj},,
   eprint = {arXiv:astro-ph/0104066},
 keywords = {Accretion, Accretion Disks, Radiative Transfer, stars: individual (HH 30), Stars: Pre-Main-Sequence, Stars: Rotation, Stars: Spots},
     year = 2001,
    month = aug,
   volume = 556,
    pages = {958-969},
      doi = {10.1086/321627},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..958C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Craig2013,
   author = {{Craig}, J. and {Krumholz}, M.~R.},
    title = "{Close Stellar Encounters in Young, Substructured, Dissolving Star Clusters: Statistics and Effects on Planetary Systems}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1304.7683},
 primaryClass = "astro-ph.EP",
 keywords = {open clusters and associations: general, planets and satellites: formation, stars: kinematics and dynamics },
     year = 2013,
    month = jun,
   volume = 769,
      eid = {150},
    pages = {150},
      doi = {10.1088/0004-637X/769/2/150},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769..150C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Czechowski2010,
   author = {{Czechowski}, A. and {Mann}, I.},
    title = "{Formation and Acceleration of Nano Dust in the Inner Heliosphere}",
  journal = {\apj},
 keywords = {acceleration of particles, interplanetary medium, solar wind},
     year = 2010,
    month = may,
   volume = 714,
      eid = {89-99},
    pages = {89-99},
      doi = {10.1088/0004-637X/714/1/89},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714...89C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DAlessio1998,
   author = {{D'Alessio}, P. and {Canto}, J. and {Calvet}, N. and {Lizano}, S.	},
    title = "{Accretion Disks around Young Objects. I. The Detailed Vertical Structure}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9806060},
 keywords = {ACCRETION, ACCRETION DISKS, RADIATIVE TRANSFER, STARS: PRE-MAIN-SEQUENCE},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {411},
      doi = {10.1086/305702},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..411D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DAlessio1999,
   author = {{D'Alessio}, P. and {Calvet}, N. and {Hartmann}, L. and {Lizano}, S. and 
	{Cant{\'o}}, J.},
    title = "{Accretion Disks around Young Objects. II. Tests of Well-mixed Models with ISM Dust}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9907330},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, ISM: DUST, EXTINCTION, STARS: PRE-MAIN-SEQUENCE},
     year = 1999,
    month = dec,
   volume = 527,
    pages = {893-909},
      doi = {10.1086/308103},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...527..893D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DAlessio2001,
   author = {{D'Alessio}, P. and {Calvet}, N. and {Hartmann}, L.},
    title = "{Accretion Disks around Young Objects. III. Grain Growth}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0101443},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2001,
    month = may,
   volume = 553,
    pages = {321-334},
      doi = {10.1086/320655},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553..321D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Daniel1978,
   author = {{Daniel}, J.-Y.},
    title = "{Monte Carlo simulation of light transfer in circumstellar dust shells}",
  journal = {\aap},
 keywords = {COSMIC DUST, LIGHT SCATTERING, POLARIZED LIGHT, RADIATIVE TRANSFER, STELLAR ENVELOPES, COMPUTERIZED SIMULATION, GRAPHITE, IRON, MONTE CARLO METHOD, PHOTONS, SILICATES},
     year = 1978,
    month = jul,
   volume = 67,
    pages = {345-353},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26A....67..345D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Daniel1980,
   author = {{Daniel}, J.-Y.},
    title = "{Monte Carlo analysis of polarization by Mie scattering in circumstellar envelopes}",
  journal = {\aap},
 keywords = {ELECTROMAGNETIC SCATTERING, MIE SCATTERING, MONTE CARLO METHOD, POLARIZATION CHARACTERISTICS, STELLAR ENVELOPES, CIRCULAR POLARIZATION, INTERSTELLAR EXTINCTION, REFRACTIVITY, STELLAR RADIATION},
     year = 1980,
    month = jul,
   volume = 87,
    pages = {204-209},
   adsurl = {http://adsabs.harvard.edu/abs/1980A%26A....87..204D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Daniel1982,
   author = {{Daniel}, J.-Y.},
    title = "{Monte Carlo study of highly polarized cool stars}",
  journal = {\aap},
 keywords = {COOL STARS, LATE STARS, LIGHT SCATTERING, MONTE CARLO METHOD, POLARIZATION CHARACTERISTICS, POLARIZED LIGHT, STELLAR ENVELOPES, BIPOLARITY, M STARS, MIE SCATTERING, NEBULAE, POLARIMETRY, STELLAR LUMINOSITY, STELLAR TEMPERATURE},
     year = 1982,
    month = jul,
   volume = 111,
    pages = {58-70},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...111...58D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Debye1909,
   author = {{Debye}, P.},
    title = "{Der Lichtdruck auf Kugeln von beliebigem Material}",
  journal = {Annalen der Physik},
     year = 1909,
   volume = 335,
    pages = {57-136},
      doi = {10.1002/andp.19093351103},
   adsurl = {http://adsabs.harvard.edu/abs/1909AnP...335...57D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Defrere2011,
   author = {{Defr{\`e}re}, D. and {Absil}, O. and {Augereau}, J.-C. and 
	{di Folco}, E. and {Berger}, J.-P. and {Coud{\'e} du Foresto}, V. and 
	{Kervella}, P. and {Le Bouquin}, J.-B. and {Lebreton}, J. and 
	{Millan-Gabet}, R. and {Monnier}, J.~D. and {Olofsson}, J. and 
	{Traub}, W.},
    title = "{Hot exozodiacal dust resolved around Vega with IOTA/IONIC}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1108.3698},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: high angular resolution, techniques: interferometric, circumstellar matter},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A5},
    pages = {A5},
      doi = {10.1051/0004-6361/201117017},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A...5D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Defrere2012,
   author = {{Defr{\`e}re}, D. and {Lebreton}, J. and {Le Bouquin}, J.-B. and 
	{Lagrange}, A.-M. and {Absil}, O. and {Augereau}, J.-C. and 
	{Berger}, J.-P. and {di Folco}, E. and {Ertel}, S. and {Kluska}, J. and 
	{Montagnier}, G. and {Millan-Gabet}, R. and {Traub}, W. and 
	{Zins}, G.},
    title = "{Hot circumstellar material resolved around <ASTROBJ>{$\beta$} Pic</ASTROBJ> with VLTI/PIONIER}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1210.1914},
 primaryClass = "astro-ph.SR",
 keywords = {instrumentation: high angular resolution, techniques: interferometric, infrared: planetary systems},
     year = 2012,
    month = oct,
   volume = 546,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201220287},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...546L...9D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deGraauw2010,
   author = {{de Graauw}, T. and {Helmich}, F.~P. and {Phillips}, T.~G. and 
	{Stutzki}, J. and {Caux}, E. and {Whyborn}, N.~D. and {Dieleman}, P. and 
	{Roelfsema}, P.~R. and {Aarts}, H. and {Assendorp}, R. and {Bachiller}, R. and 
	{Baechtold}, W. and {Barcia}, A. and {Beintema}, D.~A. and {Belitsky}, V. and 
	{Benz}, A.~O. and {Bieber}, R. and {Boogert}, A. and {Borys}, C. and 
	{Bumble}, B. and {Ca{\"i}s}, P. and {Caris}, M. and {Cerulli-Irelli}, P. and 
	{Chattopadhyay}, G. and {Cherednichenko}, S. and {Ciechanowicz}, M. and 
	{Coeur-Joly}, O. and {Comito}, C. and {Cros}, A. and {de Jonge}, A. and 
	{de Lange}, G. and {Delforges}, B. and {Delorme}, Y. and {den Boggende}, T. and 
	{Desbat}, J.-M. and {Diez-Gonz{\'a}lez}, C. and {di Giorgio}, A.~M. and 
	{Dubbeldam}, L. and {Edwards}, K. and {Eggens}, M. and {Erickson}, N. and 
	{Evers}, J. and {Fich}, M. and {Finn}, T. and {Franke}, B. and 
	{Gaier}, T. and {Gal}, C. and {Gao}, J.~R. and {Gallego}, J.-D. and 
	{Gauffre}, S. and {Gill}, J.~J. and {Glenz}, S. and {Golstein}, H. and 
	{Goulooze}, H. and {Gunsing}, T. and {G{\"u}sten}, R. and {Hartogh}, P. and 
	{Hatch}, W.~A. and {Higgins}, R. and {Honingh}, E.~C. and {Huisman}, R. and 
	{Jackson}, B.~D. and {Jacobs}, H. and {Jacobs}, K. and {Jarchow}, C. and 
	{Javadi}, H. and {Jellema}, W. and {Justen}, M. and {Karpov}, A. and 
	{Kasemann}, C. and {Kawamura}, J. and {Keizer}, G. and {Kester}, D. and 
	{Klapwijk}, T.~M. and {Klein}, T. and {Kollberg}, E. and {Kooi}, J. and 
	{Kooiman}, P.-P. and {Kopf}, B. and {Krause}, M. and {Krieg}, J.-M. and 
	{Kramer}, C. and {Kruizenga}, B. and {Kuhn}, T. and {Laauwen}, W. and 
	{Lai}, R. and {Larsson}, B. and {Leduc}, H.~G. and {Leinz}, C. and 
	{Lin}, R.~H. and {Liseau}, R. and {Liu}, G.~S. and {Loose}, A. and 
	{L{\'o}pez-Fernandez}, I. and {Lord}, S. and {Luinge}, W. and 
	{Marston}, A. and {Mart{\'{\i}}n-Pintado}, J. and {Maestrini}, A. and 
	{Maiwald}, F.~W. and {McCoey}, C. and {Mehdi}, I. and {Megej}, A. and 
	{Melchior}, M. and {Meinsma}, L. and {Merkel}, H. and {Michalska}, M. and 
	{Monstein}, C. and {Moratschke}, D. and {Morris}, P. and {Muller}, H. and 
	{Murphy}, J.~A. and {Naber}, A. and {Natale}, E. and {Nowosielski}, W. and 
	{Nuzzolo}, F. and {Olberg}, M. and {Olbrich}, M. and {Orfei}, R. and 
	{Orleanski}, P. and {Ossenkopf}, V. and {Peacock}, T. and {Pearson}, J.~C. and 
	{Peron}, I. and {Phillip-May}, S. and {Piazzo}, L. and {Planesas}, P. and 
	{Rataj}, M. and {Ravera}, L. and {Risacher}, C. and {Salez}, M. and 
	{Samoska}, L.~A. and {Saraceno}, P. and {Schieder}, R. and {Schlecht}, E. and 
	{Schl{\"o}der}, F. and {Schm{\"u}lling}, F. and {Schultz}, M. and 
	{Schuster}, K. and {Siebertz}, O. and {Smit}, H. and {Szczerba}, R. and 
	{Shipman}, R. and {Steinmetz}, E. and {Stern}, J.~A. and {Stokroos}, M. and 
	{Teipen}, R. and {Teyssier}, D. and {Tils}, T. and {Trappe}, N. and 
	{van Baaren}, C. and {van Leeuwen}, B.-J. and {van de Stadt}, H. and 
	{Visser}, H. and {Wildeman}, K.~J. and {Wafelbakker}, C.~K. and 
	{Ward}, J.~S. and {Wesselius}, P. and {Wild}, W. and {Wulff}, S. and 
	{Wunsch}, H.-J. and {Tielens}, X. and {Zaal}, P. and {Zirath}, H. and 
	{Zmuidzinas}, J. and {Zwart}, F.},
    title = "{The Herschel-Heterodyne Instrument for the Far-Infrared (HIFI)}",
  journal = {\aap},
 keywords = {instrumentation: spectrographs, methods: observational, infrared: general, submillimeter: general, techniques: spectroscopic},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L6},
    pages = {L6},
      doi = {10.1051/0004-6361/201014698},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L...6D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Demyk1999,
   author = {{Demyk}, K. and {Jones}, A.~P. and {Dartois}, E. and {Cox}, P. and 
	{D'Hendecourt}, L.},
    title = "{The chemical composition of the silicate dust around RAFGL7009S and IRAS 19110+1045}",
  journal = {\aap},
    year = 1999,
    month = sep,
   volume = 349,
    pages = {267-275},
}

@ARTICLE{DeRosa2011,
   author = {{De Rosa}, R.~J. and {Bulger}, J. and {Patience}, J. and {Leland}, B. and 
	{Macintosh}, B. and {Schneider}, A. and {Song}, I. and {Marois}, C. and 
	{Graham}, J.~R. and {Bessell}, M. and {Doyon}, R.},
    title = "{The Volume-limited A-Star (VAST) survey - I. Companions and the unexpected X-ray detection of B6-A7 stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.4363},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: high angular resolution, binaries: general, stars: early-type, stars: imaging, X-rays: stars},
     year = 2011,
    month = jul,
   volume = 415,
    pages = {854-866},
      doi = {10.1111/j.1365-2966.2011.18765.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415..854D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Devillard1999,
   author = {{Devillard}, N.},
    title = "{Infrared Jitter Imaging Data Reduction: Algorithms and Implementation}",
booktitle = {Astronomical Data Analysis Software and Systems VIII},
     year = 1999,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 172,
   editor = {{Mehringer}, D.~M. and {Plante}, R.~L. and {Roberts}, D.~A.},
    pages = {333},
   adsurl = {http://adsabs.harvard.edu/abs/1999ASPC..172..333D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{DeVoe,
   author = {{Devoe}, H.},
    title = "{Optical Properties of Molecular Aggregates. I. Classical Model of Electronic Absorption and Refraction}",
  journal = {The Journal of Chemical Physics},
     year = 1964,
    month = jul,
   volume = 41,
    pages = {393-400},
}

@ARTICLE{Dermott1984,
   author = {{Dermott}, S.~F. and {Nicholson}, P.~D. and {Burns}, J.~A. and 
	{Houck}, J.~R.},
    title = "{Origin of the solar system dust bands discovered by IRAS}",
  journal = {Nature},
      year = 1984,
    month = dec,
   volume = 312,
    pages = {505-509},
}

@ARTICLE{diFolco2004,
   author = {{Di Folco}, E. and {Th{\'e}venin}, F. and {Kervella}, P. and 
	{Domiciano de Souza}, A. and {Coud{\'e} du Foresto}, V. and 
	{S{\'e}gransan}, D. and {Morel}, P.},
    title = "{VLTI near-IR interferometric observations of Vega-like stars. Radius and age of {$\alpha$} PsA, {$\beta$} Leo, {$\beta$} Pic, {$\epsilon$} Eri and {$\tau$} Cet}",
  journal = {\aap},
 keywords = {techniques: interferometric, infrared: stars, stars: fundamental parameters, stars: circumstellar matter, stars: general},
     year = 2004,
    month = nov,
   volume = 426,
    pages = {601-617},
      doi = {10.1051/0004-6361:20047189},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...426..601D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{diFolco2007,
   author = {{Di Folco}, E. and {Absil}, O. and {Augereau}, J.-C. and {M{\'e}rand}, A. and 
	{Coud{\'e} du Foresto}, V. and {Th{\'e}venin}, F. and {Defr{\`e}re}, D. and 
	{Kervella}, P. and {ten Brummelaar}, T.~A. and {McAlister}, H.~A. and 
	{Ridgway}, S.~T. and {Sturmann}, J. and {Sturmann}, L. and {Turner}, N.~H.
	},
    title = "{A near-infrared interferometric survey of debris disk stars. I. Probing the hot dust content around {$\epsilon$} Eridani and {$\tau$} Ceti with CHARA/FLUOR}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0710.1731},
 keywords = {stars: individual: {$\tau$} Cet {$\epsilon$} Eri, stars: fundamental parameters, circumstellar matter, methods: observational, techniques: interferometric},
     year = 2007,
    month = nov,
   volume = 475,
    pages = {243-250},
      doi = {10.1051/0004-6361:20077625},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475..243D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dohnanyi1969,
   author = {{Dohnanyi}, J.~S.},
    title = "{Collisional Model of Asteroids and Their Debris}",
  journal = {Journal of Geophysical Research},
     year = 1969,
    month = may,
   volume = 74,
    pages = {2531--2554},
}

@ARTICLE{Dominik1997,
   author = {{Dominik}, C. and {Tielens}, A.~G.~G.~M.},
    title = "{The Physics of Dust Coagulation and the Structure of Dust Aggregates in Space}",
  journal = {\apj},
 keywords = {STARS: CIRCUMSTELLAR MATTER, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, ISM: CLOUDS, SOLAR SYSTEM: FORMATION},
     year = 1997,
    month = may,
   volume = 480,
    pages = {647},
      doi = {10.1086/303996},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...480..647D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dominik2003,
   author = {{Dominik}, C. and {Decin}, G.},
    title = "{Age Dependence of the Vega Phenomenon: Theory}",
  journal = {\apj},
   eprint = {astro-ph/0308364},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars},
     year = 2003,
    month = nov,
   volume = 598,
    pages = {626-635},
      doi = {10.1086/379169},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598..626D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dorschner1988,
   author = {{Dorschner}, J. and {Friedemann}, C. and {Guertler}, J. and 
	{Henning}, T.},
    title = "{Optical properties of glassy bronzite and the interstellar silicate bands}",
  journal = {\aap},
 keywords = {Infrared Spectra, Interplanetary Dust, Interstellar Matter, Optical Properties, Silicates, Stellar Envelopes, Absorptivity, Amorphous Materials, Glass, Particle Size Distribution, Pyroxenes, Refractivity},
     year = 1988,
    month = jun,
   volume = 198,
    pages = {223-232},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...198..223D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dorschner1995,
  author = {{Dorschner}, J. and {Begemann}, B. and {Henning}, T. and {J{\"a}ger}, C. and 
	{Mutschke}, H.},
  title = "{Steps toward interstellar silicate mineralogy. II. Study of Mg-Fe-silicate glasses of variable composition.}",
  journal = {\aap},
 keywords = {CIRCUMSTELLAR MATTER, DUST, EXTINCTION, INFRARED: INTERSTELLAR: LINES, METHODS: LABORATORY},
     year = 1995,
    month = aug,
   volume = 300,
    pages = {503},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...300..503D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{Doty2004,
   author = {{Doty}, S.~D. and {Sch{\"o}ier}, F.~L. and {van Dishoeck}, E.~F.
	},
    title = "{Physical-chemical modeling of the low-mass protostar IRAS 16293-2422}",
journal={\aap},
   eprint = {arXiv:astro-ph/0402610},
 keywords = {stars: formation, stars: individual: IRAS 16293-2422, ISM: molecules},
     year = 2004,
    month = may,
   volume = 418,
    pages = {1021-1034},
      doi = {10.1051/0004-6361:20034476},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...418.1021D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DraineLee1984,
   author = {{Draine}, B.~T. and {Lee}, H.~M.},
    title = "{Optical properties of interstellar graphite and silicate grains}",
  journal = {\apj},
     year = 1984,
    month = oct,
   volume = 285,
    pages = {89-108},
}

@ARTICLE{Draine1988,
   author = {{Draine}, B.~T.},
    title = "{The discrete-dipole approximation and its application to interstellar graphite grains}",
  journal = {\apj},
   year = 1988,
    month = oct,
   volume = 333,
    pages = {848-872},
}

@Article{DraineGood,
   author = {{Draine}, B.~T. and {Goodman}, J.},
    title = "{Beyond Clausius-Mossotti - Wave propagation on a polarizable point lattice and the discrete dipole approximation}",
   journal = {\apj},
     year = 1993,
    month = mar,
   volume = 405,
    pages = {685-697},
} 

@ARTICLE{DraineLaor1993,
   author = {{Laor}, A. and {Draine}, B.~T.},
    title = "{Spectroscopic constraints on the properties of dust in active galactic nuclei}",
  journal = {\apj},
   year = 1993,
    month = jan,
   volume = 402,
    pages = {441-468},
}

@ARTICLE{DraineMalhotra1993,
 author = {{Draine}, B.~T. and {Malhotra}, S.},
    title = "{On graphite and the 2175 A extinction profile}",
  journal = {\apj},
 keywords = {Astronomical Spectroscopy, Graphite, Interstellar Extinction, Interstellar Matter, Coatings, Electromagnetic Scattering, Grain Size, Shapes, Ultraviolet Spectra},
     year = 1993,
    month = sep,
   volume = 414,
    pages = {632-645},
      doi = {10.1086/173109},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...414..632D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Article{Draine1994,
   author = {{Draine}, B.~T. and {Flatau}, P.~J.},
    title = "{Discrete-dipole approximation for scattering calculations}",
  journal = {Journal of the Optical Society of America A},
     year = 1994,
    month = apr,
   volume = 11,
    pages = {1491-1499},
}

@ARTICLE{Draine1996,
   author = {{Draine}, B.~T. and {Weingartner}, J.~C.},
    title = "{Radiative Torques on Interstellar Grains. I. Superthermal Spin-up}",
  journal = {\apj},
     year = 1996,
    month = oct,
   volume = 470,
    pages = {551-565},
}

@INBOOK{Draine2000,
   author = {{Draine}, B.~T.},
    title = "{The Discrete Dipole Approximation for Light Scattering by Irregular Targets}",
booktitle = {Light Scattering by Nonspherical Particles : Theory, Measurements, and Applications},
     year = 2000,
    month = jan,
   editor = "{Mishchenko, M.~I., Hovenier, J.~W., \& Travis, L.~D.}",
    pages = {131},
}


@ARTICLE{Draine2003a,
   author = {{Draine}, B.~T.},
    title = "{Scattering by Interstellar Dust Grains. I. Optical and Ultraviolet}",
  journal = {\apj},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1017-1025}
}

@ARTICLE{Draine2003b,
   author = {{Draine}, B.~T.},
    title = "{Scattering by Interstellar Dust Grains. II. X-Rays}",
  journal = {\apj},,
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1026-1037},
}

@ARTICLE{Draine2003,
   author = {{Draine}, B.~T.},
    title = "{Interstellar Dust Grains}",
  journal = {Annual Review of Astronomy \& Astrophysics},
     year = 2003,
   volume = 41,
    pages = {241-289},
}

@ARTICLE{Draine2006,
   author = {{Draine}, B.~T.},
    title = "{On the Submillimeter Opacity of Protoplanetary Disks}",
  journal = {\apj},
   eprint = {astro-ph/0507292},
 keywords = {ISM: Dust, Extinction, Stars: Planetary Systems: Protoplanetary Disks, Submillimeter},
     year = 2006,
    month = jan,
   volume = 636,
    pages = {1114-1120},
      doi = {10.1086/498130},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636.1114D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Draine2008,
   author = {{Draine}, B.~T. and {Flatau}, P.~J.},
    title = "{Discrete-dipole approximation for periodic targets: theory and tests}",
  journal = {Journal of the Optical Society of America A},
     year = 2008,
    month = oct,
   volume = 25,
    pages = {2693-2703},
}

@Article{Draine2010,
   author = {{Draine}, B.~T. and {Flatau}, P.~J.},
    title = "{User Guide for the Discrete Dipole Approximation Code DDSCAT 7.1}",
  journal = {ArXiv e-prints},
url={http://arxiv.org/abs/1002.1505v1},
     year = 2010,
    month = feb,
}

@ARTICLE{Draine2012,
   author = {{Draine}, B.~T. and {Flatau}, P.~J.},
    title = "{User Guide for the Discrete Dipole Approximation Code DDSCAT 7.2}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1202.3424},
 primaryClass = "physics.comp-ph",
 keywords = {Physics - Computational Physics, Astrophysics - Galaxy Astrophysics, Condensed Matter - Mesoscale and Nanoscale Physics, Physics - Optics},
     year = 2012,
    month = feb,
}


@ARTICLE{Dullemond2005,
   author = {{Dullemond}, C.~P. and {Dominik}, C.},
    title = "{Dust coagulation in protoplanetary disks: A rapid depletion of small grains}",
  journal = {\aap},
   eprint = {astro-ph/0412117},
 keywords = {accretion, accretion disks, stars: circumstellar matter, stars: formation, stars: pre-main sequence, infrared: stars, ISM: dust, extinction},
     year = 2005,
    month = may,
   volume = 434,
    pages = {971-986},
      doi = {10.1051/0004-6361:20042080},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...434..971D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dullemond2007,
   author = {{Dullemond}, C.~P. and {Hollenbach}, D. and {Kamp}, I. and {D'Alessio}, P.
	},
    title = "{Models of the Structure and Evolution of Protoplanetary Disks}",
  journal = {Protostars and Planets V},
   eprint = {astro-ph/0602619},
     year = 2007,
    pages = {555-572},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..555D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dutrey1996,
   author = {{Dutrey}, A. and {Guilloteau}, S. and {Duvert}, G. and {Prato}, L. and 
	{Simon}, M. and {Schuster}, K. and {Menard}, F.},
    title = "{Dust and gas distribution around T Tauri stars in Taurus-Auriga. I. Interferometric 2.7mm continuum and \^{}13\^{}CO J=1-0 observations}",
  journal = {\aap},
 keywords = {BINARIES: CLOSE, CIRCUMSTELLAR MATTER, STARS: PRE-MAIN SEQUENCE, RADIO-LINES: STARS, RADIO CONTINUUM: STARS},
     year = 1996,
    month = may,
   volume = 309,
    pages = {493-504},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...309..493D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dutrey2014,
   author = {{Dutrey}, A. and {Semenov}, D. and {Chapillon}, E. and {Gorti}, U. and 
	{Guilloteau}, S. and {Hersant}, F. and {Hogerheijde}, M. and 
	{Hughes}, M. and {Meeus}, G. and {Nomura}, H. and {Pi{\'e}tu}, V. and 
	{Qi}, C. and {Wakelam}, V.},
    title = "{Physical and Chemical Structure of Planet-Forming Disks Probed by Millimeter Observations and Modeling}",
  journal = {Protostars and Planets VI},
archivePrefix = "arXiv",
   eprint = {1402.3503},
 primaryClass = "astro-ph.GA",
     year = 2014,
    pages = {317-338},
      doi = {10.2458/azu_uapress_9780816531240-ch014},
   adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..317D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dwek1986,
   author = {{Dwek}, E.},
    title = "{Temperature fluctuations and infrared emission from dust particles in a hot gas}",
  journal = {\apj},
 keywords = {INFRARED SPECTRA, INTERSTELLAR MATTER, ELECTRON ENERGY, GRAIN SIZE, GRAPHITE, PLASMA TEMPERATURE, SILICATES, TEMPERATURE DISTRIBUTION},
     year = 1986,
    month = mar,
   volume = 302,
    pages = {363-370},
      doi = {10.1086/163995},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...302..363D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dyck1971,
   author = {{Dyck}, H.~M. and {Forbes}, F.~F. and {Shawl}, S.~J.},
    title = "{Polarimetry of red and infrared stars at 1 to 4 microns.}",
  journal = {Astronomical Journal},
     year = 1971,
    month = nov,
   volume = 76,
    pages = {901-915},
      doi = {10.1086/111199},
   adsurl = {http://adsabs.harvard.edu/abs/1971AJ.....76..901D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eiroa2013,
   author = {{Eiroa}, C. and {Marshall}, J.~P. and {Mora}, A. and {Montesinos}, B. and 
	{Absil}, O. and {Augereau}, J.~C. and {Bayo}, A. and {Bryden}, G. and 
	{Danchi}, W. and {del Burgo}, C. and {Ertel}, S. and {Fridlund}, M. and 
	{Heras}, A.~M. and {Krivov}, A.~V. and {Launhardt}, R. and {Liseau}, R. and 
	{L{\"o}hne}, T. and {Maldonado}, J. and {Pilbratt}, G.~L. and 
	{Roberge}, A. and {Rodmann}, J. and {Sanz-Forcada}, J. and {Solano}, E. and 
	{Stapelfeldt}, K. and {Th{\'e}bault}, P. and {Wolf}, S. and 
	{Ardila}, D. and {Ar{\'e}valo}, M. and {Beichmann}, C. and {Faramaz}, V. and 
	{Gonz{\'a}lez-Garc{\'{\i}}a}, B.~M. and {Guti{\'e}rrez}, R. and 
	{Lebreton}, J. and {Mart{\'{\i}}nez-Arn{\'a}iz}, R. and {Meeus}, G. and 
	{Montes}, D. and {Olofsson}, G. and {Su}, K.~Y.~L. and {White}, G.~J. and 
	{Barrado}, D. and {Fukagawa}, M. and {Gr{\"u}n}, E. and {Kamp}, I. and 
	{Lorente}, R. and {Morbidelli}, A. and {M{\"u}ller}, S. and 
	{Mutschke}, H. and {Nakagawa}, T. and {Ribas}, I. and {Walker}, H.
	},
    title = "{DUst around NEarby Stars. The survey observational results}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1305.0155},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, planetary systems, infrared: stars},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A11},
    pages = {A11},
      doi = {10.1051/0004-6361/201321050},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..11E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eisloeffel1998,
   author = {{Eisl{\"o}ffel}, J. and {Mundt}, R.},
    title = "{Imaging and Kinematic Studies of Young Stellar Object Jets in Taurus}",
  journal = {The Astronomical Journal},
 keywords = {ISM: JETS AND OUTFLOWS, ISM: KINEMATICS AND DYNAMICS},
     year = 1998,
    month = apr,
   volume = 115,
    pages = {1554-1575},
      doi = {10.1086/300282},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1554E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Elias1978,
   author = {{Elias}, J.~H.},
    title = "{A study of the Taurus dark cloud complex}",
   journal ={\apj},
 keywords = {Early Stars, Infrared Astronomy, Stellar Evolution, Taurus Constellation, H Alpha Line, Interstellar Extinction, Nebulae, Photometry, Spectrophotometry, T Tauri Stars},
     year = 1978,
    month = sep,
   volume = 224,
    pages = {857-872},
      doi = {10.1086/156436},
   adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...224..857E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ertel2011,
   author = {{Ertel}, S. and {Wolf}, S. and {Metchev}, S. and {Schneider}, G. and 
	{Carpenter}, J.~M. and {Meyer}, M.~R. and {Hillenbrand}, L.~A. and 
	{Silverstone}, M.~D.},
    title = "{Multi-wavelength modeling of the spatially resolved debris disk of HD 107146}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.1057},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: HD 107146, techniques: high angular resolution, methods: data analysis, circumstellar matter, infrared: stars},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201015910},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A.132E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ertel2012a,
   author = {{Ertel}, S. and {Wolf}, S. and {Marshall}, J.~P. and {Eiroa}, C. and 
	{Augereau}, J.-C. and {Krivov}, A.~V. and {L{\"o}hne}, T. and 
	{Absil}, O. and {Ardila}, D. and {Ar{\'e}valo}, M. and {Bayo}, A. and 
	{Bryden}, G. and {del Burgo}, C. and {Greaves}, J. and {Kennedy}, G. and 
	{Lebreton}, J. and {Liseau}, R. and {Maldonado}, J. and {Montesinos}, B. and 
	{Mora}, A. and {Pilbratt}, G.~L. and {Sanz-Forcada}, J. and 
	{Stapelfeldt}, K. and {White}, G.~J.},
    title = "{A peculiar class of debris disks from Herschel/DUNES. A steep fall off in the far infrared}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1203.6784},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: HIP 103389, infrared: planetary systems, stars: individual: HIP 107350, infrared: stars, stars: individual: HIP 114948},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A148},
    pages = {A148},
      doi = {10.1051/0004-6361/201118077},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A.148E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ertel2012b,
   author = {{Ertel}, S. and {Wolf}, S. and {Rodmann}, J.},
    title = "{Observing planet-disk interaction in debris disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1206.3154},
 primaryClass = "astro-ph.IM",
 keywords = {techniques: high angular resolution, techniques: interferometric, planets and satellites: detection, planet-disk interactions, infrared: planetary systems, submillimeter: planetary systems},
     year = 2012,
    month = aug,
   volume = 544,
      eid = {A61},
    pages = {A61},
      doi = {10.1051/0004-6361/201219236},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...544A..61E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ertel2011Dok,
   author = {{Ertel}, S.},
    title = "{Modeling the spatial structure of debris disks}",
 journal = {Dissertation},
     year = 2011
}


@ARTICLE{Ertel2014,
   author = {{Ertel}, S. and {Marshall}, J.~P. and {Augereau}, J.-C. and 
	{Krivov}, A.~V. and {L{\"o}hne}, T. and {Eiroa}, C. and {Mora}, A. and 
	{del Burgo}, C. and {Montesinos}, B. and {Bryden}, G. and {Danchi}, W. and 
	{Kirchschlager}, F. and {Liseau}, R. and {Maldonado}, J. and 
	{Pilbratt}, G.~L. and {Sch{\"u}ppler}, C. and {Th{\'e}bault}, P. and 
	{White}, G.~J. and {Wolf}, S.},
    title = "{Potential multi-component structure of the debris disk around HIP 17439 revealed by Herschel/DUNES}",
  journal ={\aap},
archivePrefix = "arXiv",
   eprint = {1312.6385},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, circumstellar matter, stars: individual: HIP 17439},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A114},
    pages = {A114},
      doi = {10.1051/0004-6361/201219945},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A.114E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ertel2014b,
   author = {{Ertel}, S. and {Absil}, O. and {Defr{\`e}re}, D. and {Le Bouquin}, J.-B. and 
	{Augereau}, J.-C. and {Marion}, L. and {Blind}, N. and {Bonsor}, A. and 
	{Bryden}, G. and {Lebreton}, J. and {Milli}, J.},
    title = "{A near-infrared interferometric survey of debris-disk stars. IV. An unbiased sample of 92 southern stars observed in H band with VLTI/PIONIER}",
  journal ={\aap},
archivePrefix = "arXiv",
   eprint = {1409.6143},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, circumstellar matter, planetary systems, zodiacal dust},
     year = 2014,
    month = oct,
   volume = 570,
      eid = {A128},
    pages = {A128},
      doi = {10.1051/0004-6361/201424438},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...570A.128E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ertel2016,
   author = {{Ertel}, S. and {Defr{\`e}re}, D. and {Absil}, O. and {Le Bouquin}, J.-B. and 
	{Augereau}, J.-C. and {Berger}, J.-P. and {Blind}, N. and {Bonsor}, A. and 
	{Lagrange}, A.-M. and {Lebreton}, J. and {Marion}, L. and {Milli}, J. and 
	{Olofsson}, J.},
    title = "{A near-infrared interferometric survey of debris-disc stars. V. PIONIER search for variability}",
  journal = {\aap},
 keywords = {techniques: interferometric, circumstellar matter, planetary systems, zodiacal dust},
     year = 2016,
    month = oct,
   volume = 595,
      eid = {A44},
    pages = {A44},
      doi = {10.1051/0004-6361/201527721},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...595A..44E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Espaillat2014,
   author = {{Espaillat}, C. and {Muzerolle}, J. and {Najita}, J. and {Andrews}, S. and 
	{Zhu}, Z. and {Calvet}, N. and {Kraus}, S. and {Hashimoto}, J. and 
	{Kraus}, A. and {D'Alessio}, P.},
    title = "{An Observational Perspective of Transitional Disks}",
  journal = {Protostars and Planets VI},
archivePrefix = "arXiv",
   eprint = {1402.7103},
 primaryClass = "astro-ph.SR",
     year = 2014,
    pages = {497-520},
      doi = {10.2458/azu_uapress_9780816531240-ch022},
   adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..497E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Fabian2001,
   author = {{Fabian}, D. and {Henning}, T. and {J{\"a}ger}, C. and {Mutschke}, H. and 
	{Dorschner}, J. and {Wehrhan}, O.},
    title = "{Steps toward interstellar silicate mineralogy. VI. Dependence of crystalline olivine IR spectra on iron content and particle shape}",
  journal = {\aap},
 keywords = {STARS: CIRCUMSTELLAR MATTER, STARS: FORMATION, STARS: AGB AND POST-AGB, SOLAR SYSTEM: FORMATION, METHODS: LABORATORY},
     year = 2001,
    month = oct,
   volume = 378,
    pages = {228-238},
      doi = {10.1051/0004-6361:20011196},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...378..228F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Faramaz2017,
   author = {{Faramaz}, V. and {Ertel}, S. and {Booth}, M. and {Cuadra}, J. and 
	{Simmonds}, C.},
    title = "{Inner mean-motion resonances with eccentric planets: a possible origin for exozodiacal dust clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1611.02196},
 primaryClass = "astro-ph.EP",
     year = 2017,
    month = feb,
   volume = 465,
    pages = {2352-2365},
      doi = {10.1093/mnras/stw2846},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.2352F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ferrarotti2006,
   author = {{Ferrarotti}, A.~S. and {Gail}, H.-P.},
    title = "{Composition and quantities of dust produced by AGB-stars and returned to the interstellar medium}",
  journal = {\aap},
 keywords = {circumstellar matter, dust, extinction, stars: mass-loss, stars: winds, outflows, stars: AGB and post-AGB, evolution},
     year = 2006,
    month = feb,
   volume = 447,
    pages = {553-576},
      doi = {10.1051/0004-6361:20041198},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...447..553F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fischer1992Dok,
   author = {{Fischer}, O.},
    title = "{}",
 journal = {Dissertation},
     year = 1992
}

@ARTICLE{Fischer1994,
   author = {{Fischer}, O. and {Henning}, T. and {Yorke}, H.~W.},
    title = "{Simulation of polarization maps. 1: Protostellar envelopes}",
  journal = {\aap},
 keywords = {ASTRONOMICAL MAPS, COMPUTERIZED SIMULATION, LINEAR POLARIZATION, PROTOSTARS, STELLAR ENVELOPES, STELLAR MODELS, HYDRODYNAMICS, INTERSTELLAR MATTER, MONTE CARLO METHOD, PARTICLE SIZE DISTRIBUTION, RADIATIVE TRANSFER},
     year = 1994,
    month = apr,
   volume = 284,
    pages = {187-209},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...284..187F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fischer1995,
   author = {{Fischer}, O. and {Henning}, T.},
    title = "{Polarization maps of protostellar disks.}",
  journal = {Astrophysics and Space Science},
 keywords = {Circumstellar Disks: Young Stars, Circumstellar Disks: Polarization},
     year = 1995,
    month = jan,
   volume = 223,
    pages = {154},
   adsurl = {http://adsabs.harvard.edu/abs/1995Ap%26SS.223..154F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fischer1996,
   author = {{Fischer}, O. and {Henning}, T. and {Yorke}, H.~W.},
    title = "{Simulation of polarization maps. II. The circumstellar environment of pre-main sequence objects.}",
  journal = {\aap},
 keywords = {POLARIZATION, RADIATIVE TRANSFER, CIRCUMSTELLAR MATTER, INFRARED: STARS, STARS: PRE-MAIN SEQUENCE},
     year = 1996,
    month = apr,
   volume = 308,
    pages = {863-885},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...308..863F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Fitzgerald2007,
   author = {{Fitzgerald}, M.~P. and {Kalas}, P.~G. and {Duch{\^e}ne}, G. and 
	{Pinte}, C. and {Graham}, J.~R.},
    title = "{The AU Microscopii Debris Disk: Multiwavelength Imaging and Modeling}",
 journal = {\apj},
     year = 2007,
    month = nov,
   volume = 670,
    pages = {536-556},
}

@ARTICLE{Fixsen2002,
   author = {{Fixsen}, D.~J. and {Dwek}, E.},
    title = "{The Zodiacal Emission Spectrum as Determined by COBE and Its Implications}",
  journal = {\apj},
 keywords = {Infrared: Solar System, Interplanetary Medium},
     year = 2002,
    month = oct,
   volume = 578,
    pages = {1009-1014},
      doi = {10.1086/342658},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...578.1009F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{fliebach2004,
  title={Elektrodynamik: Lehrbuch zur Theoretischen Physik II},
  author={Flie{\ss}bach, T.},
  isbn={9783827415301},
  series={Lehrbuch zur Theoretischen Physik},
  year={2004},
  publisher={Spektrum Akademischer Verlag}
}

@ARTICLE{Flower1996,
   author = {{Flower}, P.~J.},
    title = "{Transformations from Theoretical Hertzsprung-Russell Diagrams to Color-Magnitude Diagrams: Effective Temperatures, B-V Colors, and Bolometric Corrections}",
  journal = {\apj},
 keywords = {STARS: ATMOSPHERES, STARS: EARLY-TYPE, STARS: FUNDAMENTAL PARAMETERS, STARS: LATE-TYPE, STARS: SUPERGIANTS, STARS: HERTZSPRUNG-RUSSELL DIAGRAM},
     year = 1996,
    month = sep,
   volume = 469,
    pages = {355},
      doi = {10.1086/177785},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...469..355F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fuentes2008,
   author = {{Fuentes}, C.~I. and {Holman}, M.~J.},
    title = "{a SUBARU Archival Search for Faint Trans-Neptunian Objects}",
  journal = {The Astronomical Journal},
 keywords = {Kuiper Belt, solar system: formation},
     year = 2008,
    month = jul,
   volume = 136,
    pages = {83-97},
      doi = {10.1088/0004-6256/136/1/83},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136...83F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fuhrmann2008,
   author = {{Fuhrmann}, K.},
    title = "{Nearby stars of the Galactic disc and halo - IV}",
  journal = {\mnras},
 keywords = {stars: fundamental parameters , Galaxy: evolution , Galaxy: formation , Galaxy: stellar content},
     year = 2008,
    month = feb,
   volume = 384,
    pages = {173-224},
      doi = {10.1111/j.1365-2966.2007.12671.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.384..173F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Furlan2006,
   author = {{Furlan}, E. and {Hartmann}, L. and {Calvet}, N. and {D'Alessio}, P. and 
	{Franco-Hern{\'a}ndez}, R. and {Forrest}, W.~J. and {Watson}, D.~M. and 
	{Uchida}, K.~I. and {Sargent}, B. and {Green}, J.~D. and {Keller}, L.~D. and 
	{Herter}, T.~L.},
    title = "{A Survey and Analysis of Spitzer Infrared Spectrograph Spectra of T Tauri Stars in Taurus}",
  journal = {\apjs},
   eprint = {astro-ph/0608038},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Planetary Systems: Protoplanetary Disks, Stars: Pre-Main-Sequence},
     year = 2006,
    month = aug,
   volume = 165,
    pages = {568-605},
      doi = {10.1086/505468},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..165..568F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Furlan2011,
   author = {{Furlan}, E. and {Luhman}, K.~L. and {Espaillat}, C. and {D'Alessio}, P. and 
	{Adame}, L. and {Manoj}, P. and {Kim}, K.~H. and {Watson}, D.~M. and 
	{Forrest}, W.~J. and {McClure}, M.~K. and {Calvet}, N. and {Sargent}, B.~A. and 
	{Green}, J.~D. and {Fischer}, W.~J.},
    title = "{The Spitzer Infrared Spectrograph Survey of T Tauri Stars in Taurus}",
  journal = {\apjs},
 keywords = {circumstellar matter, protoplanetary disks, stars: formation, stars: low-mass, stars: pre-main sequence},
     year = 2011,
    month = jul,
   volume = 195,
      eid = {3},
    pages = {3},
      doi = {10.1088/0067-0049/195/1/3},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..195....3F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaidos2000,
   author = {{Gaidos}, E.~J. and {Henry}, G.~W. and {Henry}, S.~M.},
    title = "{Spectroscopy and Photometry of Nearby Young Solar Analogs}",
  journal = {The Astronomical Journal},
 keywords = {Stars: Planetary Systems, Solar System: Formation, Stars: Evolution, Sun},
     year = 2000,
    month = aug,
   volume = 120,
    pages = {1006-1013},
      doi = {10.1086/301488},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....120.1006G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garnett1904,
   author = {{Maxwell Garnett}, J.~C.},
    title = "{Colours in Metal Glasses and in Metallic Films}",
  journal = {Royal Society of London Philosophical Transactions Series A},
     year = 1904,
   volume = 203,
    pages = {385-420}
}


@ARTICLE{Gaspar2012,
   author = {{G{\'a}sp{\'a}r}, A. and {Psaltis}, D. and {Rieke}, G.~H. and 
	{{\"O}zel}, F.},
    title = "{Modeling Collisional Cascades in Debris Disks: Steep Dust-size Distributions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.0296},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, infrared: stars, methods: numerical, planetary systems},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {74},
    pages = {74},
      doi = {10.1088/0004-637X/754/1/74},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754...74G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaspar2013,
   author = {{G{\'a}sp{\'a}r}, A. and {Rieke}, G.~H. and {Balog}, Z.},
    title = "{The Collisional Evolution of Debris Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1211.1415},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, infrared: stars, methods: numerical, planetary systems},
     year = 2013,
    month = may,
   volume = 768,
      eid = {25},
    pages = {25},
      doi = {10.1088/0004-637X/768/1/25},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768...25G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gaustad1963,
   author = {{Gaustad}, J.~E.},
    title = "{The Opacity of Diffuse Cosmic Matter and the Early Stages of Star Formation.}",
  journal = {\apj},
     year = 1963,
    month = nov,
   volume = 138,
    pages = {1050},
      doi = {10.1086/147705},
   adsurl = {http://adsabs.harvard.edu/abs/1963ApJ...138.1050G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gautier2007,
   author = {{Gautier}, III, T.~N. and {Rieke}, G.~H. and {Stansberry}, J. and 
	{Bryden}, G.~C. and {Stapelfeldt}, K.~R. and {Werner}, M.~W. and 
	{Beichman}, C.~A. and {Chen}, C. and {Su}, K. and {Trilling}, D. and 
	{Patten}, B.~M. and {Roellig}, T.~L.},
    title = "{Far-Infrared Properties of M Dwarfs}",
  journal = {\apj},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {527-536},
}

@ARTICLE{Giese1977,
   author = {{Giese}, R.~H.},
    title = "{Interpretation of the optical properties of interplanetary dust}",
  journal = {Journal of Geophysics Zeitschrift Geophysik},
 keywords = {Helios Project, Optical Properties, Zodiacal Dust, Zodiacal Light, Light Scattering, Micrometeoroids, Mie Scattering, Radial Distribution},
     year = 1977,
   volume = 42,
    pages = {705-716},
   adsurl = {http://adsabs.harvard.edu/abs/1977JGZG...42..705G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Gillett1986,
   author = {{Gillett}, F.~C.},
    title = "{IRAS observations of cool excess around main sequence stars}",
 keywords = {Infrared Astronomy Satellite, Infrared Sources (Astronomy), Main Sequence Stars, Thermal Emission, Astronomical Photometry, Photosphere, Planetary Evolution, Planetary Systems, Radiant Flux Density},
booktitle = {Light on Dark Matter},
     year = 1986,
   series = {Astrophysics and Space Science Library},
   volume = 124,
   editor = {{Israel}, F.~P.},
    pages = {61-69},
      doi = {10.1007/978-94-009-4672-9_10},
   adsurl = {http://adsabs.harvard.edu/abs/1986ASSL..124...61G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gladman2005,
   author = {{Gladman}, B.},
    title = "{The Kuiper Belt and the Solar System's Comet Disk}",
  journal = {Science},
     year = 2005,
    month = jan,
   volume = 307,
    pages = {71-75},
      doi = {10.1126/science.1100553},
   adsurl = {http://adsabs.harvard.edu/abs/2005Sci...307...71G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Glauser2008,
   author = {{Glauser}, A.~M. and {M{\'e}nard}, F. and {Pinte}, C. and {Duch{\^e}ne}, G. and 
	{G{\"u}del}, M. and {Monin}, J.-L. and {Padgett}, D.~L.},
    title = "{Multiwavelength studies of the gas and dust disc of IRAS 04158+2805}",
journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0804.3483},
 keywords = {stars: circumstellar matter, stars: pre-main-sequence, stars: individual: IRAS 04158+2805, stars: formation, stars: planetary systems:, protoplanetary discs},
     year = 2008,
    month = jul,
   volume = 485,
    pages = {531-540},
      doi = {10.1051/0004-6361:20065685},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...485..531G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gledhill1986,
   author = {{Gledhill}, T.~M. and {Warren-Smith}, R.~F. and {Scarrott}, S.~M.
	},
    title = "{Structure of the Haro 6-5 complex}",
  journal = {\mnras},
 keywords = {Emission Spectra, Herbig-Haro Objects, Linear Polarization, Stellar Winds, Optical Emission Spectroscopy, Polarimetry, T Tauri Stars},
     year = 1986,
    month = dec,
   volume = 223,
    pages = {867-875},
   adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.223..867G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goldreich1980,
   author = {{Goldreich}, P. and {Tremaine}, S.},
    title = "{Disk-satellite interactions}",
  journal = {\apj},
 keywords = {Jupiter (Planet), Momentum Transfer, Natural Satellites, Planetary Evolution, Protoplanets, Angular Momentum, Celestial Mechanics, Resonance, Solar System},
     year = 1980,
    month = oct,
   volume = 241,
    pages = {425-441},
      doi = {10.1086/158356},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...241..425G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{Goodman2005,
   author = {{Goodman}, J.~W.},
    title = "{Introduction to Fourier optics}",
booktitle = {Introduction to Fourier optics, 3rd ed., by J.W.~Goodman.~Englewood, CO: Roberts {\amp} Co.~Publishers, 2005},
     year = 2005,
   adsurl = {http://adsabs.harvard.edu/abs/2005ifo..book.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Graefe2011,
   author = {{Gr{\"a}fe}, C. and {Wolf}, S. and {Roccatagliata}, V. and {Sauter}, J. and 
	{Ertel}, S.},
    title = "{Mid-infrared observations of the transitional disks around DH Tauri, DM Tauri, and GM Aurigae}",
journal = {\aap}, 
archivePrefix = "arXiv",
   eprint = {1108.2373},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: pre-main sequence, planets and satellites: formation, protoplanetary disks, planet-disk interactions, stars: general},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A89},
    pages = {A89},
      doi = {10.1051/0004-6361/201015927},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..89G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graefe2013,
   author = {{Gr{\"a}fe}, C. and {Wolf}, S. and {Guilloteau}, S. and {Dutrey}, A. and 
	{Stapelfeldt}, K.~R. and {Pontoppidan}, K.~M. and {Sauter}, J.
	},
    title = "{Vertical settling and radial segregation of large dust grains in the circumstellar disk of the Butterfly Star}",
journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.6499},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary disks, stars: pre-main sequence, stars: individual: IRAS 04302+2247, circumstellar matter, planets and satellites: formation, radiative transfer},
     year = 2013,
    month = may,
   volume = 553,
      eid = {A69},
    pages = {A69},
      doi = {10.1051/0004-6361/201220720},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...553A..69G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graefe2013Dok,
   author = {{Gr{\"a}efe}, Ch.},
    title = "{Beobachtung und Modellierung zirkumstellarer Scheiben}",
 journal = {Dissertation},
     year = 2013,
    month = Okt
}


@ARTICLE{Gray2003,
   author = {{Gray}, R.~O. and {Corbally}, C.~J. and {Garrison}, R.~F. and 
	{McFadden}, M.~T. and {Robinson}, P.~E.},
    title = "{Contributions to the Nearby Stars (NStars) Project: Spectroscopy of Stars Earlier than M0 within 40 Parsecs: The Northern Sample. I.}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/0308182},
 keywords = {Stars: Abundances, Stars: Activity, Stars: Fundamental Parameters, Stars: Statistics, Surveys},
     year = 2003,
    month = oct,
   volume = 126,
    pages = {2048-2059},
      doi = {10.1086/378365},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.2048G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gray2006,
   author = {{Gray}, R.~O. and {Corbally}, C.~J. and {Garrison}, R.~F. and 
	{McFadden}, M.~T. and {Bubar}, E.~J. and {McGahee}, C.~E. and 
	{O'Donoghue}, A.~A. and {Knox}, E.~R.},
    title = "{Contributions to the Nearby Stars (NStars) Project: Spectroscopy of Stars Earlier than M0 within 40 pc-The Southern Sample}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/0603770},
 keywords = {Galaxy: Solar Neighborhood, Stars: Abundances, Stars: Activity, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Statistics},
     year = 2006,
    month = jul,
   volume = 132,
    pages = {161-170},
      doi = {10.1086/504637},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132..161G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greaves2004,
   author = {{Greaves}, J.~S. and {Wyatt}, M.~C. and {Holland}, W.~S. and 
	{Dent}, W.~R.~F.},
    title = "{The debris disc around {$\tau$} Ceti: a massive analogue to the Kuiper Belt}",
  journal = {\mnras},
 keywords = {Kuiper Belt: circumstellar matter: planetary systems: formation: planetary systems: protoplanetary discs: infrared: stars},
     year = 2004,
    month = jul,
   volume = 351,
    pages = {L54-L58},
      doi = {10.1111/j.1365-2966.2004.07957.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.351L..54G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greaves2009,
   author = {{Greaves}, J.~S. and {Wyatt}, M.~C. and {Bryden}, G.},
    title = "{Debris discs around nearby solar analogues}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.3677},
 primaryClass = "astro-ph.GA",
 keywords = {circumstellar matter , planetary systems: formation},
     year = 2009,
    month = aug,
   volume = 397,
    pages = {757-762},
      doi = {10.1111/j.1365-2966.2009.15048.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397..757G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Greenberg1990,
   author = {{Greenberg}, J.~M. and {Hage}, J.~I.},
    title = "{From interstellar dust to comets - A unification of observational constraints}",
  journal = {\apj},
     year = 1990,
    month = sep,
   volume = 361,
    pages = {260-274},
}

@ARTICLE{Griffin2010,
   author = {{Griffin}, M.~J. and {Abergel}, A. and {Abreu}, A. and {Ade}, P.~A.~R. and 
	{Andr{\'e}}, P. and {Augueres}, J.-L. and {Babbedge}, T. and 
	{Bae}, Y. and {Baillie}, T. and {Baluteau}, J.-P. and {Barlow}, M.~J. and 
	{Bendo}, G. and {Benielli}, D. and {Bock}, J.~J. and {Bonhomme}, P. and 
	{Brisbin}, D. and {Brockley-Blatt}, C. and {Caldwell}, M. and 
	{Cara}, C. and {Castro-Rodriguez}, N. and {Cerulli}, R. and 
	{Chanial}, P. and {Chen}, S. and {Clark}, E. and {Clements}, D.~L. and 
	{Clerc}, L. and {Coker}, J. and {Communal}, D. and {Conversi}, L. and 
	{Cox}, P. and {Crumb}, D. and {Cunningham}, C. and {Daly}, F. and 
	{Davis}, G.~R. and {de Antoni}, P. and {Delderfield}, J. and 
	{Devin}, N. and {di Giorgio}, A. and {Didschuns}, I. and {Dohlen}, K. and 
	{Donati}, M. and {Dowell}, A. and {Dowell}, C.~D. and {Duband}, L. and 
	{Dumaye}, L. and {Emery}, R.~J. and {Ferlet}, M. and {Ferrand}, D. and 
	{Fontignie}, J. and {Fox}, M. and {Franceschini}, A. and {Frerking}, M. and 
	{Fulton}, T. and {Garcia}, J. and {Gastaud}, R. and {Gear}, W.~K. and 
	{Glenn}, J. and {Goizel}, A. and {Griffin}, D.~K. and {Grundy}, T. and 
	{Guest}, S. and {Guillemet}, L. and {Hargrave}, P.~C. and {Harwit}, M. and 
	{Hastings}, P. and {Hatziminaoglou}, E. and {Herman}, M. and 
	{Hinde}, B. and {Hristov}, V. and {Huang}, M. and {Imhof}, P. and 
	{Isaak}, K.~J. and {Israelsson}, U. and {Ivison}, R.~J. and 
	{Jennings}, D. and {Kiernan}, B. and {King}, K.~J. and {Lange}, A.~E. and 
	{Latter}, W. and {Laurent}, G. and {Laurent}, P. and {Leeks}, S.~J. and 
	{Lellouch}, E. and {Levenson}, L. and {Li}, B. and {Li}, J. and 
	{Lilienthal}, J. and {Lim}, T. and {Liu}, S.~J. and {Lu}, N. and 
	{Madden}, S. and {Mainetti}, G. and {Marliani}, P. and {McKay}, D. and 
	{Mercier}, K. and {Molinari}, S. and {Morris}, H. and {Moseley}, H. and 
	{Mulder}, J. and {Mur}, M. and {Naylor}, D.~A. and {Nguyen}, H. and 
	{O'Halloran}, B. and {Oliver}, S. and {Olofsson}, G. and {Olofsson}, H.-G. and 
	{Orfei}, R. and {Page}, M.~J. and {Pain}, I. and {Panuzzo}, P. and 
	{Papageorgiou}, A. and {Parks}, G. and {Parr-Burman}, P. and 
	{Pearce}, A. and {Pearson}, C. and {P{\'e}rez-Fournon}, I. and 
	{Pinsard}, F. and {Pisano}, G. and {Podosek}, J. and {Pohlen}, M. and 
	{Polehampton}, E.~T. and {Pouliquen}, D. and {Rigopoulou}, D. and 
	{Rizzo}, D. and {Roseboom}, I.~G. and {Roussel}, H. and {Rowan-Robinson}, M. and 
	{Rownd}, B. and {Saraceno}, P. and {Sauvage}, M. and {Savage}, R. and 
	{Savini}, G. and {Sawyer}, E. and {Scharmberg}, C. and {Schmitt}, D. and 
	{Schneider}, N. and {Schulz}, B. and {Schwartz}, A. and {Shafer}, R. and 
	{Shupe}, D.~L. and {Sibthorpe}, B. and {Sidher}, S. and {Smith}, A. and 
	{Smith}, A.~J. and {Smith}, D. and {Spencer}, L. and {Stobie}, B. and 
	{Sudiwala}, R. and {Sukhatme}, K. and {Surace}, C. and {Stevens}, J.~A. and 
	{Swinyard}, B.~M. and {Trichas}, M. and {Tourette}, T. and {Triou}, H. and 
	{Tseng}, S. and {Tucker}, C. and {Turner}, A. and {Vaccari}, M. and 
	{Valtchanov}, I. and {Vigroux}, L. and {Virique}, E. and {Voellmer}, G. and 
	{Walker}, H. and {Ward}, R. and {Waskett}, T. and {Weilert}, M. and 
	{Wesson}, R. and {White}, G.~J. and {Whitehouse}, N. and {Wilson}, C.~D. and 
	{Winter}, B. and {Woodcraft}, A.~L. and {Wright}, G.~S. and 
	{Xu}, C.~K. and {Zavagno}, A. and {Zemcov}, M. and {Zhang}, L. and 
	{Zonca}, E.},
    title = "{The Herschel-SPIRE instrument and its in-flight performance}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.5123},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: photometers, instrumentation: spectrographs, space vehicles: instruments, submillimeter: general},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L3},
    pages = {L3},
      doi = {10.1051/0004-6361/201014519},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L...3G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Grun99,
   author = {{Gr{\"u}n}, E.},
    title = "{Interplanetary Dust and the Zodiacal Cloud}",
journal={Enceclopedia of the Solar System},
pages = {673-696},
     year = 1999
}

@BOOK{Grun2001,
   author = {{Gr{\"u}n}, E.  and Gustafson, B.A.S. and Dermott, S. and Fechtig, H. (Eds.)},
    title = "{Interplanetary Dust}",
booktitle = {},
     year = 2001,
series ="{Astronomy \& Astrophysics Library}",
   publisher = "{Springer}",
    pages = {804},
}

@ARTICLE{Guilloteau2011,
   author = {{Guilloteau}, S. and {Dutrey}, A. and {Pi{\'e}tu}, V. and {Boehler}, Y.
	},
    title = "{A dual-frequency sub-arcsecond study of proto-planetary disks at mm wavelengths: first evidence for radial variations of the dust properties}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.1296},
 primaryClass = "astro-ph.GA",
 keywords = {protoplanetary disks, stars: formation, planetary systems, dust, extinction},
     year = 2011,
    month = may,
   volume = 529,
      eid = {A105},
    pages = {A105},
      doi = {10.1051/0004-6361/201015209},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A.105G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gutkowicz2004,
   author = {{Gutkowicz-Krusin}, D. and {Draine}, B.~T.},
    title = "{Propagation of Electromagnetic Waves on a Rectangular Lattice of Polarizable Points}",
  journal = {ArXiv Astrophysics e-prints},
   eprint = {astro-ph/0403082},
 keywords = {Astrophysics},
     year = 2004,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2004astro.ph..3082G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Habing2001,
   author = {{Habing}, H.~J. and {Dominik}, C. and {Jourdain de Muizon}, M. and 
	{Laureijs}, R.~J. and {Kessler}, M.~F. and {Leech}, K. and {Metcalfe}, L. and 
	{Salama}, A. and {Siebenmorgen}, R. and {Trams}, N. and {Bouchet}, P.
	},
    title = "{Incidence and survival of remnant disks around main-sequence stars}",
 journal = {\aap},
   eprint = {astro-ph/0011137},
 keywords = {STARS: PLANETARY SYSTEMS, INFRARED: STARS},
     year = 2001,
    month = jan,
   volume = 365,
    pages = {545-561},
      doi = {10.1051/0004-6361:20000075},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365..545H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hage1990,
   author = {{Hage}, J.~I. and {Greenberg}, J.~M.},
    title = "{A model for the optical properties of porous grains}",
  journal = {\apj},
     year = 1990,
    month = sep,
   volume = 361,
    pages = {251-259}
}

@ARTICLE{Hahn,
   author = {{Hahn}, J.~M.},
    title = "{Diagnosing Circumstellar Debris Disks}",
  journal = {\apj},
     year = 2010,
    month = aug,
   volume = 719,
    pages = {1699--1714},
}

@ARTICLE{Hahn2002,
   author = {{Hahn}, J.~M. and {Zook}, H.~A. and {Cooper}, B. and {Sunkara}, B.
	},
    title = "{Clementine Observations of the Zodiacal Light and the Dust Content of the Inner Solar System}",
  journal = {Icarus},
   eprint = {astro-ph/0204111},
     year = 2002,
    month = aug,
   volume = 158,
    pages = {360-378},
      doi = {10.1006/icar.2002.6881},
   adsurl = {http://adsabs.harvard.edu/abs/2002Icar..158..360H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Haisch2001,
   author = {{Haisch}, Jr., K.~E. and {Lada}, E.~A. and {Lada}, C.~J.},
    title = "{Disk Frequencies and Lifetimes in Young Clusters}",
  journal = {\apj},
   eprint = {astro-ph/0104347},
 keywords = {Infrared: Stars, Galaxy: Open Clusters and Associations: General, Stars: Planetary Systems: Protoplanetary Disks, Stars: Formation},
     year = 2001,
    month = jun,
   volume = 553,
    pages = {L153-L156},
      doi = {10.1086/320685},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553L.153H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Haracz1984,
   author = {{Haracz}, R.~D. and {Cohen}, L.~D. and {Cohen}, A.},
    title = "{Perturbation theory for scattering from dielectric spheroids and short cylinders}",
  journal = {Applied Optics},
 keywords = {Circular Cylinders, Dielectrics, Electromagnetic Scattering, Perturbation Theory, Scattering Amplitude, Spheroids, Aspect Ratio, Electric Fields, Maxwell Equation, Polarization Characteristics, Refractivity},
     year = 1984,
    month = feb,
   volume = 23,
    pages = {436-441},
      doi = {10.1364/AO.23.000436},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApOpt..23..436H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haracz1985,
   author = {{Haracz}, R.~D. and {Cohen}, L.~D. and {Cohen}, A.},
    title = "{Scattering of linearly polarized light from randomly oriented cylinders and spheroids}",
  journal = {Journal of Applied Physics},
 keywords = {Aerosols, Atmospheric Optics, Light Scattering, Polarized Light, Clouds, Cylindrical Bodies, Linear Polarization, Perturbation Theory, Spheroids},
     year = 1985,
    month = nov,
   volume = 58,
    pages = {3322-3327},
      doi = {10.1063/1.335792},
   adsurl = {http://adsabs.harvard.edu/abs/1985JAP....58.3322H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hartigan2003,
   author = {{Hartigan}, P. and {Kenyon}, S.~J.},
    title = "{A Spectroscopic Survey of Subarcsecond Binaries in the Taurus-Auriga Dark Cloud with the Hubble Space Telescope}",
  journal = {\apj},
   eprint = {astro-ph/0209608},
 keywords = {Stars: Binaries: General, Stars: Binaries: Visual, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2003,
    month = jan,
   volume = 583,
    pages = {334-357},
      doi = {10.1086/345293},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...583..334H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hartmann1998,
   author = {{Hartmann}, L. and {Calvet}, N. and {Gullbring}, E. and {D'Alessio}, P.
	},
    title = "{Accretion and the Evolution of T Tauri Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE, Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 1998,
    month = mar,
   volume = 495,
    pages = {385-400},
      doi = {10.1086/305277},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...495..385H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Harwit63,
   author = {{Harwit}, M.},
    title = "{Origins of the Zodiacal Dust Cloud}",
  journal = {Journal of Geophysical Research},
     year = 1963,
    month = apr,
   volume = 68,
    pages = {2171-2180},
}


@ARTICLE{Hauck1998,
   author = {{Hauck}, B. and {Mermilliod}, M.},
    title = "{Uvbybeta photoelectric photometric catalogue}",
  journal = {\aaps},
 keywords = {STARS: GENERAL, STARS: FUNDAMENTAL PARAMETERS, CATALOGUE, TECHNIQUES: PHOTOMETRIC},
     year = 1998,
    month = may,
   volume = 129,
    pages = {431-433},
      doi = {10.1051/aas:1998195},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..129..431H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Henning1993,
   author = {{Henning}, T. and {Stognienko}, R.},
    title = "{Porous grains and polarization of light: The silicate features}",
 journal = {\aap},
 keywords = {COSMIC DUST, GRANULAR MATERIALS, INTERSTELLAR EXTINCTION, POLARIZED LIGHT, POROUS MATERIALS, SILICATES, STELLAR ENVELOPES, ABSORPTIVITY, ASTRONOMICAL POLARIMETRY, CHEMICAL COMPOSITION, DISCRETE FUNCTIONS},
     year = 1993,
    month = dec,
   volume = 280,
    pages = {609-616},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...280..609H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HenryDraper1995,
   author = {{Nesterov}, V.~V. and {Kuzmin}, A.~V. and {Ashimbaeva}, N.~T. and 
	{Volchkov}, A.~A. and {R{\"o}ser}, S. and {Bastian}, U.},
    title = "{The Henry Draper Extension Charts: A catalogue of accurate positions, proper motions, magnitudes and spectral types of 86933 stars}",
  journal = {\aaps},
     year = 1995,
    month = apr,
   volume = 110,
    pages = {367-370},
}

@ARTICLE{Hildebrand1983,
   author = {{Hildebrand}, R.~H.},
    title = "{The Determination of Cloud Masses and Dust Characteristics from Submillimetre Thermal Emission}",
  journal = {Quarterly Journal of the Royal Astronomical Society},
     year = 1983,
    month = sep,
   volume = 24,
    pages = {267},
   adsurl = {http://adsabs.harvard.edu/abs/1983QJRAS..24..267H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hildebrand1995,
   author = {{Hildebrand}, R.~H. and {Dragovan}, M.},
    title = "{The Shapes and Alignment Properties of Interstellar Dust Grains}",
  journal = {\apj},
 keywords = {INFRARED: ISM: CONTINUUM, ISM: DUST, EXTINCTION, POLARIZATION},
     year = 1995,
    month = sep,
   volume = 450,
    pages = {663},
      doi = {10.1086/176173},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...450..663H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hillenbrand2008,
   author = {{Hillenbrand}, L.~A. and {Carpenter}, J.~M. and {Kim}, J.~S. and 
	{Meyer}, M.~R. and {Backman}, D.~E. and {Moro-Mart{\'{\i}}n}, A. and 
	{Hollenbach}, D.~J. and {Hines}, D.~C. and {Pascucci}, I. and 
	{Bouwman}, J.},
    title = "{The Complete Census of 70 {$\mu$}m-bright Debris Disks within ``the Formation and Evolution of Planetary Systems'' Spitzer Legacy Survey of Sun-like Stars}",
  journal ={\apj},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {630-656},
}


@BOOK{Hiltner1962,
   author = {{Hiltner}, W.~A.},
    title = "{Astronomical techniques.}",
 keywords = {ASTRONOMICAL INSTRUMENTS},
booktitle = {Chicago, University Press [1962]},
     year = 1962,
   adsurl = {http://adsabs.harvard.edu/abs/1962aste.book.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hioki2011,
   author = {{Hioki}, T. and {Itoh}, Y. and {Oasa}, Y. and {Fukagawa}, M. and 
	{Hayashi}, M.},
    title = "{High-Resolution Optical and Near-Infrared Images of the FS Tauri Circumbinary Disk}",
  journal = {Publications of the Astronomical Society of Japan},
archivePrefix = "arXiv",
   eprint = {1103.0155},
 primaryClass = "astro-ph.SR",
 keywords = {star: individual (FS Taurus), star: pre-main sequence, techniques: high angular resolution},
     year = 2011,
    month = jun,
   volume = 63,
    pages = {543-},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASJ...63..543H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hogg2010,
   author = {{Hogg}, D.~W. and {Bovy}, J. and {Lang}, D.},
    title = "{Data analysis recipes: Fitting a model to data}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1008.4686},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Data Analysis, Statistics and Probability},
     year = 2010,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1008.4686H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hollenbach1994,
   author = {{Hollenbach}, D. and {Johnstone}, D. and {Lizano}, S. and {Shu}, F.
	},
    title = "{Photoevaporation of disks around massive stars and application to ultracompact H II regions}",
  journal = {\apj},
 keywords = {Astronomical Models, Deposition, Disk Galaxies, Evaporation, Galactic Evolution, H Ii Regions, Massive Stars, Photons, Stellar Winds, Mass Flow, Numerical Analysis, Photoionization, Radiative Transfer},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {654-669},
      doi = {10.1086/174276},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428..654H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Holmberg2009,
   author = {{Holmberg}, J. and {Nordstr{\"o}m}, B. and {Andersen}, J.},
    title = "{The Geneva-Copenhagen survey of the solar neighbourhood. III. Improved distances, ages, and kinematics}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0811.3982},
 keywords = {solar neighborhood, Galaxy: disk, Galaxy: stellar, content, Galaxy: kinematics and dynamics, Galaxy: evolution, stars: fundamental parameters},
     year = 2009,
    month = jul,
   volume = 501,
    pages = {941-947},
      doi = {10.1051/0004-6361/200811191},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501..941H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Holweger2001,
   author = {{Holweger}, H.},
    title = "{Photospheric abundances: Problems, updates, implications}",
booktitle = {Joint SOHO/ACE workshop ''Solar and Galactic Composition''},
     year = 2001,
   series = {American Institute of Physics Conference Series},
   volume = 598,
   editor = "{R.~F.~Wimmer-Schweingruber}",
    month = nov,
    pages = {23-30},
}


@ARTICLE{Hony2002,
   author = {{Hony}, S. and {Waters}, L.~B.~F.~M. and {Tielens}, A.~G.~G.~M.
	},
    title = "{The carrier of the ``30'' mu m emission feature in evolved stars. A simple model using magnesium sulfide}",
 journal = {\aap},
   eprint = {astro-ph/0204330},
 keywords = {stars: AGB and post-AGB, stars: carbon, circumstellar matter, stars: mass-loss, planetary nebulae: general, infrared: stars},
     year = 2002,
    month = aug,
   volume = 390,
    pages = {533-553},
      doi = {10.1051/0004-6361:20020603},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...390..533H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Hulst57,
   author = {{van de Hulst}, H.~C.},
    title = "{Light Scattering by Small Particles}",
booktitle = {Light Scattering by Small Particles, New York: John Wiley {\&} Sons, 1957},
     year = 1957,
   editor = "{van de Hulst, H.~C.}",
}

@ARTICLE{Isella2007,
   author = {{Isella}, A. and {Testi}, L. and {Natta}, A. and {Neri}, R. and 
	{Wilner}, D. and {Qi}, C.},
    title = "{Millimeter imaging of HD 163296: probing the disk structure and kinematics}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.0616},
 keywords = {accretion, accretion disks, techniques: interferometric, stars: planetary systems: protoplanetary disks, stars: circumstellar matter},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {213-222},
      doi = {10.1051/0004-6361:20077385},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..213I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ishihara2010,
   author = {{Ishihara}, D. and {Onaka}, T. and {Kataza}, H. and {Salama}, A. and 
	{Alfageme}, C. and {Cassatella}, A. and {Cox}, N. and {Garc{\'{\i}}a-Lario}, P. and 
	{Stephenson}, C. and {Cohen}, M. and {Fujishiro}, N. and {Fujiwara}, H. and 
	{Hasegawa}, S. and {Ita}, Y. and {Kim}, W. and {Matsuhara}, H. and 
	{Murakami}, H. and {M{\"u}ller}, T.~G. and {Nakagawa}, T. and 
	{Ohyama}, Y. and {Oyabu}, S. and {Pyo}, J. and {Sakon}, I. and 
	{Shibai}, H. and {Takita}, S. and {Tanab{\'e}}, T. and {Uemizu}, K. and 
	{Ueno}, M. and {Usui}, F. and {Wada}, T. and {Watarai}, H. and 
	{Yamamura}, I. and {Yamauchi}, C.},
    title = "{The AKARI/IRC mid-infrared all-sky survey}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.0270},
 primaryClass = "astro-ph.IM",
 keywords = {infrared: general, techniques: image processing, surveys},
     year = 2010,
    month = may,
   volume = 514,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/200913811},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...514A...1I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Jackson,
title={"Classical Electromagnetism"},
author={J.D. Jackson},
editor={Wiley, New York},
year={1975},
}

@ARTICLE{Jackson2014,
   author = {{Jackson}, A.~P. and {Wyatt}, M.~C. and {Bonsor}, A. and {Veras}, D.
	},
    title = "{Debris froms giant impacts between planetary embryos at large orbital radii}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1403.1888},
 primaryClass = "astro-ph.EP",
 keywords = {celestial mechanics, planets and satellites: detection, planets and satellites: formation, planet-disc interactions, circumstellar matter},
     year = 2014,
    month = jun,
   volume = 440,
    pages = {3757-3777},
      doi = {10.1093/mnras/stu476},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.440.3757J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jager1998,
   author = {{J{\"a}ger}, C. and {Mutschke}, H. and {Henning}, T.},
    title = "{Optical properties of carbonaceous dust analogues}",
  journal = {\aap},
 keywords = {CIRCUMSTELLAR MATTER, DUST, EXTINCTION, INFRARED: ISM: LINES AND BANDS},
     year = 1998,
    month = apr,
   volume = 332,
    pages = {291-299},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...332..291J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Johnson1996,
   author = {{Johnson}, B.~R.},
    title = "{Light scattering by a multilayer sphere}",
  journal = {Applied Optics},
     year = 1996,
    month = jun,
   volume = 35,
    pages = {3286--3296},
}

@ARTICLE{Kalas2005,
   author = {{Kalas}, P. and {Graham}, J.~R. and {Clampin}, M.},
    title = "{A planetary system as the origin of structure in Fomalhaut's dust belt}",
  journal = {Nature},
   eprint = {astro-ph/0506574},
     year = 2005,
    month = jun,
   volume = 435,
    pages = {1067-1070},
      doi = {10.1038/nature03601},
   adsurl = {http://adsabs.harvard.edu/abs/2005Natur.435.1067K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalas2008,
   author = {{Kalas}, P. and {Graham}, J.~R. and {Chiang}, E. and {Fitzgerald}, M.~P. and 
	{Clampin}, M. and {Kite}, E.~S. and {Stapelfeldt}, K. and {Marois}, C. and 
	{Krist}, J.},
    title = "{Optical Images of an Exosolar Planet 25 Light-Years from Earth}",
  journal = {Science},
     year = 2008,
    month = nov,
   volume = 322,
    pages = {1345--1348}
}

@ARTICLE{Kataoka2013a,
   author = {{Kataoka}, A. and {Tanaka}, H. and {Okuzumi}, S. and {Wada}, K.
	},
    title = "{Static compression of porous dust aggregates}",
 journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.3351},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, methods: numerical, methods: analytical, protoplanetary disks},
     year = 2013,
    month = jun,
   volume = 554,
      eid = {A4},
    pages = {A4},
      doi = {10.1051/0004-6361/201321325},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...554A...4K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kataoka2013b,
   author = {{Kataoka}, A. and {Tanaka}, H. and {Okuzumi}, S. and {Wada}, K.
	},
    title = "{Fluffy dust forms icy planetesimals by static compression}",
 journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.7984},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, methods: analytical, protoplanetary disks},
     year = 2013,
    month = sep,
   volume = 557,
      eid = {L4},
    pages = {L4},
      doi = {10.1051/0004-6361/201322151},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...557L...4K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kataoka2014,
   author = {{Kataoka}, A. and {Okuzumi}, S. and {Tanaka}, H. and {Nomura}, H.
	},
    title = "{Opacity of fluffy dust aggregates}",
 journal = {\aap}, 
archivePrefix = "arXiv",
   eprint = {1312.1459},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, protoplanetary disks},
     year = 2014,
    month = aug,
   volume = 568,
      eid = {A42},
    pages = {A42},
      doi = {10.1051/0004-6361/201323199},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...568A..42K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kattawar,
   author = {{Kattawar}, G.~W. and {Eisner}, M.},
    title = "{Radiation from a homogeneous isothermal sphere.}",
  journal = {Applied Optics},
     year = 1970,
   volume = 9,
    pages = {2685-2690},
}

@ARTICLE{Keenan1983,
   author = {{Keenan}, P.~C.},
    title = "{Revised MK Spectral Standard Stars Later than G0}",
  journal = {Bulletin d'Information du Centre de Donnees Stellaires},
     year = 1983,
    month = mar,
   volume = 24,
    pages = {19},
   adsurl = {http://adsabs.harvard.edu/abs/1983BICDS..24...19K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennedy2012a,
   author = {{Kennedy}, G.~M. and {Wyatt}, M.~C. and {Sibthorpe}, B. and 
	{Duch{\^e}ne}, G. and {Kalas}, P. and {Matthews}, B.~C. and 
	{Greaves}, J.~S. and {Su}, K.~Y.~L. and {Fitzgerald}, M.~P.},
    title = "{99 Herculis: host to a circumbinary polar-ring debris disc}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.1911},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, stars: individual: 99 Herculis},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {2264-2276},
      doi = {10.1111/j.1365-2966.2012.20448.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2264K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennedy2012b,
   author = {{Kennedy}, G.~M. and {Wyatt}, M.~C. and {Sibthorpe}, B. and 
	{Phillips}, N.~M. and {Matthews}, B.~C. and {Greaves}, J.~S.
	},
    title = "{Coplanar circumbinary debris discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.1759},
 primaryClass = "astro-ph.EP",
 keywords = {binaries: general, circumstellar matter, stars: formation, stars: individual: {$\beta$} Trianguli, stars: individual: {$\alpha$} Coronae Borealis, stars: individual: 99 Herculis, HD 98800},
     year = 2012,
    month = nov,
   volume = 426,
    pages = {2115-2128},
      doi = {10.1111/j.1365-2966.2012.21865.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.2115K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennedy2013,
   author = {{Kennedy}, G.~M. and {Wyatt}, M.~C.},
    title = "{The bright end of the exo-Zodi luminosity function: disc evolution and implications for exo-Earth detectability}",
  journal = {\mnras},
 keywords = {circumstellar matter, stars: individual: HD 19257, stars: individual: HD 23586, stars: individual: HD 94893, stars: individual: HD 154593, stars: individual: HD 194931},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {2334-2356},
      doi = {10.1093/mnras/stt900},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.2334K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Kenyon2004,
   author = {{Kenyon}, S.~J. and {Bromley}, B.~C.},
    title = "{Collisional Cascades in Planetesimal Disks. II. Embedded Planets}",
  journal = {The Astronomical Journal},
     year = 2004,
    month = jan,
   volume = 127,
    pages = {513--530}
}

@ARTICLE{Kenyon1987,
   author = {{Kenyon}, S.~J. and {Hartmann}, L.},
    title = "{Spectral energy distributions of T Tauri stars - Disk flaring and limits on accretion}",
  journal = {\apj},
 keywords = {ASTRONOMICAL PHOTOGRAPHY, ENERGY DISTRIBUTION, STELLAR MASS ACCRETION, STELLAR SPECTRA, T TAURI STARS, ABSORPTION SPECTRA, EMISSION SPECTRA, INFRARED SPECTRA, STELLAR FLARES, STELLAR MODELS, STELLAR RADIATION},
     year = 1987,
    month = dec,
   volume = 323,
    pages = {714-733},
      doi = {10.1086/165866},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...323..714K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kimura1997,
   author = {{Kimura}, H. and {Ishimoto}, H. and {Mukai}, T.},
    title = "{A study on solar dust ring formation based on fractal dust models}",
 journal = {\aap},
    year = 1997,
    month = april,
   volume = 326,
    pages = {263-270},
}

@ARTICLE{Kimura1998,
   author = {{Kimura}, H. and {Mann}, I.},
    title = "{Brightness of the solar F-corona}",
  journal = {Earth, Planets, and Space},
     year = 1998,
    month = jun,
   volume = 50,
    pages = {493-499},
      doi = {10.1186/BF03352140},
   adsurl = {http://adsabs.harvard.edu/abs/1998EP%26S...50..493K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kirchschlager2011,
   author = {{Kirchschlager}, F.},
    title = "{Staubk{\"o}rner in Debris-Scheiben}",
 journal = {Diplomarbeit},
     year = 2011,
    month = Okt
}

@ARTICLE{Kirchschlager2013,
   author = {{Kirchschlager}, F. and {Wolf}, S.},
    title = "{Porous dust grains in debris disks}",
 journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.5275},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, protoplanetary disks, infrared: stars, interplanetary medium, scattering},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201220486},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A..54K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kirchschlager2014,
   author = {{Kirchschlager}, F. and {Wolf}, S.},
    title = "{Effect of dust grain porosity on the appearance of protoplanetary disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1407.6575},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary disks, stars: pre-main sequence, circumstellar matter, planets and satellites: formation, radiative transfer},
     year = 2014,
    month = aug,
   volume = 568,
      eid = {A103},
    pages = {A103},
      doi = {10.1051/0004-6361/201323176},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...568A.103K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirchschlager2016,
   author = {{Kirchschlager}, F. and {Wolf}, S. and {Madlener}, D.},
    title = "{The circumstellar disc of FS Tau B - a self-consistent model based on observations in the mid-infrared with NACO}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.05449},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, planets and satellites: formation, protoplanetary discs, circumstellar matter, stars: individual: FS Tau B, stars: pre-main sequence},
     year = 2016,
    month = oct,
   volume = 462,
    pages = {858-866},
      doi = {10.1093/mnras/stw1692},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.462..858K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Kirkpatrick1983,
   author = {{Kirkpatrick}, S. and {Gelatt}, C.~D. and {Vecchi}, M.~P.},
    title = "{Optimization by Simulated Annealing}",
  journal = {Science},
     year = 1983,
    month = may,
   volume = 220,
    pages = {671-680},
      doi = {10.1126/science.220.4598.671},
   adsurl = {http://adsabs.harvard.edu/abs/1983Sci...220..671K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kitamura2002,
   author = {{Kitamura}, Y. and {Momose}, M. and {Yokogawa}, S. and {Kawabe}, R. and 
	{Tamura}, M. and {Ida}, S.},
    title = "{Investigation of the Physical Properties of Protoplanetary Disks around T Tauri Stars by a 1 Arcsecond Imaging Survey: Evolution and Diversity of the Disks in Their Accretion Stage}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems: Formation, Radio Lines: Stars, Stars: Pre-Main-Sequence},
     year = 2002,
    month = dec,
   volume = 581,
    pages = {357-380},
      doi = {10.1086/344223},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...581..357K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Kittel2005,
  title={Einführung in die Festkörperphysik},
  author={Kittel, C.},
  isbn={9783486577235},
  year={2005},
  publisher={Oldenbourg}
}

@ARTICLE{Kobayashi2009,
   author = {{Kobayashi}, H. and {Watanabe}, S.-i. and {Kimura}, H. and {Yamamoto}, T.
	},
    title = "{Dust ring formation due to sublimation of dust grains drifting radially inward by the Poynting-Robertson drag: An analytical model}",
  journal = {Icarus},
     year = 2009,
    month = may,
   volume = 201,
    pages = {395-405},
      doi = {10.1016/j.icarus.2009.01.002},
   adsurl = {http://adsabs.harvard.edu/abs/2009Icar..201..395K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kobayashi2011,
   author = {{Kobayashi}, H. and {Kimura}, H. and {Watanabe}, S.-i. and {Yamamoto}, T. and 
	{M{\"u}ller}, S.},
    title = "{Sublimation temperature of circumstellar dust particles and its importance for dust ring formation}",
  journal = {Earth, Planets, and Space},
archivePrefix = "arXiv",
   eprint = {1104.5627},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = oct,
   volume = 63,
    pages = {1067-1075},
      doi = {10.5047/eps.2011.03.012},
   adsurl = {http://adsabs.harvard.edu/abs/2011EP%26S...63.1067K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koehler02,
   author = {{K{\"o}hler}, M. and {Mann}, I.},
    title = "{Model calculations of dynamical forces and effects on dust in circumstellar debris disks}", 
 journal = {Proceedings of Asteroids, Comets, Meteors - ACM 2002.},
     year = 2002,
   volume = 500,
    month = nov,
    pages = {771-774},
}

@ARTICLE{Koehler04,
   author = {{K{\"o}hler}, M. and {Mann}, I.},
    title = "{Light-scattering models applied to circumstellar dust properties}",
  journal = {Journal of Quantitative Spectroscopy {\&} Radiative Transfer},
     year = 2004,
   volume = 89,
    pages = {453-460},
}

@ARTICLE{Koehler06,
   author = {{K{\"o}hler}, M. and {Kimura}, H. and {Mann}, I.},
    title = "{Applicability of the discrete-dipole approximation to light-scattering simulations of large cosmic dust aggregates}",
  journal = {\aap},
 keywords = {scattering, solar system: general, circumstellar matter, dust, extinction, meteors, meteoroids},
     year = 2006,
    month = mar,
   volume = 448,
    pages = {395-399},
}

@ARTICLE{Koehler2007,
   author = {{K{\"o}hler}, M. and {Minato}, T. and {Kimura}, H. and {Mann}, I.
	},
    title = "{Radiation pressure force acting on cometary aggregates}",
  journal = {Advances in Space Research},
     year = 2007,
   volume = 40,
    pages = {266-271}
}

@INPROCEEDINGS{Kolokolova2011a,
   author = {{Kolokolova}, L. and {Petrova}, E. and {Kimura}, H.},
    title = "{Effects of Interaction of Electromagnetic Waves in Complex Particles}",
   booktitle = {Electromagnetic Waves},
     year = 2011,
    month = jun,
    editor = {{Zhurbenko}, V.},
    doi = {10.5772/16456},
    isbn={9789533073040},
    url = {http://www.intechopen.com/books/electromagnetic-waves/effects-of-interaction-of-electromagnetic-waves-in-complex-particles},
}

@ARTICLE{Kolokolova2011b,
   author = {{Kolokolova}, L. and {Liu}, L. and {Buratti}, B. and {Mishchenko}, M.~I.},
    title = "{Modeling variations in near-infrared spectra caused by the coherent backscattering effect}",
  journal = {Journal of Quantitative Spectroscopy {\&} Radiative Transfer},
     year = 2011,
    month = sep,
   volume = 112,
    pages = {2175-2181},
      doi = {10.1016/j.jqsrt.2011.03.010},
   adsurl = {http://adsabs.harvard.edu/abs/2011JQSRT.112.2175K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kopparapu2013,
   author = {{Kopparapu}, R.~K. and {Ramirez}, R. and {Kasting}, J.~F. and 
	{Eymet}, V. and {Robinson}, T.~D. and {Mahadevan}, S. and {Terrien}, R.~C. and 
	{Domagal-Goldman}, S. and {Meadows}, V. and {Deshpande}, R.},
    title = "{Habitable Zones around Main-sequence Stars: New Estimates}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.6674},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems },
     year = 2013,
    month = mar,
   volume = 765,
      eid = {131},
    pages = {131},
      doi = {10.1088/0004-637X/765/2/131},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...765..131K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@book{kopitzki2004,
  title={Einf{\"u}hrung in die Festk{\"o}rperphysik},
  author={Kopitzki, K. and Herzog, P.},
  isbn={9783519430834},
  year={2004},
  publisher={Teubner}
}

@ARTICLE{Kospal2009,
   author = {{K{\'o}sp{\'a}l}, {\'A}. and {Ardila}, D.~R. and {Mo{\'o}r}, A. and 
	{{\'A}brah{\'a}m}, P.},
    title = "{On the Relationship Between Debris Disks and Planets}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0907.0028},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, infrared: stars, Kuiper Belt, planetary systems},
     year = 2009,
    month = aug,
   volume = 700,
    pages = {L73-L77},
      doi = {10.1088/0004-637X/700/2/L73},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...700L..73K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kothe2013,
   author = {{Kothe}, S. and {Blum}, J. and {Weidling}, R. and {G{\"u}ttler}, C.
	},
    title = "{Free collisions in a microgravity many-particle experiment. III. The collision behavior of sub-millimeter-sized dust aggregates}",
  journal = {Icarus},
archivePrefix = "arXiv",
   eprint = {1302.5532},
 primaryClass = "astro-ph.EP",
     year = 2013,
    month = jul,
   volume = 225,
    pages = {75-85},
      doi = {10.1016/j.icarus.2013.02.034},
   adsurl = {http://adsabs.harvard.edu/abs/2013Icar..225...75K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Krist1998,
   author = {{Krist}, J.~E. and {Stapelfeldt}, K.~R. and {Burrows}, C.~J. and 
	{Ballester}, G.~E. and {Clarke}, J.~T. and {Crisp}, D. and {Evans}, R.~W. and 
	{Gallagher}, III, J.~S. and {Griffiths}, R.~E. and {Hester}, J.~J. and 
	{Hoessel}, J.~G. and {Holtzman}, J.~A. and {Mould}, J.~R. and 
	{Scowen}, P.~A. and {Trauger}, J.~T. and {Watson}, A.~M. and 
	{Westphal}, J.~A.},
    title = "{Hubble Space Telescope WFPC2 Imaging of FS Tauri and Haro 6-5B}",
  journal = {\apj},
 keywords = {STARS: BINARIES: VISUAL, STARS: CIRCUMSTELLAR MATTER, STARS: INDIVIDUAL NAME: HARO 6-5B, STARS: INDIVIDUAL CONSTELLATION NAME: FS TAURI, ISM: JETS AND OUTFLOWS},
     year = 1998,
    month = jul,
   volume = 501,
    pages = {841},
      doi = {10.1086/305861},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...501..841K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krist2005,
   author = {{Krist}, J.~E. and {Ardila}, D.~R. and {Golimowski}, D.~A. and 
	{Clampin}, M. and {Ford}, H.~C. and {Illingworth}, G.~D. and 
	{Hartig}, G.~F. and {Bartko}, F. and {Ben{\'{\i}}tez}, N. and 
	{Blakeslee}, J.~P. and {Bouwens}, R.~J. and {Bradley}, L.~D. and 
	{Broadhurst}, T.~J. and {Brown}, R.~A. and {Burrows}, C.~J. and 
	{Cheng}, E.~S. and {Cross}, N.~J.~G. and {Demarco}, R. and {Feldman}, P.~D. and 
	{Franx}, M. and {Goto}, T. and {Gronwall}, C. and {Holden}, B. and 
	{Homeier}, N. and {Infante}, L. and {Kimble}, R.~A. and {Lesser}, M.~P. and 
	{Martel}, A.~R. and {Mei}, S. and {Menanteau}, F. and {Meurer}, G.~R. and 
	{Miley}, G.~K. and {Motta}, V. and {Postman}, M. and {Rosati}, P. and 
	{Sirianni}, M. and {Sparks}, W.~B. and {Tran}, H.~D. and {Tsvetanov}, Z.~I. and 
	{White}, R.~L. and {Zheng}, W.},
    title = "{Hubble Space Telescope Advanced Camera for Surveys Coronagraphic Imaging of the AU Microscopii Debris Disk}",
  journal = {The Astronomical Journal},
     year = 2005,
    month = feb,
   volume = 129,
    pages = {1008-1017},
}

@ARTICLE{Krivov2006,
   author = {{Krivov}, A.~V. and {L{\"o}hne}, T. and {Srem{\v c}evi{\'c}}, M.
	},
    title = "{Dust distributions in debris disks: effects of gravity, radiation pressure and collisions}",
    journal = {\aap},
     year = 2006,
    month = aug,
   volume = 455,
    pages = {509-519},
}

@ARTICLE{Krivov2008,
   author = {{Krivov}, A.~V. and {M{\"u}ller}, S. and {L{\"o}hne}, T. and 
	{Mutschke}, H.},
    title = "{Collisional and Thermal Emission Models of Debris Disks: Toward Planetesimal Population Properties}",
  journal = {\apj},
    year = 2008,
    month = nov,
   volume = 687,
    pages = {608-622},
}

@ARTICLE{Krivov2010,
   author = {{Krivov}, A.~V.},
    title = "{Debris disks: seeing dust, thinking of planetesimals and planets}",
  journal = {Research in Astronomy and Astrophysics},
archivePrefix = "arXiv",
   eprint = {1003.5229},
 primaryClass = "astro-ph.EP",
     year = 2010,
    month = may,
   volume = 10,
    pages = {383-414},
      doi = {10.1088/1674-4527/10/5/001},
   adsurl = {http://adsabs.harvard.edu/abs/2010RAA....10..383K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{kruegel2002,
  title={The Physics of Interstellar Dust},
  author={Kr{\"u}gel, E.},
  isbn={9781420033335},
  lccn={2007299968},
  series={Series in Astronomy \& Astrophysics},
  url={http://books.google.de/books?id=LP2FwYKYrkMC},
  year={2002},
  publisher={Taylor {\&} Francis}
}



@ARTICLE{Kruger2011,
   author = {{Kruger}, A.~J. and {Richter}, M.~J. and {Carr}, J.~S. and {Najita}, J.~R. and 
	{Doppmann}, G.~W. and {Seifahrt}, A.},
    title = "{Gas and Dust Toward DG Tau B and VV CrA}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1102.1983},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, ISM: abundances, protoplanetary disks, stars: individual: DG Tau B VV CrA, stars: pre-main sequence},
     year = 2011,
    month = mar,
   volume = 729,
      eid = {145},
    pages = {145},
      doi = {10.1088/0004-637X/729/2/145},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...729..145K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kuhn2001,
   author = {{Kuhn}, J.~R. and {Potter}, D. and {Parise}, B.},
    title = "{Imaging Polarimetric Observations of a New Circumstellar Disk System}",
  journal = {\apj},
   eprint = {astro-ph/0105239},
 keywords = {Stars: Circumstellar Matter, Techniques: Polarimetric},
     year = 2001,
    month = jun,
   volume = 553,
    pages = {L189-L191},
      doi = {10.1086/320686},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553L.189K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1969,
   author = {{Kurucz}, R.~L.},
    title = "{A Matrix Method for Calculating the Source Function, Mean Intensity, and Flux in a Model Atmosphere}",
  journal = {\apj},
     year = 1969,
    month = apr,
   volume = 156,
    pages = {235},
      doi = {10.1086/149960},
   adsurl = {http://adsabs.harvard.edu/abs/1969ApJ...156..235K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lachaume1999,
   author = {{Lachaume}, R. and {Dominik}, C. and {Lanz}, T. and {Habing}, H.~J.
	},
    title = "{Age determinations of main-sequence stars: combining different methods}",
  journal = {\aap},
 keywords = {STARS: ACTIVITY, STARS: CHROMOSPHERES, STARS: EVOLUTION, STARS: ROTATION},
     year = 1999,
    month = aug,
   volume = 348,
    pages = {897-909},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...348..897L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Lada1987,
   author = {{Lada}, C.~J.},
    title = "{Star formation - From OB associations to protostars}",
 keywords = {B Stars, Binary Stars, O Stars, Protostars, Star Formation, Infrared Spectra, Molecular Clouds, Ophiuchi Clouds, Spectral Energy Distribution, Star Clusters, Stellar Evolution},
booktitle = {Star Forming Regions},
     year = 1987,
   series = {IAU Symposium},
   volume = 115,
   editor = {{Peimbert}, M. and {Jugaku}, J.},
    pages = {1-17},
   adsurl = {http://adsabs.harvard.edu/abs/1987IAUS..115....1L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LamyGrun,
   author = {{Lamy}, P.~L. and {Gruen}, E. and {Perrin}, J.~M.},
    title = "{Comet P/Halley - Implications of the mass distribution function for the photopolarimetric properties of the dust coma}",
journal={\aap},
year=1987,
    month = nov,
   volume = 187,
    pages = {767-773}
}

@ARTICLE{Lamy74b,
   author = {{Lamy}, P.~L.},
    title = "{Interaction of interplanetary dust grains with the solar radiation field}",
  journal = {\aap},
     year = 1974,
    month = oct,
   volume = 35,
    pages = {197-207}
}

@ARTICLE{Lamoreaux1987,
 author = {{Lamoreaux}, R.~H. and {Hildenbrand}, D.~L. and {Brewer}, L.
	},
    title = "{High-Temperature Vaporization Behavior of Oxides II. Oxides of Be, Mg, Ca, Sr, Ba, B, Al, Ga, In, Tl, Si, Ge, Sn, Pb, Zn, Cd, and Hg}",
  journal = {Journal of Physical and Chemical Reference Data},
     year = 1987,
    month = jul,
   volume = 16,
    pages = {419-443},
      doi = {10.1063/1.555799},
   adsurl = {http://adsabs.harvard.edu/abs/1987JPCRD..16..419L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lawler2014,
   author = {{Lawler}, S.~M. and {Di Francesco}, J. and {Kennedy}, G.~M. and 
	{Sibthorpe}, B. and {Booth}, M. and {Vandenbussche}, B. and 
	{Matthews}, B.~C. and {Holland}, W.~S. and {Greaves}, J. and 
	{Wilner}, D.~J. and {Tuomi}, M. and {Blommaert}, J.~A.~D.~L. and 
	{de Vries}, B.~L. and {Dominik}, C. and {Fridlund}, M. and {Gear}, W. and 
	{Heras}, A.~M. and {Ivison}, R. and {Olofsson}, G.},
    title = "{The debris disc of solar analogue {$\tau$} Ceti: Herschel observations and dynamical simulations of the proposed multiplanet system}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.2791},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: dynamical evolution and stability, planet-disc interactions, circumstellar matter, stars: individual: {$\tau$} Ceti},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {2665-2675},
      doi = {10.1093/mnras/stu1641},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.2665L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lebreton2013,
   author = {{Lebreton}, J. and {van Lieshout}, R. and {Augereau}, J.-C. and 
	{Absil}, O. and {Mennesson}, B. and {Kama}, M. and {Dominik}, C. and 
	{Bonsor}, A. and {Vandeportal}, J. and {Beust}, H. and {Defr{\`e}re}, D. and 
	{Ertel}, S. and {Faramaz}, V. and {Hinz}, P. and {Kral}, Q. and 
	{Lagrange}, A.-M. and {Liu}, W. and {Th{\'e}bault}, P.},
    title = "{An interferometric study of the Fomalhaut inner debris disk. III. Detailed models of the exozodiacal disk and its origin}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1306.0956},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, zodiacal dust, infrared: planetary systems, stars: individual: Fomalhaut, radiative transfer, circumstellar matter},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A146},
    pages = {A146},
      doi = {10.1051/0004-6361/201321415},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A.146L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lebouteiller2011,
   author = {{Lebouteiller}, V. and {Barry}, D.~J. and {Spoon}, H.~W.~W. and 
	{Bernard-Salas}, J. and {Sloan}, G.~C. and {Houck}, J.~R. and 
	{Weedman}, D.~W.},
    title = "{CASSIS: The Cornell Atlas of Spitzer/Infrared Spectrograph Sources}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1108.3507},
 primaryClass = "astro-ph.IM",
 keywords = {atlases, catalogs, infrared: general, methods: data analysis, techniques: spectroscopic},
     year = 2011,
    month = sep,
   volume = 196,
      eid = {8},
    pages = {8},
      doi = {10.1088/0067-0049/196/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..196....8L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lebreton2012,
   author = {{Lebreton}, J. and {Augereau}, J.-C. and {Thi}, W.-F. and {Roberge}, A. and 
	{Donaldson}, J. and {Schneider}, G. and {Maddison}, S.~T. and 
	{M{\'e}nard}, F. and {Riviere-Marichalar}, P. and {Mathews}, G.~S. and 
	{Kamp}, I. and {Pinte}, C. and {Dent}, W.~R.~F. and {Barrado}, D. and 
	{Duch{\^e}ne}, G. and {Gonzalez}, J.-F. and {Grady}, C.~A. and 
	{Meeus}, G. and {Pantin}, E. and {Williams}, J.~P. and {Woitke}, P.
	},
    title = "{An icy Kuiper belt around the young solar-type star HD 181327}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.3398},
 primaryClass = "astro-ph.EP",
 keywords = {stars: individual:HD 181327, circumstellar matter, infrared: planetary systems, radiative transfer},
     year = 2012,
    month = mar,
   volume = 539,
      eid = {A17},
    pages = {A17},
      doi = {10.1051/0004-6361/201117714},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A..17L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lee2004,
   author = {{Lee}, J.-E. and {Bergin}, E.~A. and {Evans}, II, N.~J.},
    title = "{Evolution of Chemistry and Molecular Line Profiles during Protostellar Collapse}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0408091},
 keywords = {Astrochemistry, ISM: Clouds, ISM: Molecules, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2004,
    month = dec,
   volume = 617,
    pages = {360-383},
      doi = {10.1086/425153},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...617..360L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee1985,
   author = {{Lee}, H.~M. and {Draine}, B.~T.},
    title = "{Infrared extinction and polarization due to partially aligned spheroidal grains - Models for the dust toward the BN object}",
  journal = {\apj},
 keywords = {Cosmic Dust, Infrared Astronomy, Molecular Clouds, Point Sources, Radiation Sources, Astronomical Models, Emission Spectra, Linear Polarization, Optical Properties, Orion Nebula, Shapes, Silicates},
     year = 1985,
    month = mar,
   volume = 290,
    pages = {211-228},
      doi = {10.1086/162974},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...290..211L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2003,
   author = {{Leggett}, S.~K. and {Hawarden}, T.~G. and {Currie}, M.~J. and 
	{Adamson}, A.~J. and {Carroll}, T.~C. and {Kerr}, T.~H. and 
	{Kuhn}, O.~P. and {Seigar}, M.~S. and {Varricatt}, W.~P. and 
	{Wold}, T.},
    title = "{L' and M' standard stars for the Mauna Kea Observatories Near-Infrared system}",
  journal = {\mnras},
   eprint = {astro-ph/0307032},
 keywords = {methods: data analysis, techniques: photometric, infrared: stars},
     year = 2003,
    month = oct,
   volume = 345,
    pages = {144-152},
      doi = {10.1046/j.1365-8711.2003.06943.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345..144L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Leinert1996,
   author = {{Leinert}, C.},
    title = "{Solar system objects and extragalactic background light.}",
 keywords = {Zodiacal Light: Models, Zodiacal Light: Infrared Radiation, Zodiacal Light: Comets, Zodiacal Light: Infrared Background, Interplanetary physics, Far infrared, Background radiations},
booktitle = {American Institute of Physics Conference Series},
     year = 1996,
   series = {American Institute of Physics Conference Series},
   volume = 348,
   editor = {{Dwek}, E.},
    pages = {53-63},
   adsurl = {http://adsabs.harvard.edu/abs/1996AIPC..348...53L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Lenzen2003,
   author = {{Lenzen}, R. and {Hartung}, M. and {Brandner}, W. and {Finger}, G. and 
	{Hubin}, N.~N. and {Lacombe}, F. and {Lagrange}, A.-M. and {Lehnert}, M.~D. and 
	{Moorwood}, A.~F.~M. and {Mouillet}, D.},
    title = "{NAOS-CONICA first on sky results in a variety of observing modes}",
booktitle = {Instrument Design and Performance for Optical/Infrared Ground-based Telescopes},
     year = 2003,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4841,
   editor = {{Iye}, M. and {Moorwood}, A.~F.~M.},
    month = mar,
    pages = {944-952},
      doi = {10.1117/12.460044},
   adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4841..944L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Li1998,
   author = {{Li}, A. and {Greenberg}, J.~M.},
    title = "{A comet dust model for the beta Pictoris disk}",
  journal = {\aap},
 keywords = {STARS: INDIVIDUAL: BETA PICTORIS, STARS: CIRCUMSTELLAR MATTER, STARS: PLANETARY SYSTEMS, ISM: DUST, COMETS: GENERAL},
     year = 1998,
    month = mar,
   volume = 331,
    pages = {291-313},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...331..291L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lisse2008,
   author = {{Lisse}, C.~M. and {Chen}, C.~H. and {Wyatt}, M.~C. and {Morlok}, A.
	},
    title = "{Circumstellar Dust Created by Terrestrial Planet Formation in HD 113766}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.0839},
 keywords = {infrared: stars, planetary systems: formation, planetary systems: protoplanetary disks, radiation mechanisms: thermal, techniques: spectroscopic},
     year = 2008,
    month = feb,
   volume = 673,
      eid = {1106-1122},
    pages = {1106-1122},
      doi = {10.1086/523626},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673.1106L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lisse2009,
   author = {{Lisse}, C.~M. and {Chen}, C.~H. and {Wyatt}, M.~C. and {Morlok}, A. and 
	{Song}, I. and {Bryden}, G. and {Sheehan}, P.},
    title = "{Abundant Circumstellar Silica Dust and SiO Gas Created by a Giant Hypervelocity Collision in the \~{}12 Myr HD172555 System}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0906.2536},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, infrared: stars, planetary systems: formation, planetary systems: protoplanetary disks, radiation mechanisms: thermal, techniques: spectroscopic},
     year = 2009,
    month = aug,
   volume = 701,
    pages = {2019-2032},
      doi = {10.1088/0004-637X/701/2/2019},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...701.2019L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Liu2012,
   author = {{Liu}, Y. and {Madlener}, D. and {Wolf}, S. and {Wang}, H. and 
	{Ruge}, J.~P.},
    title = "{DoAr 33: a good candidate for revealing dust growth and settling in protoplanetary disks}",
  journal = {\aap},
 keywords = {circumstellar matter, protoplanetary disks, radiative transfer},
     year = 2012,
    month = oct,
   volume = 546,
      eid = {A7},
    pages = {A7},
      doi = {10.1051/0004-6361/201219336},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...546A...7L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodders2003,
   author = {{Lodders}, K.},
    title = "{Solar System Abundances and Condensation Temperatures of the Elements}",
  journal = {\apj},
     year = 2003,
    month = jul,
   volume = 591,
    pages = {1220-1247},
}

@ARTICLE{Loehne2008,
   author = {{L{\"o}hne}, T. and {Krivov}, A.~V. and {Rodmann}, J.},
    title = "{Long-Term Collisional Evolution of Debris Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.4294},
 keywords = {circumstellar matter, planetary systems: formation},
     year = 2008,
    month = feb,
   volume = 673,
      eid = {1123-1137},
    pages = {1123-1137},
      doi = {10.1086/524840},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673.1123L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Loehne2012,
   author = {{L{\"o}hne}, T. and {Augereau}, J.-C. and {Ertel}, S. and {Marshall}, J.~P. and 
	{Eiroa}, C. and {Mora}, A. and {Absil}, O. and {Stapelfeldt}, K. and 
	{Th{\'e}bault}, P. and {Bayo}, A. and {Del Burgo}, C. and {Danchi}, W. and 
	{Krivov}, A.~V. and {Lebreton}, J. and {Letawe}, G. and {Magain}, P. and 
	{Maldonado}, J. and {Montesinos}, B. and {Pilbratt}, G.~L. and 
	{White}, G.~J. and {Wolf}, S.},
    title = "{Modelling the huge, Herschel-resolved debris ring around HD 207129}",
  journal = {\aap},
 keywords = {interplanetary medium, stars: individual: HD 207129},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A110},
    pages = {A110},
      doi = {10.1051/0004-6361/201117731},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.110L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lopez2014,
   author = {{Lopez}, B. and {Lagarde}, S. and {Jaffe}, W. and {Petrov}, R. and 
	{Sch{\"o}ller}, M. and {Antonelli}, P. and {Beckmann}, U. and 
	{Berio}, P. and {Bettonvil}, F. and {Glindemann}, A. and {Gonzalez}, J.-C. and 
	{Graser}, U. and {Hofmann}, K.-H. and {Millour}, F. and {Robbe-Dubois}, S. and 
	{Venema}, L. and {Wolf}, S. and {Henning}, T. and {Lanz}, T. and 
	{Weigelt}, G. and {Agocs}, T. and {Bailet}, C. and {Bresson}, Y. and 
	{Bristow}, P. and {Dugu{\'e}}, M. and {Heininger}, M. and {Kroes}, G. and 
	{Laun}, W. and {Lehmitz}, M. and {Neumann}, U. and {Augereau}, J.-C. and 
	{Avila}, G. and {Behrend}, J. and {van Belle}, G. and {Berger}, J.-P. and 
	{van Boekel}, R. and {Bonhomme}, S. and {Bourget}, P. and {Brast}, R. and 
	{Clausse}, J.-M. and {Connot}, C. and {Conzelmann}, R. and {Cruzal{\`e}bes}, P. and 
	{Csepany}, G. and {Danchi}, W. and {Delbo}, M. and {Delplancke}, F. and 
	{Dominik}, C. and {van Duin}, A. and {Elswijk}, E. and {Fantei}, Y. and 
	{Finger}, G. and {Gabasch}, A. and {Gay}, J. and {Girard}, P. and 
	{Girault}, V. and {Gitton}, P. and {Glazenborg}, A. and {Gont{\'e}}, F. and 
	{Guitton}, F. and {Guniat}, S. and {De Haan}, M. and {Haguenauer}, P. and 
	{Hanenburg}, H. and {Hogerheijde}, M. and {ter Horst}, R. and 
	{Hron}, J. and {Hugues}, Y. and {Hummel}, C. and {Idserda}, J. and 
	{Ives}, D. and {Jakob}, G. and {Jasko}, A. and {Jolley}, P. and 
	{Kiraly}, S. and {K{\"o}hler}, R. and {Kragt}, J. and {Kroener}, T. and 
	{Kuindersma}, S. and {Labadie}, L. and {Leinert}, C. and {Le Poole}, R. and 
	{Lizon}, J.-L. and {Lucuix}, C. and {Marcotto}, A. and {Martinache}, F. and 
	{Martinot-Lagarde}, G. and {Mathar}, R. and {Matter}, A. and 
	{Mauclert}, N. and {Mehrgan}, L. and {Meilland}, A. and {Meisenheimer}, K. and 
	{Meisner}, J. and {Mellein}, M. and {Menardi}, S. and {Menut}, J.-L. and 
	{Merand}, A. and {Morel}, S. and {Mosoni}, L. and {Navarro}, R. and 
	{Nussbaum}, E. and {Ottogalli}, S. and {Palsa}, R. and {Panduro}, J. and 
	{Pantin}, E. and {Parra}, T. and {Percheron}, I. and {Duc}, T.~P. and 
	{Pott}, J.-U. and {Pozna}, E. and {Przygodda}, F. and {Rabbia}, Y. and 
	{Richichi}, A. and {Rigal}, F. and {Roelfsema}, R. and {Rupprecht}, G. and 
	{Schertl}, D. and {Schmidt}, C. and {Schuhler}, N. and {Schuil}, M. and 
	{Spang}, A. and {Stegmeier}, J. and {Thiam}, L. and {Tromp}, N. and 
	{Vakili}, F. and {Vannier}, M. and {Wagner}, K. and {Woillez}, J.
	},
    title = "{An Overview of the MATISSE Instrument {\mdash} Science, Concept and Current Status}",
  journal = {The Messenger},
     year = 2014,
    month = sep,
   volume = 157,
    pages = {5-12},
   adsurl = {http://adsabs.harvard.edu/abs/2014Msngr.157....5L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Lorentz,
title={"Theory of Electrons"},
author={ H. A. Lorentz},
publisher={Teubner, Leipzig},
year={1909},
}

@ARTICLE{Lucy1999,
   author = {{Lucy}, L.~B.},
    title = "{Computing radiative equilibria with Monte Carlo techniques}",
  journal = {\aap},
 keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, STARS: ATMOSPHERES},
     year = 1999,
    month = apr,
   volume = 344,
    pages = {282-288},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...344..282L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luhman2010,
   author = {{Luhman}, K.~L. and {Allen}, P.~R. and {Espaillat}, C. and {Hartmann}, L. and 
	{Calvet}, N.},
    title = "{The Disk Population of the Taurus Star-Forming Region}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0911.5457},
 primaryClass = "astro-ph.GA",
 keywords = {accretion, accretion disks, brown dwarfs, protoplanetary disks, stars: formation, stars: low-mass, stars: pre-main sequence},
     year = 2010,
    month = jan,
   volume = 186,
    pages = {111-174},
      doi = {10.1088/0067-0049/186/1/111},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186..111L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mackowski1991,
   author = {{Mackowski}, D.~W.},
    title = "{Analysis of radiative scattering for multiple sphere configurations}",
  journal = {Royal Society of London Proceedings Series A},
 keywords = {Atmospheric Scattering, Radiation Absorption, Radiative Transfer, Scattering Coefficients, Atmospheric Models, Mie Scattering, Spherical Harmonics},
     year = 1991,
    month = jun,
   volume = 433,
    pages = {599-614},
      doi = {10.1098/rspa.1991.0066},
   adsurl = {http://adsabs.harvard.edu/abs/1991RSPSA.433..599M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mackowski1996,
   author = {{Mackowski}, D.~W. and {Mishchenko}, M.~I.},
    title = "{Calculation of the T matrix and the scattering matrix for ensembles of spheres}",
  journal = {Journal of the Optical Society of America A},
     year = 1996,
    month = nov,
   volume = 13,
    pages = {2266-2278},
      doi = {10.1364/JOSAA.13.002266},
   adsurl = {http://adsabs.harvard.edu/abs/1996JOSAA..13.2266M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Madlener2012,
   author = {{Madlener}, D. and {Wolf}, S. and {Dutrey}, A. and {Guilloteau}, S.
	},
    title = "{The circumstellar disk of HH 30. Searching for signs of disk evolution with multi-wavelength modeling}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.4901},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, methods: data analysis, stars: formation, stars: variables: T Tauri, Herbig Ae/Be, stars: individual: HH 30, protoplanetary disks},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {A81},
    pages = {A81},
      doi = {10.1051/0004-6361/201117615},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A..81M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magnelli2013,
   author = {{Magnelli}, B. and {Popesso}, P. and {Berta}, S. and {Pozzi}, F. and 
	{Elbaz}, D. and {Lutz}, D. and {Dickinson}, M. and {Altieri}, B. and 
	{Andreani}, P. and {Aussel}, H. and {B{\'e}thermin}, M. and 
	{Bongiovanni}, A. and {Cepa}, J. and {Charmandaris}, V. and 
	{Chary}, R.-R. and {Cimatti}, A. and {Daddi}, E. and {F{\"o}rster Schreiber}, N.~M. and 
	{Genzel}, R. and {Gruppioni}, C. and {Harwit}, M. and {Hwang}, H.~S. and 
	{Ivison}, R.~J. and {Magdis}, G. and {Maiolino}, R. and {Murphy}, E. and 
	{Nordon}, R. and {Pannella}, M. and {P{\'e}rez Garc{\'{\i}}a}, A. and 
	{Poglitsch}, A. and {Rosario}, D. and {Sanchez-Portal}, M. and 
	{Santini}, P. and {Scott}, D. and {Sturm}, E. and {Tacconi}, L.~J. and 
	{Valtchanov}, I.},
    title = "{The deepest Herschel-PACS far-infrared survey: number counts and infrared luminosity functions from combined PEP/GOODS-H observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.4436},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, infrared: galaxies, galaxies: starburst, galaxies: statistics},
     year = 2013,
    month = may,
   volume = 553,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201321371},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...553A.132M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maldonado2010,
   author = {{Maldonado}, J. and {Mart{\'{\i}}nez-Arn{\'a}iz}, R.~M. and 
	{Eiroa}, C. and {Montes}, D. and {Montesinos}, B.},
    title = "{A spectroscopy study of nearby late-type stars, possible members of stellar kinematic groups}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1007.1132},
 primaryClass = "astro-ph.SR",
 keywords = {stars: late-type, stars: kinematics and dynamics, open clusters and associations: general},
     year = 2010,
    month = oct,
   volume = 521,
      eid = {A12},
    pages = {A12},
      doi = {10.1051/0004-6361/201014948},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...521A..12M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maldonado2012,
   author = {{Maldonado}, J. and {Eiroa}, C. and {Villaver}, E. and {Montesinos}, B. and 
	{Mora}, A.},
    title = "{Metallicity of solar-type stars with debris discs and planets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1202.5884},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: spectroscopic, stars: abundances, circumstellar matter, stars: late-type, planetary systems},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A40},
    pages = {A40},
      doi = {10.1051/0004-6361/201218800},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A..40M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mamajek2012,
   author = {{Mamajek}, E.~E.},
    title = "{On the Age and Binarity of Fomalhaut}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1206.6353},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, circumstellar matter, planetary systems, stars: activity, stars: fundamental parameters, stars: individual: Fomalhaut TW PsA},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/754/2/L20},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754L..20M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mamajek2014,
   author = {{Mamajek}, E.~E. and {Bell}, C.~P.~M.},
    title = "{On the age of the {$\beta$} Pictoris moving group}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.2737},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: fundamental parameters, stars: kinematics and dynamics, open clusters and associations: individual: {$\beta$} Pictoris moving group},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {2169-2180},
      doi = {10.1093/mnras/stu1894},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445.2169M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mann2004,
   author = {{Mann}, I. and {Kimura}, H. and {Biesecker}, D.~A. and {Tsurutani}, B.~T. and 
	{Gr{\"u}n}, E. and {McKibben}, R.~B. and {Liou}, J.-C. and {MacQueen}, R.~M. and 
	{Mukai}, T. and {Guhathakurta}, M. and {Lamy}, P.},
    title = "{Dust Near The Sun}",
  journal = {\ssr},
     year = 2004,
    month = jan,
   volume = 110,
    pages = {269-305},
      doi = {10.1023/B:SPAC.0000023440.82735.ba},
   adsurl = {http://adsabs.harvard.edu/abs/2004SSRv..110..269M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marion2014,
   author = {{Marion}, L. and {Absil}, O. and {Ertel}, S. and {Le Bouquin}, J.-B. and 
	{Augereau}, J.-C. and {Blind}, N. and {Defr{\`e}re}, D. and 
	{Lebreton}, J. and {Milli}, J.},
    title = "{Searching for faint companions with VLTI/PIONIER. II. 92 main sequence stars from the Exozodi survey}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1409.6105},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: close, circumstellar matter, techniques: interferometric},
     year = 2014,
    month = oct,
   volume = 570,
      eid = {A127},
    pages = {A127},
      doi = {10.1051/0004-6361/201424780},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...570A.127M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marshall2014,
   author = {{Marshall}, J.~P. and {Kirchschlager}, F. and {Ertel}, S. and 
	{Augereau}, J.-C. and {Kennedy}, G.~M. and {Booth}, M. and {Wolf}, S. and 
	{Montesinos}, B. and {Eiroa}, C. and {Matthews}, B.},
    title = "{Interpreting the extended emission around three nearby debris disc host stars}",
  journal = {\aap},,
archivePrefix = "arXiv",
   eprint = {1408.5649},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: HIP 22263, stars: individual: HIP 62207, stars: individual: HIP 72848, infrared: stars},
     year = 2014,
    month = oct,
   volume = 570,
      eid = {A114},
    pages = {A114},
      doi = {10.1051/0004-6361/201424517},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...570A.114M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marshall2016,
author = {{Marshall}, J.~P. and {Cotton}, D.~V. and {Bott}, K. and {Ertel}, S. and 
	{Kennedy}, G.~M. and {Wyatt}, M.~C. and {del Burgo}, C. and 
	{Absil}, O. and {Bailey}, J. and {Kedziora-Chudczer}, L.},
    title = "{Polarization Measurements of Hot Dust Stars and the Local Interstellar Medium}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1604.08286},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, dust, extinction, planetary systems, polarization},
     year = 2016,
    month = jul,
   volume = 825,
      eid = {124},
    pages = {124},
      doi = {10.3847/0004-637X/825/2/124},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...825..124M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Marti1993,
   author = {{Marti}, J. and {Rodriguez}, L.~F. and {Reipurth}, B.},
    title = "{HH 80-81: A Highly Collimated Herbig-Haro Complex Powered by a Massive Young Star}",
  journal = {\apj},
 keywords = {ISM: JETS AND OUTFLOWS, RADIO CONTINUUM: INTERSTELLAR, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE},
     year = 1993,
    month = oct,
   volume = 416,
    pages = {208},
      doi = {10.1086/173227},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...416..208M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Martinez2010,
   author = {{Mart{\'{\i}}nez-Arn{\'a}iz}, R. and {Maldonado}, J. and {Montes}, D. and 
	{Eiroa}, C. and {Montesinos}, B.},
    title = "{Chromospheric activity and rotation of FGK stars in the solar vicinity. An estimation of the radial velocity jitter}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.4391},
 primaryClass = "astro-ph.SR",
 keywords = {solar neighbourhood, stars: late-type, stars: activity, stars: chromospheres, stars: rotation, planetary systems},
     year = 2010,
    month = sep,
   volume = 520,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/200913725},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...520A..79M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Mather2010,
   author = {{Mather}, J.~C.},
    title = "{The James Webb Space Telescope Mission}",
 keywords = {astronomical telescopes, galaxies, cosmology, infrared detectors, dark matter, Astrometric and interferometric instruments, Galaxy clusters, Origin and formation of the Universe, Charge-coupled devices image detectors and IR detector arrays, Dark energy},
booktitle = {American Institute of Physics Conference Series},
     year = 2010,
   series = {American Institute of Physics Conference Series},
   volume = 1294,
   editor = {{Whalen}, D.~J. and {Bromm}, V. and {Yoshida}, N.},
    month = nov,
    pages = {1-8},
      doi = {10.1063/1.3518853},
   adsurl = {http://adsabs.harvard.edu/abs/2010AIPC.1294....1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mathieu2000,
   author = {{Mathieu}, R.~D. and {Ghez}, A.~M. and {Jensen}, E.~L.~N. and 
	{Simon}, M.},
    title = "{Young Binary Stars and Associated Disks}",
  journal = {Protostars and Planets IV},
   eprint = {astro-ph/9909424},
     year = 2000,
    month = may,
    pages = {703},
   adsurl = {http://adsabs.harvard.edu/abs/2000prpl.conf..703M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mathis1977,
   author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
    title = "{The size distribution of interstellar grains}",
  journal = {\apj},
 keywords = {COSMIC DUST, INTERSTELLAR EXTINCTION, INTERSTELLAR MATTER, PARTICLE SIZE DISTRIBUTION, ENSTATITE, GRAPHITE, MAGNETITE, OLIVINE, POLARIZATION CHARACTERISTICS, ULTRAVIOLET ASTRONOMY},
     year = 1977,
    month = oct,
   volume = 217,
    pages = {425-433},
      doi = {10.1086/155591},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matter2016a,
   author = {{Matter}, A. and {Lopez}, B. and {Antonelli}, P. and {Lehmitz}, M. and 
	{Bettonvil}, F. and {Beckmann}, U. and {Lagarde}, S. and {Jaffe}, W. and 
	{Petrov}, R.~G. and {Berio}, P. and {Millour}, F. and {Robbe-Dubois}, S. and 
	{Glindemann}, A. and {Bristow}, P. and {Schoeller}, M. and {Lanz}, T. and 
	{Henning}, T. and {Weigelt}, G. and {Heininger}, M. and {Morel}, S. and 
	{Cruzalebes}, P. and {Meisenheimer}, K. and {Hofferbert}, R. and 
	{Wolf}, S. and {Bresson}, Y. and {Agocs}, T. and {Allouche}, F. and 
	{Augereau}, J.-C. and {Avila}, G. and {Bailet}, C. and {Behrend}, J. and 
	{Van Belle}, G. and {Berger}, J.-P. and {van Boekel}, R. and 
	{Bourget}, P. and {Brast}, R. and {Clausse}, J.-M. and {Connot}, C. and 
	{Conzelmann}, R. and {Csepany}, G. and {Danchi}, W.~C. and {Delbo}, M. and 
	{Dominik}, C. and {van Duin}, A. and {Elswijk}, E. and {Fantei}, Y. and 
	{Finger}, G. and {Gabasch}, A. and {Gont{\'e}}, F. and {Graser}, U. and 
	{Guitton}, F. and {Guniat}, S. and {De Haan}, M. and {Haguenauer}, P. and 
	{Hanenburg}, H. and {Hofmann}, K.-H. and {Hogerheijde}, M. and 
	{ter Horst}, R. and {Hron}, J. and {Hummel}, C. and {Isderda}, J. and 
	{Ives}, D. and {Jakob}, G. and {Jasko}, A. and {Jolley}, P. and 
	{Kiraly}, S. and {Kragt}, J. and {Kroener}, T. and {Kroes}, G. and 
	{Kuindersma}, S. and {Labadie}, L. and {Laun}, W. and {Leinert}, C. and 
	{Lizon}, J.-L. and {Lucuix}, C. and {Marcotto}, A. and {Martinache}, F. and 
	{Martinot-Lagarde}, G. and {Mauclert}, N. and {Mehrgan}, L. and 
	{Meilland}, A. and {Mellein}, M. and {Menardi}, S. and {Merand}, A. and 
	{Neumann}, U. and {Nussbaum}, E. and {Ottogalli}, S. and {Palsa}, R. and 
	{Panduro}, J. and {Pantin}, E. and {Percheron}, I. and {Phan Duc}, T. and 
	{Pott}, J.-U. and {Pozna}, E. and {Roelfsema}, R. and {Rupprecht}, G. and 
	{Schertl}, D. and {Schmidt}, C. and {Schuil}, M. and {Spang}, A. and 
	{stegmeier}, J. and {Tromp}, N. and {Vakili}, F. and {Vannier}, M. and 
	{Wagner}, K. and {Venema}, L. and {Woillez}, J.},
    title = "{An overview of the mid-infrared spectro-interferometer MATISSE: science, concept, and current status}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.02350},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160802350M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matter2016b,
   author = {{Matter}, A. and {Lagarde}, S. and {Petrov}, R.~G. and {Berio}, P. and 
	{Robbe-Dubois}, S. and {Lopez}, B. and {Antonelli}, P. and {Allouche}, F. and 
	{Cruzalebes}, P. and {Millour}, F. and {Bazin}, G. and {Bourg{\`e}s}, L.
	},
    title = "{MATISSE: specifications and expected performances}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.02351},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160802351M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Matthews2010,
   author = {{Matthews}, B.~C. and {Sibthorpe}, B. and {Kennedy}, G. and 
	{Phillips}, N. and {Churcher}, L. and {Duch{\^e}ne}, G. and 
	{Greaves}, J.~S. and {Lestrade}, J.-F. and {Moro-Martin}, A. and 
	{Wyatt}, M.~C. and {Bastien}, P. and {Biggs}, A. and {Bouvier}, J. and 
	{Butner}, H.~M. and {Dent}, W.~R.~F. and {di Francesco}, J. and 
	{Eisl{\"o}ffel}, J. and {Graham}, J. and {Harvey}, P. and {Hauschildt}, P. and 
	{Holland}, W.~S. and {Horner}, J. and {Ibar}, E. and {Ivison}, R.~J. and 
	{Johnstone}, D. and {Kalas}, P. and {Kavelaars}, J. and {Rodriguez}, D. and 
	{Udry}, S. and {van der Werf}, P. and {Wilner}, D. and {Zuckerman}, B.
	},
    title = "{Resolving debris discs in the far-infrared: Early highlights from the DEBRIS survey}",
  journal = {\aap},
 keywords = {circumstellar matter, stars: individual: {$\beta$} Leo, infrared: stars, stars: individual: {$\beta$} UMa, stars: individual: {$\eta$} Corvi},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L135},
    pages = {L135},
      doi = {10.1051/0004-6361/201014667},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L.135M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Matthews2014,
 author = {{Matthews}, B.~C. and {Krivov}, A.~V. and {Wyatt}, M.~C. and 
	{Bryden}, G. and {Eiroa}, C.},
    title = "{Observations, Modeling, and Theory of Debris Disks}",
  journal = {Protostars and Planets VI},
archivePrefix = "arXiv",
   eprint = {1401.0743},
 primaryClass = "astro-ph.SR",
     year = 2014,
    pages = {521-544},
      doi = {10.2458/azu_uapress_9780816531240-ch023},
   adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..521M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mawet2011,
   author = {{Mawet}, D. and {Mennesson}, B. and {Serabyn}, E. and {Stapelfeldt}, K. and 
	{Absil}, O.},
    title = "{A Dim Candidate Companion to epsilon Cephei}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1107.3872},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, instrumentation: adaptive optics, instrumentation: high angular resolution, stars: low-mass, techniques: high angular resolution},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {L12},
    pages = {L12},
      doi = {10.1088/2041-8205/738/1/L12},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738L..12M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{McCabe2003,
   author = {{McCabe}, C. and {Duch{\^e}ne}, G. and {Ghez}, A.~M.},
    title = "{The First Detection of Spatially Resolved Mid-Infrared Scattered Light from a Protoplanetary Disk}",
  journal = {\apj},
   eprint = {astro-ph/0304083},
 keywords = {Stars: Binaries: Visual, ISM: Dust, Extinction, Stars: Planetary Systems: Protoplanetary Disks, Scattering, Stars: Individual: Constellation Name: HK Tauri, Stars: Pre-Main-Sequence},
     year = 2003,
    month = may,
   volume = 588,
    pages = {L113-L116},
      doi = {10.1086/375632},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588L.113M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McCaughrean2000,
   author = {{McCaughrean}, M.~J. and {Stapelfeldt}, K.~R. and {Close}, L.~M.
	},
    title = "{High-Resolution Optical and Near-Infrared Imaging of Young Circumstellar Disks}",
  journal = {Protostars and Planets IV},
     year = 2000,
    month = may,
    pages = {485},
   adsurl = {http://adsabs.harvard.edu/abs/2000prpl.conf..485M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{McDonald2009,
   author = {{Mc Donald}, J. and {Golden}, A. and {Jennings}, S.~G.},
    title = "{OpenDDA: A Novel High-Performance Computational Framework for the Discrete Dipole Approximation.}",
  journal = {International Journal of High Performance Computing Applications (IJHPCA)},
     year = 2009,
    month = aug,
volume = 23,
number=1,
pages= {42-61}
}

@ARTICLE{Menard1988,
   author = {{Menard}, F. and {Bastien}, P. and {Robert}, C.},
    title = "{Detection of circular polarization in R Monocerotis and NGC 2261 - Implications for the polarization mechanism}",
  journal = {\apj},
 keywords = {CIRCULAR POLARIZATION, EARLY STARS, REFLECTION NEBULAE, STELLAR ENVELOPES, STELLAR MAGNETIC FIELDS, AMBIPOLAR DIFFUSION, LINEAR POLARIZATION, MOLECULAR CLOUDS, STAR FORMATION, STELLAR LUMINOSITY},
     year = 1988,
    month = dec,
   volume = 335,
    pages = {290-294},
      doi = {10.1086/166926},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...335..290M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Mennesson2014,
   author = {{Mennesson}, B. and {Millan-Gabet}, R. and {Serabyn}, E. and 
	{Colavita}, M.~M. and {Absil}, O. and {Bryden}, G. and {Wyatt}, M. and 
	{Danchi}, W. and {Defr{\`e}re}, D. and {Dor{\'e}}, O. and {Hinz}, P. and 
	{Kuchner}, M. and {Ragland}, S. and {Scott}, N. and {Stapelfeldt}, K. and 
	{Traub}, W. and {Woillez}, J.},
    title = "{Constraining the Exozodiacal Luminosity Function of Main-sequence Stars: Complete Results from the Keck Nuller Mid-infrared Surveys}",
  journal = {\apj},
 keywords = {circumstellar matter, infrared: stars, instrumentation: interferometers },
     year = 2014,
    month = dec,
   volume = 797,
      eid = {119},
    pages = {119},
      doi = {10.1088/0004-637X/797/2/119},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...797..119M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Metchev2004,
   author = {{Metchev}, S.~A. and {Hillenbrand}, L.~A. and {Meyer}, M.~R.},
    title = "{Ten Micron Observations of Nearby Young Stars}",
  journal = {\apj},
     year = 2004,
    month = jan,
   volume = 600,
    pages = {435-450},
}


@ARTICLE{Metchev2005,
   author = {{Metchev}, S.~A. and {Eisner}, J.~A. and {Hillenbrand}, L.~A. and 
	{Wolf}, S.},
    title = "{Adaptive Optics Imaging of the AU Microscopii Circumstellar Disk: Evidence for Dynamical Evolution}",
  journal = {\apj},
   eprint = {astro-ph/0412143},
 keywords = {Stars: Circumstellar Matter, Instrumentation: Adaptive Optics, Stars: Planetary Systems: Protoplanetary Disks, Stars: Individual: Constellation Name: AU Microscopii, Stars: Low-Mass, Brown Dwarfs},
     year = 2005,
    month = mar,
   volume = 622,
    pages = {451-462},
      doi = {10.1086/427869},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..451M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Meyer2008,
   author = {{Meyer}, M.~R. and {Carpenter}, J.~M. and {Mamajek}, E.~E. and 
	{Hillenbrand}, L.~A. and {Hollenbach}, D. and {Moro-Martin}, A. and 
	{Kim}, J.~S. and {Silverstone}, M.~D. and {Najita}, J. and {Hines}, D.~C. and 
	{Pascucci}, I. and {Stauffer}, J.~R. and {Bouwman}, J. and {Backman}, D.~E.},
    title = "{Evolution of Mid-Infrared Excess around Sun-like Stars: Constraints on Models of Terrestrial Planet Formation}",
  journal = {\apj},
     year = 2008,
    month = feb,
   volume = 673,
    pages = {L181-L184}
}

@Article{Mie1908,
 author = {{Mie}, G.},
    title = "{Beitr{\"a}ge zur Optik tr{\"u}ber Medien, speziell kolloidaler Metall{\"o}sungen}",
  journal = {Annalen der Physik},
     year = 1908,
   volume = 330,
    pages = {377-445},
      doi = {10.1002/andp.19083300302},
   adsurl = {http://adsabs.harvard.edu/abs/1908AnP...330..377M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Millour2008,
   author = {{Millour}, F.},
    title = "{All you ever wanted to know about optical long baseline stellar interferometry, but were too shy to ask your adviser}",
  journal = {New Astronomy Reviews},
archivePrefix = "arXiv",
   eprint = {0804.2368},
     year = 2008,
    month = jun,
   volume = 52,
    pages = {177-185},
      doi = {10.1016/j.newar.2008.04.012},
   adsurl = {http://adsabs.harvard.edu/abs/2008NewAR..52..177M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Millour2016,
   author = {{Millour}, F. and {Berio}, P and {Heininger}, M and {Hofmann}, K.-H and 
	{Schertl}, D and {Weigelt}, G and {Guitton}, F and {Jaffe}, W and 
	{Beckmann}, U and {Petrov}, R and {Allouche}, F and {Robbe-Dubois}, S and 
	{Lagarde}, S and {Soulain}, A and {Meilland}, A and {Matter}, A and 
	{Cruzal{\`e}bes}, P and {Lopez}, B},
    title = "{Data reduction for the MATISSE instrument}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.01913},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160801913M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Min2003,
   author = {{Min}, M. and {Hovenier}, J.~W. and {de Koter}, A.},
    title = "{Shape effects in scattering and absorption by randomly oriented particles small compared to the wavelength}",
  journal = {\aap},
 keywords = {scattering, stars: circumstellar matter, stars: planetary systems: protoplanetary disks},
     year = 2003,
    month = jun,
   volume = 404,
    pages = {35-46},
      doi = {10.1051/0004-6361:20030456},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...404...35M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Min2005,
   author = {{Min}, M. and {Hovenier}, J.~W. and {de Koter}, A.},
    title = "{Modeling optical properties of cosmic dust grains using a distribution of hollow spheres}",
  journal = {\aap},
     year = 2005,
    month = mar,
   volume = 432,
    pages = {909-920}
}

@ARTICLE{Min2007,
   author = {{Min}, M. and {Waters}, L.~B.~F.~M. and {de Koter}, A. and {Hovenier}, J.~W. and 
	{Keller}, L.~P. and {Markwick-Kemper}, F.},
    title = "{The shape and composition of interstellar silicate grains}",
  journal = {\aap},
   eprint = {astro-ph/0611329},
 keywords = {dust, extinction, infrared: ISM},
     year = 2007,
    month = feb,
   volume = 462,
    pages = {667-676},
      doi = {10.1051/0004-6361:20065436},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...462..667M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Min2011,
   author = {{Min}, M. and {Dullemond}, C.~P. and {Kama}, M. and {Dominik}, C.
	},
    title = "{The thermal structure and the location of the snow line in the protosolar nebula: Axisymmetric models with full 3-D radiative transfer}",
  journal = {Icarus},
archivePrefix = "arXiv",
   eprint = {1012.0727},
 primaryClass = "astro-ph.EP",
     year = 2011,
    month = mar,
   volume = 212,
    pages = {416-426},
      doi = {10.1016/j.icarus.2010.12.002},
   adsurl = {http://adsabs.harvard.edu/abs/2011Icar..212..416M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Min2012,
   author = {{Min}, M. and {Canovas}, H. and {Mulders}, G.~D. and {Keller}, C.~U.
	},
    title = "{The effects of disk and dust structure on observed polarimetric images of protoplanetary disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.4348},
 primaryClass = "astro-ph.EP",
 keywords = {radiative transfer, polarization, stars: pre-main sequence, protoplanetary disks, scattering},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A75},
    pages = {A75},
      doi = {10.1051/0004-6361/201117333},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..75M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mishchenko2006,
   author = {{Mishchenko}, M.~I. and {Rosenbush}, V.~K. and {Kiselev}, N.~N.
	},
    title = "{Weak localization of electromagnetic waves and opposition phenomena exhibited by high-albedo atmosphereless solar system objects}",
  journal = {Applied Optics IP},
 keywords = {Coherent optical effects, Radiative transfer, Backscattering, Multiple scattering, Scattering, particles},
     year = 2006,
    month = jun,
   volume = 45,
    pages = {4459-4463},
      doi = {10.1364/AO.45.004459},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApOpt..45.4459M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mishchenko2009,
   author = {{Mishchenko}, M.~I. and {Dlugach}, J.~M. and {Liu}, L. and {Rosenbush}, V.~K. and 
	{Kiselev}, N.~N. and {Shkuratov}, Y.~G.},
    title = "{Direct Solutions of the Maxwell Equations Explain Opposition Phenomena Observed for High-Albedo Solar System Objects}",
  journal = {\apjl},
 keywords = {minor planets, asteroids, planets and satellites: individual: Europa, polarization, radiative transfer, scattering},
     year = 2009,
    month = nov,
   volume = 705,
    pages = {L118-L122},
      doi = {10.1088/0004-637X/705/2/L118},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705L.118M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Monnier2003,
   author = {{Monnier}, J.~D.},
    title = "{Optical interferometry in astronomy}",
  journal = {Reports on Progress in Physics},
   eprint = {astro-ph/0307036},
     year = 2003,
    month = may,
   volume = 66,
    pages = {789-857},
      doi = {10.1088/0034-4885/66/5/203},
   adsurl = {http://adsabs.harvard.edu/abs/2003RPPh...66..789M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Monnier2012,
   author = {{Monnier}, J.~D. and {Che}, X. and {Zhao}, M. and {Ekstr{\"o}m}, S. and 
	{Maestro}, V. and {Aufdenberg}, J. and {Baron}, F. and {Georgy}, C. and 
	{Kraus}, S. and {McAlister}, H. and {Pedretti}, E. and {Ridgway}, S. and 
	{Sturmann}, J. and {Sturmann}, L. and {ten Brummelaar}, T. and 
	{Thureau}, N. and {Turner}, N. and {Tuthill}, P.~G.},
    title = "{Resolving Vega and the Inclination Controversy with CHARA/MIRC}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1211.6055},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, stars: individual: Vega, stars: rotation, techniques: interferometric},
     year = 2012,
    month = dec,
   volume = 761,
      eid = {L3},
    pages = {L3},
      doi = {10.1088/2041-8205/761/1/L3},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...761L...3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Montesinos2016,
   author = {{Montesinos}, B. and {Eiroa}, C. and {Krivov}, A.~V. and {Marshall}, J.~P. and 
	{Pilbratt}, G.~L. and {Liseau}, R. and {Mora}, A. and {Maldonado}, J. and 
	{Wolf}, S. and {Ertel}, S. and {Bayo}, A. and {Augereau}, J.-C. and 
	{Heras}, A.~M. and {Fridlund}, M. and {Danchi}, W.~C. and {Solano}, E. and 
	{Kirchschlager}, F. and {del Burgo}, C. and {Montes}, D.},
    title = "{Incidence of debris discs around FGK stars in the solar neighbourhood}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1605.05837},
 primaryClass = "astro-ph.SR",
 keywords = {stars: late-type, circumstellar matter, protoplanetary disks, infrared: stars},
     year = 2016,
    month = sep,
   volume = 593,
      eid = {A51},
    pages = {A51},
      doi = {10.1051/0004-6361/201628329},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...593A..51M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Moor2006,
   author = {{Mo{\'o}r}, A. and {{\'A}brah{\'a}m}, P. and {Derekas}, A. and 
	{Kiss}, C. and {Kiss}, L.~L. and {Apai}, D. and {Grady}, C. and 
	{Henning}, T.},
    title = "{Nearby Debris Disk Systems with High Fractional Luminosity Reconsidered}",
  journal = {\apj},
     year = 2006,
    month = jun,
   volume = 644,
    pages = {525-542},
}

@ARTICLE{Moreno2003,
   author = {{Moreno}, F. and {Mu{\~n}oz}, O. and {Vilaplana}, R. and {Molina}, A.
	},
    title = "{Irregular Particles in Comet C/1995 O1 Hale-Bopp Inferred from its Mid-Infrared Spectrum}",
  journal = {\apj},
 keywords = {Comets: General, Comets: Individual: Name: Hale-Bopp (C/1995 O1), ISM: Dust, Extinction, Infrared: Solar System},
     year = 2003,
    month = sep,
   volume = 595,
    pages = {522-530},
      doi = {10.1086/377340},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...595..522M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mueller2010,
   author = {{M{\"u}ller}, S. and {L{\"o}hne}, T. and {Krivov}, A.~V.},
    title = "{The Debris Disk of Vega: A Steady-state Collisional Cascade, Naturally}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.1190},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, planetary systems: formation, radiation mechanisms: thermal, stars: individual: Vega},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {1728-1747},
      doi = {10.1088/0004-637X/708/2/1728},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708.1728M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Muinonen2002,
   author = {{Muinonen}, K. and {Piironen}, J. and {Shkuratov}, Y.~G. and 
	{Ovcharenko}, A. and {Clark}, B.~E.},
    title = "{Asteroid Photometric and Polarimetric Phase Effects}",
  journal = {Asteroids III},
     year = 2002,
    pages = {123-138},
   adsurl = {http://adsabs.harvard.edu/abs/2002aste.conf..123M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mukai1992,
   author = {{Mukai}, T. and {Ishimoto}, H. and {Kozasa}, T. and {Blum}, J. and 
	{Greenberg}, J.~M.},
    title = "{Radiation pressure forces of fluffy porous grains}",
  journal = {Annual Review of Astronomy {\&} Astrophysics},
     year = 1992,
    month = aug,
   volume = 262,
    pages = {315-320},
}


@ARTICLE{Mundt1984,
   author = {{Mundt}, R. and {Buehrke}, T. and {Fried}, J.~W. and {Neckel}, T. and 
	{Sarcander}, M. and {Stocke}, J.},
    title = "{Jets from young stars. III - The case of Haro 6-5B, HH 33/40, HH 19, and 1548C27}",
    journal = {\aap},
 keywords = {Early Stars, Herbig-Haro Objects, Jet Flow, Stellar Mass Ejection, Stellar Winds, T Tauri Stars, Emission Spectra, H Alpha Line, Line Spectra, Nebulae, Photographic Plates},
     year = 1984,
    month = nov,
   volume = 140,
    pages = {17-23},
   adsurl = {http://adsabs.harvard.edu/abs/1984A%26A...140...17M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Munoz2015,
   author = {{Mu{\~n}oz}, D.~J. and {Kratter}, K. and {Vogelsberger}, M. and 
	{Hernquist}, L. and {Springel}, V.},
    title = "{Stellar orbit evolution in close circumstellar disc encounters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1410.4561},
 primaryClass = "astro-ph.EP",
 keywords = {hydrodynamics, methods: numerical, planets and satellites: formation, protoplanetary discs, binaries: general},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {2010-2029},
      doi = {10.1093/mnras/stu2220},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.2010M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murakawa2010,
   author = {{Murakawa}, K.},
    title = "{Polarization disks in near-infrared high-resolution imaging}",
    journal = {\aap},
 keywords = {circumstellar matter, dust, extinction},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {A63},
    pages = {A63},
      doi = {10.1051/0004-6361/201014159},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518A..63M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mutschke1998,
   author = {{Mutschke}, H. and {Begemann}, B. and {Dorschner}, J. and {Guertler}, J. and 
	{Gustafson}, B. and {Henning}, T. and {Stognienko}, R.},
    title = "{Steps toward interstellar silicate mineralogy. III. The role of aluminium in circumstellar amorphous silicates}",
  journal = {\aap},
 keywords = {CIRCUMSTELLAR MATTER, STARS: AGB AND POST-AGB, STARS: VARIABLES: OTHER, INFRARED: STARS},
     year = 1998,
    month = may,
   volume = 333,
    pages = {188-198},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...333..188M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NajitaWilliams2005,
   author = {{Najita}, J. and {Williams}, J.~P.},
    title = "{An 850 {$\mu$}m Survey for Dust around Solar-Mass Stars}",
  journal = {\apj},
     year = 2005,
    month = dec,
   volume = 635,
    pages = {625-635},
}

@ARTICLE{Natta2007,
   author = {{Natta}, A. and {Testi}, L. and {Calvet}, N. and {Henning}, T. and 
	{Waters}, R. and {Wilner}, D.},
    title = "{Dust in Protoplanetary Disks: Properties and Evolution}",
  journal = {Protostars and Planets V},
   eprint = {arXiv:astro-ph/0602041},
     year = 2007,
    pages = {767-781},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..767N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nesvorny2010,
   author = {{Nesvorn{\'y}}, D. and {Jenniskens}, P. and {Levison}, H.~F. and
        {Bottke}, W.~F. and {Vokrouhlick{\'y}}, D. and {Gounelle}, M.
        },
    title = "{Cometary Origin of the Zodiacal Cloud and Carbonaceous Micrometeorites. Implications for Hot
Debris Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.4322},
 primaryClass = "astro-ph.EP",
 keywords = {comets: general, minor planets, asteroids: general, zodiacal dust},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {816-836},
      doi = {10.1088/0004-637X/713/2/816},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713..816N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Okuzumi2012,
   author = {{Okuzumi}, S. and {Tanaka}, H. and {Kobayashi}, H. and {Wada}, K.
	},
    title = "{Rapid Coagulation of Porous Dust Aggregates outside the Snow Line: A Pathway to Successful Icy Planetesimal Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.5035},
 primaryClass = "astro-ph.EP",
 keywords = {dust, extinction, planets and satellites: formation, protoplanetary disks},
     year = 2012,
    month = jun,
   volume = 752,
      eid = {106},
    pages = {106},
      doi = {10.1088/0004-637X/752/2/106},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...752..106O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{OLeary1967,
   author = {{O'Leary}, B.~T.},
    title = "{The Opposition Effect of Mars}",
  journal = {\apj},
     year = 1967,
    month = sep,
   volume = 149,
    pages = {L147},
      doi = {10.1086/180077},
   adsurl = {http://adsabs.harvard.edu/abs/1967ApJ...149L.147O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ormel2007,
   author = {{Ormel}, C.~W. and {Spaans}, M. and {Tielens}, A.~G.~G.~M.},
    title = "{Dust coagulation in protoplanetary disks: porosity matters}",
    journal = {\aap},
   eprint = {astro-ph/0610030},
 keywords = {ISM: dust, extinction, planetary systems: formation, planetary systems: protoplanetary disks, accretion, accretion disks},
     year = 2007,
    month = jan,
   volume = 461,
    pages = {215-232},
      doi = {10.1051/0004-6361:20065949},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...461..215O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ormel2008,
   author = {{Ormel}, C.~W. and {Cuzzi}, J.~N. and {Tielens}, A.~G.~G.~M.
	},
    title = "{Co-Accretion of Chondrules and Dust in the Solar Nebula}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0802.4048},
 keywords = {Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks, Solar System: Formation},
     year = 2008,
    month = jun,
   volume = 679,
    pages = {1588-1610},
      doi = {10.1086/587836},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...679.1588O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ossenkopf1991,
   author = {{Ossenkopf}, V.},
    title = "{Effective-medium theories for cosmic dust grains}",
journal={\aap},
     year = 1991,
    month = nov,
   volume = 251,
    pages = {210-219},
}

@ARTICLE{Osterloh1995,
   author = {{Osterloh}, M. and {Beckwith}, S.~V.~W.},
    title = "{Millimeter-wave continuum measurements of young stars}",
  journal = {\apj},
 keywords = {Accretion Disks, Binary Stars, Continuous Spectra, Millimeter Waves, Pre-Main Sequence Stars, Radio Observation, Thermal Radiation, Flux Density, H Alpha Line, Spectrum Analysis, Stellar Luminosity},
     year = 1995,
    month = jan,
   volume = 439,
    pages = {288-302},
      doi = {10.1086/175172},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...439..288O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Ott2010,
   author = {{Ott}, S.},
    title = "{The Herschel Data Processing System {\mdash} HIPE and Pipelines {\mdash} Up and Running Since the Start of the Mission}",
booktitle = {Astronomical Data Analysis Software and Systems XIX},
     year = 2010,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 434,
archivePrefix = "arXiv",
   eprint = {1011.1209},
 primaryClass = "astro-ph.IM",
   editor = {{Mizumoto}, Y. and {Morita}, K.-I. and {Ohishi}, M.},
    month = dec,
    pages = {139},
   adsurl = {http://adsabs.harvard.edu/abs/2010ASPC..434..139O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pace2013,
   author = {{Pace}, G.},
    title = "{Chromospheric activity as age indicator. An L-shaped chromospheric-activity versus age diagram}",
 journal={\aap},
 keywords = {stars: activity},
     year = 2013,
    month = mar,
   volume = 551,
      eid = {L8},
    pages = {L8},
      doi = {10.1051/0004-6361/201220364},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...551L...8P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Padgett1999,
   author = {{Padgett}, D.~L. and {Brandner}, W. and {Stapelfeldt}, K.~R. and 
	{Strom}, S.~E. and {Terebey}, S. and {Koerner}, D.},
    title = "{HUBBLE SPACE TELESCOPE/NICMOS Imaging of Disks and Envelopes around Very Young Stars}",
  journal = {The Astronomical Journal},
   eprint = {astro-ph/9902101},
 keywords = {STARS: CIRCUMSTELLAR MATTER, ISM: JETS AND OUTFLOWS, STARS: PRE-MAIN-SEQUENCE},
     year = 1999,
    month = mar,
   volume = 117,
    pages = {1490-1504},
      doi = {10.1086/300781},
   adsurl = {http://adsabs.harvard.edu/abs/1999AJ....117.1490P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pan2012,
   author = {{Pan}, M. and {Schlichting}, H.~E.},
    title = "{Self-consistent Size and Velocity Distributions of Collisional Cascades}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.0667},
 primaryClass = "astro-ph.EP",
 keywords = {Kuiper belt: general, minor planets, asteroids: general, planetary systems, protoplanetary disks},
     year = 2012,
    month = mar,
   volume = 747,
      eid = {113},
    pages = {113},
      doi = {10.1088/0004-637X/747/2/113},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...747..113P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pantin1997,
   author = {{Pantin}, E. and {Lagage}, P.~O. and {Artymowicz}, P.},
    title = "{Mid-infrared images and models of the beta Pictoris dust disk}",
  journal = {\aap},
 keywords = {STARS INDIVIDUAL: BETA PICTORIS, DUST, STARS: INFRARED, PLANETARY SYSTEMS},
     year = 1997,
    month = nov,
   volume = 327,
    pages = {1123-1136},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...327.1123P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pedersen2011,
   author = {{Pedersen}, A. and {G{\'o}mez de Castro}, A.~I.},
    title = "{Photoelectric Charging of Dust Grains in the Environment of Young Stellar Objects}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.3748},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, ISM: general, stars: variables: T Tauri, Herbig Ae/Be, ultraviolet: ISM},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/740/2/77},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740...77P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pepe2011,
   author = {{Pepe}, F. and {Lovis}, C. and {S{\'e}gransan}, D. and {Benz}, W. and 
	{Bouchy}, F. and {Dumusque}, X. and {Mayor}, M. and {Queloz}, D. and 
	{Santos}, N.~C. and {Udry}, S.},
    title = "{The HARPS search for Earth-like planets in the habitable zone. I. Very low-mass planets around <ASTROBJ>HD 20794</ASTROBJ>, <ASTROBJ>HD 85512</ASTROBJ>, and <ASTROBJ>HD 192310</ASTROBJ>}",
journal={\aap},
archivePrefix = "arXiv",
   eprint = {1108.3447},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, instrumentation: spectrographs, techniques: radial velocities, stars: individual: HD 20794, stars: individual: HD 85512, stars: individual: HD 192310},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A58},
    pages = {A58},
      doi = {10.1051/0004-6361/201117055},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A..58P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Perryman1997,
   author = {{Perryman}, M.~A.~C. and {Lindegren}, L. and {Kovalevsky}, J. and 
	{Hoeg}, E. and {Bastian}, U. and {Bernacca}, P.~L. and {Cr{\'e}z{\'e}}, M. and 
	{Donati}, F. and {Grenon}, M. and {van Leeuwen}, F. and {van der Marel}, H. and 
	{Mignard}, F. and {Murray}, C.~A. and {Le Poole}, R.~S. and 
	{Schrijver}, H. and {Turon}, C. and {Arenou}, F. and {Froeschl{\'e}}, M. and 
	{Petersen}, C.~S.},
    title = "{The HIPPARCOS Catalogue}",
  journal = {\aap},
     year = 1997,
    month = jul,
   volume = 323,
    pages = {L49-L52}
}

@ARTICLE{Peterson2006,
   author = {{Peterson}, D.~M. and {Hummel}, C.~A. and {Pauls}, T.~A. and 
	{Armstrong}, J.~T. and {Benson}, J.~A. and {Gilbreath}, G.~C. and 
	{Hindsley}, R.~B. and {Hutter}, D.~J. and {Johnston}, K.~J. and 
	{Mozurkewich}, D. and {Schmitt}, H.~R.},
    title = "{Vega is a rapidly rotating star}",
  journal = {Nature},
   eprint = {astro-ph/0603520},
     year = 2006,
    month = apr,
   volume = 440,
    pages = {896-899},
      doi = {10.1038/nature04661},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.440..896P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Pety2006,
   author = {{Pety}, J. and {Gueth}, F. and {Guilloteau}, S. and {Dutrey}, A.
	},
    title = "{Plateau de Bure interferometer observations of the disk and outflow of HH 30}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0608218},
 keywords = {stars: individual: HH30, stars: formation, stars: circumstellar, matter, ISM: dust, extinction, ISM: molecules, ISM: jets and outflows},
     year = 2006,
    month = nov,
   volume = 458,
    pages = {841-854},
      doi = {10.1051/0004-6361:20065814},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...458..841P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pfalzner2005,
   author = {{Pfalzner}, S. and {Umbreit}, S. and {Henning}, T.},
    title = "{Disk-Disk Encounters between Low-Mass Protoplanetary Accretion Disks}",
  journal = {\apj},
   eprint = {astro-ph/0504590},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {526-534},
      doi = {10.1086/431350},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..526P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pilbratt2010,
   author = {{Pilbratt}, G.~L. and {Riedinger}, J.~R. and {Passvogel}, T. and 
	{Crone}, G. and {Doyle}, D. and {Gageur}, U. and {Heras}, A.~M. and 
	{Jewell}, C. and {Metcalfe}, L. and {Ott}, S. and {Schmidt}, M.
	},
    title = "{Herschel Space Observatory. An ESA facility for far-infrared and submillimetre astronomy}",
  journal = {\aap},,
archivePrefix = "arXiv",
   eprint = {1005.5331},
 primaryClass = "astro-ph.IM",
 keywords = {space vehicles, space vehicles: instruments, infrared: general, submillimetre: general},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L1},
    pages = {L1},
      doi = {10.1051/0004-6361/201014759},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pinte2008,
   author = {{Pinte}, C. and {Padgett}, D.~L. and {M{\'e}nard}, F. and {Stapelfeldt}, K.~R. and 
	{Schneider}, G. and {Olofsson}, J. and {Pani{\'c}}, O. and {Augereau}, J.~C. and 
	{Duch{\^e}ne}, G. and {Krist}, J. and {Pontoppidan}, K. and 
	{Perrin}, M.~D. and {Grady}, C.~A. and {Kessler-Silacci}, J. and 
	{van Dishoeck}, E.~F. and {Lommen}, D. and {Silverstone}, M. and 
	{Hines}, D.~C. and {Wolf}, S. and {Blake}, G.~A. and {Henning}, T. and 
	{Stecklum}, B.},
    title = "{Probing dust grain evolution in IM Lupi's circumstellar disc. Multi-wavelength observations and modelling of the dust disc}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0808.0619},
 keywords = {circumstellar matter, accretion, accretion disks, planetary systems: protoplanetary disks, radiative transfer, stars: formation, pulsars: individual: IM , Lupi},
     year = 2008,
    month = oct,
   volume = 489,
    pages = {633-650},
      doi = {10.1051/0004-6361:200810121},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489..633P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Plavchan2009,
   author = {{Plavchan}, P. and {Werner}, M.~W. and {Chen}, C.~H. and {Stapelfeldt}, K.~R. and 
	{Su}, K.~Y.~L. and {Stauffer}, J.~R. and {Song}, I.},
    title = "{New Debris Disks Around Young, Low-Mass Stars Discovered with the Spitzer Space Telescope}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.0819},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, planetary systems: formation},
     year = 2009,
    month = jun,
   volume = 698,
    pages = {1068-1094},
      doi = {10.1088/0004-637X/698/2/1068},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...698.1068P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Podio2012,
   author = {{Podio}, L. and {Kamp}, I. and {Flower}, D. and {Howard}, C. and 
	{Sandell}, G. and {Mora}, A. and {Aresu}, G. and {Brittain}, S. and 
	{Dent}, W.~R.~F. and {Pinte}, C. and {White}, G.~J.},
    title = "{Herschel/PACS observations of young sources in Taurus: the far-infrared counterpart of optical jets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1207.3435},
 primaryClass = "astro-ph.SR",
 keywords = {astrochemistry, stars: formation, ISM: jets and outflows, ISM: molecules, ISM: general},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A44},
    pages = {A44},
      doi = {10.1051/0004-6361/201219475},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A..44P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Poglitsch2010,
   author = {{Poglitsch}, A. and {Waelkens}, C. and {Geis}, N. and {Feuchtgruber}, H. and 
	{Vandenbussche}, B. and {Rodriguez}, L. and {Krause}, O. and 
	{Renotte}, E. and {van Hoof}, C. and {Saraceno}, P. and {Cepa}, J. and 
	{Kerschbaum}, F. and {Agn{\`e}se}, P. and {Ali}, B. and {Altieri}, B. and 
	{Andreani}, P. and {Augueres}, J.-L. and {Balog}, Z. and {Barl}, L. and 
	{Bauer}, O.~H. and {Belbachir}, N. and {Benedettini}, M. and 
	{Billot}, N. and {Boulade}, O. and {Bischof}, H. and {Blommaert}, J. and 
	{Callut}, E. and {Cara}, C. and {Cerulli}, R. and {Cesarsky}, D. and 
	{Contursi}, A. and {Creten}, Y. and {De Meester}, W. and {Doublier}, V. and 
	{Doumayrou}, E. and {Duband}, L. and {Exter}, K. and {Genzel}, R. and 
	{Gillis}, J.-M. and {Gr{\"o}zinger}, U. and {Henning}, T. and 
	{Herreros}, J. and {Huygen}, R. and {Inguscio}, M. and {Jakob}, G. and 
	{Jamar}, C. and {Jean}, C. and {de Jong}, J. and {Katterloher}, R. and 
	{Kiss}, C. and {Klaas}, U. and {Lemke}, D. and {Lutz}, D. and 
	{Madden}, S. and {Marquet}, B. and {Martignac}, J. and {Mazy}, A. and 
	{Merken}, P. and {Montfort}, F. and {Morbidelli}, L. and {M{\"u}ller}, T. and 
	{Nielbock}, M. and {Okumura}, K. and {Orfei}, R. and {Ottensamer}, R. and 
	{Pezzuto}, S. and {Popesso}, P. and {Putzeys}, J. and {Regibo}, S. and 
	{Reveret}, V. and {Royer}, P. and {Sauvage}, M. and {Schreiber}, J. and 
	{Stegmaier}, J. and {Schmitt}, D. and {Schubert}, J. and {Sturm}, E. and 
	{Thiel}, M. and {Tofani}, G. and {Vavrek}, R. and {Wetzstein}, M. and 
	{Wieprecht}, E. and {Wiezorrek}, E.},
    title = "{The Photodetector Array Camera and Spectrometer (PACS) on the Herschel Space Observatory}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.1487},
 primaryClass = "astro-ph.IM",
 keywords = {space vehicles: instruments, instrumentation: photometers, instrumentation: spectrographs},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201014535},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L...2P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Poynting1903,
   author = {{Poynting}, J.~H.},
    title = "{Radiation in the solar system : its effect on temperature and its pressure on small bodies}",
  journal = {\mnras},
     year = 1903,
    month = nov,
   volume = 64,
    pages = {A1},
   adsurl = {http://adsabs.harvard.edu/abs/1903MNRAS..64A...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@book{Press2007,
 author = {Press, William H. and Teukolsky, Saul A. and Vetterling, William T. and Flannery, Brian P.},
 title = {Numerical Recipes 3rd Edition: The Art of Scientific Computing},
 year = {2007},
 edition = {3},
 publisher = {Cambridge University Press},
} 

@book{Purcell1965,
  title={Berkeley Physics Course: Electricity and magnetism},
  author={Purcell, E.~M.},
  series={Berkeley Physics Course},
  volume = 2,
  year={1965},
  publisher={New York: McGraw-Hill}
}


@ARTICLE{PurcellPenny1973,
   author = {{Purcell}, E.~M. and {Pennypacker}, C.~R.},
    title = "{Scattering and Absorption of Light by Nonspherical Dielectric Grains}",
  journal = {\apj},
     year = 1973,
    month = dec,
   volume = 186,
    pages = {705-714},
      doi = {10.1086/152538},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...186..705P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quanz2011,
   author = {{Quanz}, S.~P. and {Schmid}, H.~M. and {Geissler}, K. and {Meyer}, M.~R. and 
	{Henning}, T. and {Brandner}, W. and {Wolf}, S.},
    title = "{Very Large Telescope/NACO Polarimetric Differential Imaging of HD100546{\mdash}Disk Structure and Dust Grain Properties between 10 and 140 AU}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.1101},
 primaryClass = "astro-ph.GA",
 keywords = {protoplanetary disks, stars: formation, stars: pre-main sequence},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {23},
    pages = {23},
      doi = {10.1088/0004-637X/738/1/23},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738...23Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Rawlings2001,
   author = {{Rawlings}, J.~M.~C. and {Yates}, J.~A.},
    title = "{Modelling line profiles in infalling cores}",
  journal = {\mnras},
 keywords = {line: profiles, radiative transfer, stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: molecules},
     year = 2001,
    month = oct,
   volume = 326,
    pages = {1423-1430},
      doi = {10.1111/j.1365-8711.2001.04674.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.326.1423R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Reipurth1993,
   author = {{Reipurth}, B. and {Chini}, R. and {Krugel}, E. and {Kreysa}, E. and 
	{Sievers}, A.},
    title = "{Cold Dust around Herbig-Haro Energy Sources - a 1300-MICRON Survey}",
    journal ={\aap},
 keywords = {interstellar medium: jets and outflows, radio continuum: stars, circumstellar matter, stars: formation of, stars: pre-main sequence},
     year = 1993,
    month = jun,
   volume = 273,
    pages = {221},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...273..221R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ricci2012,
   author = {{Ricci}, L. and {Trotta}, F. and {Testi}, L. and {Natta}, A. and 
	{Isella}, A. and {Wilner}, D.~J.},
    title = "{The effect of local optically thick regions in the long-wave emission of young circumstellar disks}",
    journal = {\aap},
     year = 2012,
    month = apr,
   volume = 540,
    pages = {A6},
}

@ARTICLE{Ricci2010,
   author = {{Ricci}, L. and {Testi}, L. and {Natta}, A. and {Neri}, R. and 
	{Cabrit}, S. and {Herczeg}, G.~J.},
    title = "{Dust properties of protoplanetary disks in the Taurus-Auriga star forming region from millimeter wavelengths}",
    journal = {\aap},
     year = 2010,
    month = mar,
   volume = 512,
      eid = {A15},
    pages = {A15},
}

@ARTICLE{Rieke2005,
   author = {{Rieke}, G.~H. and {Su}, K.~Y.~L. and {Stansberry}, J.~A. and 
	{Trilling}, D. and {Bryden}, G. and {Muzerolle}, J. and {White}, B. and 
	{Gorlova}, N. and {Young}, E.~T. and {Beichman}, C.~A. and {Stapelfeldt}, K.~R. and 
	{Hines}, D.~C.},
    title = "{Decay of Planetary Debris Disks}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Planetary Systems: Formation},
     year = 2005,
    month = feb,
   volume = 620,
    pages = {1010-1026},
      doi = {10.1086/426937},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...620.1010R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Rieke2016,
   author = {{Rieke}, G.~H. and {G{\'a}sp{\'a}r}, A. and {Ballering}, N.~P.
	},
    title = "{Magnetic Grain Trapping and the Hot Excesses around Early-type Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.04998},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, infrared: planetary systems, methods: numerical},
     year = 2016,
    month = jan,
   volume = 816,
      eid = {50},
    pages = {50},
      doi = {10.3847/0004-637X/816/2/50},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...816...50R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roberge2012,
   author = {{Roberge}, A. and {Chen}, C.~H. and {Millan-Gabet}, R. and {Weinberger}, A.~J. and 
	{Hinz}, P.~M. and {Stapelfeldt}, K.~R. and {Absil}, O. and {Kuchner}, M.~J. and 
	{Bryden}, G.},
    title = "{The Exozodiacal Dust Problem for Direct Observations of Exo-Earths}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1204.0025},
 primaryClass = "astro-ph.EP",
     year = 2012,
    month = aug,
   volume = 124,
    pages = {799-808},
      doi = {10.1086/667218},
   adsurl = {http://adsabs.harvard.edu/abs/2012PASP..124..799R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Roberge2013,
   author = {{Roberge}, A. and {Kamp}, I. and {Montesinos}, B. and {Dent}, W.~R.~F. and 
	{Meeus}, G. and {Donaldson}, J.~K. and {Olofsson}, J. and {Mo{\'o}r}, A. and 
	{Augereau}, J.-C. and {Howard}, C. and {Eiroa}, C. and {Thi}, W.-F. and 
	{Ardila}, D.~R. and {Sandell}, G. and {Woitke}, P.},
    title = "{Herschel Observations of Gas and Dust in the Unusual 49 Ceti Debris Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.2894},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, Kuiper belt: general, protoplanetary disks, stars: individual: 49 Ceti},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {69},
    pages = {69},
      doi = {10.1088/0004-637X/771/1/69},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...69R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Robertson1937,
   author = {{Robertson}, H.~P.},
    title = "{Dynamical effects of radiation in the solar system}",
  journal = {\mnras},
     year = 1937,
    month = apr,
   volume = 97,
    pages = {423},
   adsurl = {http://adsabs.harvard.edu/abs/1937MNRAS..97..423R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Robitaille2007,
   author = {{Robitaille}, T.~P. and {Whitney}, B.~A. and {Indebetouw}, R. and 
	{Wood}, K.},
    title = "{Interpreting Spectral Energy Distributions from Young Stellar Objects. II. Fitting Observed SEDs Using a Large Grid of Precomputed Models}",
  journal = {\apjs},
   eprint = {astro-ph/0612690},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Radiative Transfer, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2007,
    month = apr,
   volume = 169,
    pages = {328-352},
      doi = {10.1086/512039},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..169..328R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Roccatagliata2009,
author = {{Roccatagliata}, V. and {Henning}, T. and {Wolf}, S. and {Rodmann}, J. and 
	{Corder}, S. and {Carpenter}, J.~M. and {Meyer}, M.~R. and {Dowell}, D.
	},
    title = "{Long-wavelength observations of debris discs around sun-like stars}",
  journal = {\aap},
     year = 2009,
    month = apr,
   volume = 497,
    pages = {409-421},
}

@phdthesis{Rodmann,
author = {{Rodmann}, J.},
    title = "{Dust in circumstellar disks}",
school={Combined Faculties for the Natural Sciences and for Mathematics of the Ruperto-Carola University of Heidelberg, Germany},
     year = 2006,
    month = feb,
}

@ARTICLE{Rouleau1991,
   author = {{Rouleau}, F. and {Martin}, P.~G.},
    title = "{Shape and clustering effects on the optical properties of amorphous carbon}",
  journal = {\apj},
     year = 1991,
    month = aug,
   volume = 377,
    pages = {526-540},
}

@INPROCEEDINGS{Rousset2003,
   author = {{Rousset}, G. and {Lacombe}, F. and {Puget}, P. and {Hubin}, N.~N. and 
	{Gendron}, E. and {Fusco}, T. and {Arsenault}, R. and {Charton}, J. and 
	{Feautrier}, P. and {Gigan}, P. and {Kern}, P.~Y. and {Lagrange}, A.-M. and 
	{Madec}, P.-Y. and {Mouillet}, D. and {Rabaud}, D. and {Rabou}, P. and 
	{Stadler}, E. and {Zins}, G.},
    title = "{NAOS, the first AO system of the VLT: on-sky performance}",
booktitle = {Adaptive Optical System Technologies II},
     year = 2003,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4839,
   editor = {{Wizinowich}, P.~L. and {Bonaccini}, D.},
    month = feb,
    pages = {140-149},
      doi = {10.1117/12.459332},
   adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4839..140R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Rosenbush2002,
   author = {{Rosenbush}, V. and {Kiselev}, N. and {Avramchuk}, V. and {Mishchenko}, M.
	},
    title = "{Photometric and Polarimetric Opposition Phenomena Exhibited by Solar System Bodies}",
booktitle = {Optics of Cosmic Dust},
     year = 2002,
   editor = {{Videen}, G. and {Kocifaj}, M.},
    pages = {191},
   adsurl = {http://adsabs.harvard.edu/abs/2002ocd..conf..191R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rosenbush2006,
   author = {{Rosenbush}, V. and {Kiselev}, N. and {Avramchuk}, V.},
    title = "{Similarity and diversity in photometric and polarimetric opposition effects of small Solar System bodies}",
  journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
     year = 2006,
    month = jul,
   volume = 100,
    pages = {325-339},
      doi = {10.1016/j.jqsrt.2005.11.049},
   adsurl = {http://adsabs.harvard.edu/abs/2006JQSRT.100..325R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Santos2004,
   author = {{Santos}, N.~C. and {Israelian}, G. and {Mayor}, M.},
    title = "{Spectroscopic [Fe/H] for 98 extra-solar planet-host stars.  Exploring the probability of planet formation}",
    journal = {\aap},
   eprint = {astro-ph/0311541},
 keywords = {stars: abundances, stars: fundamental parameters, stars: planetary systems, stars: planetary systems: formation, stars: chemically peculiar},
     year = 2004,
    month = mar,
   volume = 415,
    pages = {1153-1166},
      doi = {10.1051/0004-6361:20034469},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...415.1153S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sauter2009,
   author = {{Sauter}, J. and {Wolf}, S. and {Launhardt}, R. and {Padgett}, D.~L. and 
	{Stapelfeldt}, K.~R. and {Pinte}, C. and {Duch{\^e}ne}, G. and 
	{M{\'e}nard}, F. and {McCabe}, C.-E. and {Pontoppidan}, K. and 
	{Dunham}, M. and {Bourke}, T.~L. and {Chen}, J.-H.},
    title = "{The circumstellar disc in the Bok globule CB 26. Multi-wavelength observations and modelling of the dust disc and envelope}",
    journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1074},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, planetary systems: protoplanetary disks, radiative transfer, stars: formation, stars: individual: CB 26},
     year = 2009,
    month = oct,
   volume = 505,
    pages = {1167-1182},
      doi = {10.1051/0004-6361/200912397},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...505.1167S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Scally2001,
   author = {{Scally}, A. and {Clarke}, C.},
    title = "{Destruction of protoplanetary discs in the Orion Nebula Cluster}",
  journal = {\mnras},
   eprint = {astro-ph/0012098},
 keywords = {ACCRETION, ACCRETION DISCS, STELLAR DYNAMICS, SOLAR SYSTEM: FORMATION, PLANETARY SYSTEMS, OPEN CLUSTERS AND ASSOCIATIONS: INDIVIDUAL: ORION NEBULA CLUSTER},
     year = 2001,
    month = aug,
   volume = 325,
    pages = {449-456},
      doi = {10.1046/j.1365-8711.2001.04274.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.325..449S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SchmidtKaler,
   author = {{Schmidt-Kaler}, Th.},
    title = "{Interplanetry Dust and the Zodiacal Cloud}",
  journal = {Landolt-Bornstein Numerical Data and Functional Relationships and Technology},
     year = 1982,
   volume = 2,
}

@ARTICLE{Seeliger1893,
   author = {{Seeliger}, H.},
    title = "{Theorie der Beleuchtung staubförmiger kosmischer Massen insbesondere des S a t u r n r i n g e s }",
  journal = {Abhandlungen der mathematisch-physikalischen Classe der königlich bayerischen Akademie der Wissenschaften},
     year = 1893,
   volume = 18
}

@ARTICLE{Semenov2003,
   author = {{Semenov}, D. and {Henning}, T. and {Helling}, C. and {Ilgner}, M. and 
	{Sedlmayr}, E.},
    title = "{Rosseland and Planck mean opacities for protoplanetary discs}",
    journal = {\aap},
   eprint = {astro-ph/0308344},
 keywords = {accretion, accretion discs, hydrodynamics, atomic processes, molecular processes, stars: planetary systems: protoplanetary discs},
     year = 2003,
    month = nov,
   volume = 410,
    pages = {611-621},
      doi = {10.1051/0004-6361:20031279},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...410..611S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ShakuraSunyaev1973,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{Black holes in binary systems. Observational appearance.}",
    journal = {\aap},
     year = 1973,
   volume = 24,
    pages = {337-355},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shu1987,
   author = {{Shu}, F.~H. and {Adams}, F.~C. and {Lizano}, S.},
    title = "{Star formation in molecular clouds - Observation and theory}",
  journal = {Annual review of astronomy and astrophysics},
 keywords = {ASTROPHYSICS, MOLECULAR CLOUDS, STAR FORMATION, STELLAR MODELS, ASTRONOMICAL MAPS, BINARY STARS, GRAVITATIONAL COLLAPSE, PROTOSTARS, STAR CLUSTERS, STELLAR MASS},
     year = 1987,
   volume = 25,
    pages = {23-81},
      doi = {10.1146/annurev.aa.25.090187.000323},
   adsurl = {http://adsabs.harvard.edu/abs/1987ARA%26A..25...23S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Siebenmorgen2012,
   author = {{Siebenmorgen}, R. and {Heymann}, F.},
    title = "{Shadows, gaps, and ring-like structures in protoplanetary disks}",
  journal = {\aap},,
archivePrefix = "arXiv",
   eprint = {1201.3577},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, protoplanetary disks, dust, extinction},
     year = 2012,
    month = mar,
   volume = 539,
      eid = {A20},
    pages = {A20},
      doi = {10.1051/0004-6361/201118493},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A..20S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Siess2000,
   author = {{Siess}, L. and {Dufour}, E. and {Forestini}, M.},
    title = "{An internet server for pre-main sequence tracks of low- and intermediate-mass stars}",
  journal = {\aap},
   eprint = {astro-ph/0003477},
 keywords = {EQUATION OF STATE, STARS: EVOLUTION, STARS: HERTZSPRUNG-RUSSEL (HR) AND C-M DIAGRAMS, STARS: PRE-MAIN SEQUENCE, ASTRONOMICAL DATA BASES: MISCELLANEOUS},
     year = 2000,
    month = jun,
   volume = 358,
    pages = {593-599},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...358..593S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Simon1992,
   author = {{Simon}, M. and {Chen}, W.~P. and {Howell}, R.~R. and {Benson}, J.~A. and 
	{Slowik}, D.},
    title = "{Multiplicity among the young stars in Taurus}",
  journal = {\apj},
 keywords = {Binary Stars, Early Stars, Star Formation, Stellar Systems, Infrared Astronomy, Occultation, Pre-Main Sequence Stars},
     year = 1992,
    month = jan,
   volume = 384,
    pages = {212-219},
      doi = {10.1086/170864},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...384..212S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Simmons1982,
   author = {{Simmons}, J.~F.~L.},
    title = "{Analytic treatment of polarization by arbitrary scattering mechanisms in circumstellar envelopes. I - Single stars}",
  journal = {\mnras},
 keywords = {DENSITY DISTRIBUTION, LIGHT SCATTERING, MIE SCATTERING, POLARIZED LIGHT, STELLAR ENVELOPES, STOKES LAW OF RADIATION, INTERSTELLAR EXTINCTION, PARTICLE SIZE DISTRIBUTION, RAYLEIGH SCATTERING, REFRACTIVITY, THOMSON SCATTERING},
     year = 1982,
    month = jul,
   volume = 200,
    pages = {91-113},
   adsurl = {http://adsabs.harvard.edu/abs/1982MNRAS.200...91S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skrutskie1990,
   author = {{Skrutskie}, M.~F. and {Dutkevitch}, D. and {Strom}, S.~E. and 
	{Edwards}, S. and {Strom}, K.~M. and {Shure}, M.~A.},
    title = "{A sensitive 10-micron search for emission arising from circumstellar dust associated with solar-type pre-main-sequence stars}",
  journal = {Astronomical Journal},
 keywords = {Cosmic Dust, Emission Spectra, Infrared Astronomy, Pre-Main Sequence Stars, Stellar Envelopes, H Alpha Line, Optical Thickness, Photosphere, Spectral Energy Distribution, Spectral Line Width, Stellar Evolution},
     year = 1990,
    month = apr,
   volume = 99,
    pages = {1187-1195},
      doi = {10.1086/115407},
   adsurl = {http://adsabs.harvard.edu/abs/1990AJ.....99.1187S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Skrutskie2006,
   author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and 
	{Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and 
	{Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and 
	{Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and 
	{Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and 
	{Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and 
	{Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and 
	{Wheelock}, S.},
    title = "{The Two Micron All Sky Survey (2MASS)}",
  journal = {The Astronomical Journal},
 keywords = {Catalogs, Infrared: General, Surveys},
     year = 2006,
    month = feb,
   volume = 131,
    pages = {1163-1183},
      doi = {10.1086/498708},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1163S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Smith1984,
   author = {{Smith}, B.~A. and {Terrile}, R.~J.},
    title = "{A circumstellar disk around Beta Pictoris}",
  journal = {Science},
     year = 1984,
    month = dec,
   volume = 226,
    pages = {1421-1424},
}

@ARTICLE{Sousa2008,
   author = {{Sousa}, S.~G. and {Santos}, N.~C. and {Mayor}, M. and {Udry}, S. and 
	{Casagrande}, L. and {Israelian}, G. and {Pepe}, F. and {Queloz}, D. and 
	{Monteiro}, M.~J.~P.~F.~G.},
    title = "{Spectroscopic parameters for 451 stars in the HARPS GTO planet search program. Stellar [Fe/H] and the frequency of exo-Neptunes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0805.4826},
 keywords = {methods: data analysis, techniques: spectroscopic, stars: fundamental parameters, stars: planetary systems, stars: planetary systems: formation, Galaxy: solar neighborhood},
     year = 2008,
    month = aug,
   volume = 487,
    pages = {373-381},
      doi = {10.1051/0004-6361:200809698},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487..373S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stapelfeldt1998,
   author = {{Stapelfeldt}, K.~R. and {Krist}, J.~E. and {Menard}, F. and 
	{Bouvier}, J. and {Padgett}, D.~L. and {Burrows}, C.~J.},
    title = "{An Edge-On Circumstellar Disk in the Young Binary System HK Tauri}",
  journal = {Astrophysical Journal Letters},
 keywords = {STARS: BINARIES: GENERAL, STARS: INDIVIDUAL CONSTELLATION NAME: HK TAURI, STARS: CIRCUMSTELLAR MATTER, STARS: PRE-MAIN-SEQUENCE},
     year = 1998,
    month = jul,
   volume = 502,
    pages = {L65},
      doi = {10.1086/311479},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...502L..65S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stapelfeldt2003,
   author = {{Stapelfeldt}, K.~R. and {M{\'e}nard}, F. and {Watson}, A.~M. and 
	{Krist}, J.~E. and {Dougados}, C. and {Padgett}, D.~L. and {Brandner}, W.
	},
    title = "{Hubble Space Telescope WFPC2 Imaging of the Disk and Jet of HV Tauri C}",
  journal = {\apj},
 keywords = {Stars: Binaries: General, Stars: Circumstellar Matter, Stars: Individual: Constellation Name: HV Tauri, Stars: Pre-Main-Sequence},
     year = 2003,
    month = may,
   volume = 589,
    pages = {410-418},
      doi = {10.1086/374374},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...589..410S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stapelfeldt2004,
   author = {{Stapelfeldt}, K.~R. and {Holmes}, E.~K. and {Chen}, C. and 
	{Rieke}, G.~H. and {Su}, K.~Y.~L. and {Hines}, D.~C. and {Werner}, M.~W. and 
	{Beichman}, C.~A. and {Jura}, M. and {Padgett}, D.~L. and {Stansberry}, J.~A. and 
	{Bendo}, G. and {Cadien}, J. and {Marengo}, M. and {Thompson}, T. and 
	{Velusamy}, T. and {Backus}, C. and {Blaylock}, M. and {Egami}, E. and 
	{Engelbracht}, C.~W. and {Frayer}, D.~T. and {Gordon}, K.~D. and 
	{Keene}, J. and {Latter}, W.~B. and {Megeath}, T. and {Misselt}, K. and 
	{Morrison}, J.~E. and {Muzerolle}, J. and {Noriega-Crespo}, A. and 
	{Van Cleve}, J. and {Young}, E.~T.},
    title = "{First Look at the Fomalhaut Debris Disk with the Spitzer Space Telescope}",
  journal = {\apjs},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Planetary Systems, Stars: Individual: Name: Fomalhaut},
     year = 2004,
    month = sep,
   volume = 154,
    pages = {458-462},
      doi = {10.1086/423135},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154..458S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stark2006,
   author = {{Stark}, D.~P. and {Whitney}, B.~A. and {Stassun}, K. and {Wood}, K.
	},
    title = "{Near-Infrared Synthetic Images of Protostellar Disks and Envelopes}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Radiative Transfer, Scattering, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2006,
    month = oct,
   volume = 649,
    pages = {900-913},
      doi = {10.1086/506926},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649..900S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stock2010,
   author = {{Stock}, N.~D. and {Su}, K.~Y.~L. and {Liu}, W. and {Hinz}, P.~M. and 
	{Rieke}, G.~H. and {Marengo}, M. and {Stapelfeldt}, K.~R. and 
	{Hines}, D.~C. and {Trilling}, D.~E.},
    title = "{The Structure of the {$\beta$} Leonis Debris Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1010.0003},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, infrared: stars, planetary systems, stars: individual: {$\beta$} Leo o Leo, techniques: interferometric},
     year = 2010,
    month = dec,
   volume = 724,
    pages = {1238-1255},
      doi = {10.1088/0004-637X/724/2/1238},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...724.1238S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Stokes1852,
   author = {{Stokes}, G.~G.},
    title = "{On the Change of Refrangibility of Light}",
  journal = {Royal Society of London Philosophical Transactions Series I},
     year = 1852,
   volume = 142,
    pages = {463-562},
   adsurl = {http://adsabs.harvard.edu/abs/1852RSPT..142..463S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Strom1989,
   author = {{Strom}, K.~M. and {Strom}, S.~E. and {Edwards}, S. and {Cabrit}, S. and 
	{Skrutskie}, M.~F.},
    title = "{Circumstellar material associated with solar-type pre-main-sequence stars - A possible constraint on the timescale for planet building}",
  journal = {Astronomical Journal},
 keywords = {Pre-Main Sequence Stars, Stellar Envelopes, Stellar Spectrophotometry, T Tauri Stars, Frequency Distribution, H Alpha Line, Infrared Spectra, Spectral Energy Distribution, Star Formation},
     year = 1989,
    month = may,
   volume = 97,
    pages = {1451-1470},
      doi = {10.1086/115085},
   adsurl = {http://adsabs.harvard.edu/abs/1989AJ.....97.1451S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Strom1993,
   author = {{Strom}, S.~E. and {Edwards}, S. and {Skrutskie}, M.~F.},
    title = "{Evolutionary time scales for circumstellar disks associated with intermediate- and solar-type stars}",
 keywords = {Accretion Disks, Pre-Main Sequence Stars, Star Formation, Stellar Envelopes, Stellar Evolution, Spectral Energy Distribution, Stellar Physics, Time Response},
booktitle = {Protostars and Planets III},
     year = 1993,
   editor = {{Levy}, E.~H. and {Lunine}, J.~I.},
    pages = {837-866},
   adsurl = {http://adsabs.harvard.edu/abs/1993prpl.conf..837S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Strubbe2006,
   author = {{Strubbe}, L.~E. and {Chiang}, E.~I.},
    title = "{Dust Dynamics, Surface Brightness Profiles, and Thermal Spectra of Debris Disks: The Case of AU Microscopii}",
  journal = {\apj},
     year = 2006,
    month = sep,
   volume = 648,
    pages = {652-665},
}

@ARTICLE{Su2006,
 author = {{Su}, K.~Y.~L. and {Rieke}, G.~H. and {Stansberry}, J.~A. and 
	{Bryden}, G. and {Stapelfeldt}, K.~R. and {Trilling}, D.~E. and 
	{Muzerolle}, J. and {Beichman}, C.~A. and {Moro-Martin}, A. and 
	{Hines}, D.~C. and {Werner}, M.~W.},
    title = "{Debris Disk Evolution around A Stars}",
  journal = {\apj},
   eprint = {astro-ph/0608563},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Planetary Systems: Formation},
     year = 2006,
    month = dec,
   volume = 653,
    pages = {675-689},
      doi = {10.1086/508649},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653..675S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Su2013,
   author = {{Su}, K.~Y.~L. and {Rieke}, G.~H. and {Malhotra}, R. and {Stapelfeldt}, K.~R. and 
	{Hughes}, A.~M. and {Bonsor}, A. and {Wilner}, D.~J. and {Balog}, Z. and 
	{Watson}, D.~M. and {Werner}, M.~W. and {Misselt}, K.~A.},
    title = "{Asteroid Belts in Debris Disk Twins: Vega and Fomalhaut}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.1331},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, infrared: stars, planetary systems, stars: individual: Vega Fomalhaut},
     year = 2013,
    month = feb,
   volume = 763,
      eid = {118},
    pages = {118},
      doi = {10.1088/0004-637X/763/2/118},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763..118S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Takeda2005,
   author = {{Takeda}, Y. and {Ohkubo}, M. and {Sato}, B. and {Kambe}, E. and 
	{Sadakane}, K.},
    title = "{Spectroscopic Study on the Atmospheric Parameters of Nearby F--K Dwarfs and Subgiants}",
  journal = {Publications of the Astronomical Society of Japan},
 keywords = {stars: abundances, stars: atmospheres, stars: fundamental parameters, stars: late-type},
     year = 2005,
    month = feb,
   volume = 57,
    pages = {27-43},
      doi = {10.1093/pasj/57.1.27},
   adsurl = {http://adsabs.harvard.edu/abs/2005PASJ...57...27T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tamazian2002,
   author = {{Tamazian}, V.~S. and {Docobo}, J.~A. and {White}, R.~J. and 
	{Woitas}, J.},
    title = "{Preliminary Orbits and System Masses for Five Binary T Tauri Stars}",
  journal = {\apj},
 keywords = {Astrometry, Stars: Binaries: General, Celestial Mechanics, Stars: Individual: Constellation Name: V773 Tauri, stars: individual (FO Tauri, FS Tauri), Stars: Individual: Constellation Name: DF Tauri, Stars: Individual: Constellation Name: GG Tauri, Stars: Pre-Main-Sequence},
     year = 2002,
    month = oct,
   volume = 578,
    pages = {925-934},
      doi = {10.1086/342621},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...578..925T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tambovtseva2006,
   author = {{Tambovtseva}, L.~V. and {Grinin}, V.~P. and {Weigelt}, G.},
    title = "{Moving shadows on the dusty disks of young stars}",
  journal = {\aap},
 keywords = {accretion, accretion disks, stars: formation, binaries: close, circumstellar matter, stars: pre-main sequence},
     year = 2006,
    month = mar,
   volume = 448,
    pages = {633-639},
      doi = {10.1051/0004-6361:20053884},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...448..633T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tamura1999,
   author = {{Tamura}, M. and {Hough}, J.~H. and {Greaves}, J.~S. and {Morino}, J.-I. and 
	{Chrysostomou}, A. and {Holland}, W.~S. and {Momose}, M.},
    title = "{First Detection of Submillimeter Polarization from T Tauri Stars}",
  journal = {\apj},
 keywords = {STARS: CIRCUMSTELLAR MATTER, ISM: MAGNETIC FIELDS, POLARIZATION, STARS: INDIVIDUAL (GM AURIGAE, DG TAURI), STARS: PRE-MAIN-SEQUENCE, Stars: Circumstellar Matter, ISM: Magnetic Fields, Polarization, stars: individual (GM Aurigae, DG Tauri), Stars: Pre-Main-Sequence},
     year = 1999,
    month = nov,
   volume = 525,
    pages = {832-836},
      doi = {10.1086/307953},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...525..832T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Terebey1984,
   author = {{Terebey}, S. and {Shu}, F.~H. and {Cassen}, P.},
    title = "{The collapse of the cores of slowly rotating isothermal clouds}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Gravitational Collapse, Molecular Clouds, Planetary Evolution, Rotating Matter, Stellar Evolution, Angular Momentum, Differential Equations, Hydrodynamic Equations, Nebulae, Plasma Density, Plasma Equilibrium, Protostars, Stellar Envelopes},
     year = 1984,
    month = nov,
   volume = 286,
    pages = {529-551},
      doi = {10.1086/162628},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...286..529T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Testi2014,
   author = {{Testi}, L. and {Birnstiel}, T. and {Ricci}, L. and {Andrews}, S. and 
	{Blum}, J. and {Carpenter}, J. and {Dominik}, C. and {Isella}, A. and 
	{Natta}, A. and {Williams}, J.~P. and {Wilner}, D.~J.},
    title = "{Dust Evolution in Protoplanetary Disks}",
  journal = {Protostars and Planets VI},
archivePrefix = "arXiv",
   eprint = {1402.1354},
 primaryClass = "astro-ph.SR",
     year = 2014,
    pages = {339-361},
      doi = {10.2458/azu_uapress_9780816531240-ch015},
   adsurl = {http://adsabs.harvard.edu/abs/2014prpl.conf..339T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thamm1994,
   author = {{Thamm}, E. and {Steinacker}, J. and {Henning}, T.},
    title = "{Ambiguities of parametrized dust disk models for young stellar objects}",
  journal = {\aap},,
 keywords = {Accretion Disks, Fitting, Parameterization, Pre-Main Sequence Stars, Stellar Envelopes, Stellar Models, Algorithms, Minima, Radii, Spectral Energy Distribution, Stellar Mass, Stellar Temperature},
     year = 1994,
    month = jul,
   volume = 287,
    pages = {493-502},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...287..493T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Thebault2003,
   author = {{Th{\'e}bault}, P. and {Augereau}, J.~C. and {Beust}, H.},
    title = "{Dust production from collisions in extrasolar planetary systems. The inner beta  Pictoris disc}",
  journal = {\aap},
       year = 2003,
    month = sep,
   volume = 408,
    pages = {775-788},
}

@ARTICLE{Thebault2007,
   author = {{Th{\'e}bault}, P. and {Augereau}, J.-C.},
    title = "{Collisional processes and size distribution in spatially extended debris discs}",
    journal = {\aap},
    year = 2007,
    month = sep,
   volume = 472,
    pages = {169-185},
   }


@ARTICLE{Thebault2012,
   author = {{Thebault}, P. and {Kral}, Q. and {Ertel}, S.},
    title = "{Planet signatures in collisionally active debris discs: scattered light images}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1209.3969},
 primaryClass = "astro-ph.EP",
 keywords = {planet-disk interactions, planets and satellites: formation, circumstellar matter},
     year = 2012,
    month = nov,
   volume = 547,
      eid = {A92},
    pages = {A92},
      doi = {10.1051/0004-6361/201219962},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...547A..92T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}   
   
@ARTICLE{Thompson1998,
   author = {{Thompson}, R.~I. and {Rieke}, M. and {Schneider}, G. and {Hines}, D.~C. and 
	{Corbin}, M.~R.},
    title = "{Initial On-Orbit Performance of NICMOS}",
  journal = {\apj},
 keywords = {INSTRUMENTATION: DETECTORS, MISCELLANEOUS, SPACE VEHICLES, Instrumentation: Detectors, Miscellaneous, Space Vehicles},
     year = 1998,
    month = jan,
   volume = 492,
    pages = {L95-L97},
      doi = {10.1086/311095},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...492L..95T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}   


@ARTICLE{Toomre1964,
   author = {{Toomre}, A.},
    title = "{On the gravitational stability of a disk of stars}",
  journal = {\apj},
     year = 1964,
    month = may,
   volume = 139,
    pages = {1217-1238},
      doi = {10.1086/147861},
   adsurl = {http://adsabs.harvard.edu/abs/1964ApJ...139.1217T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

   
@ARTICLE{Trilling2008,
author = {{Trilling}, D.~E. and {Bryden}, G. and {Beichman}, C.~A. and 
	{Rieke}, G.~H. and {Su}, K.~Y.~L. and {Stansberry}, J.~A. and 
	{Blaylock}, M. and {Stapelfeldt}, K.~R. and {Beeman}, J.~W. and 
	{Haller}, E.~E.},
    title = "{Debris Disks around Sun-like Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.5498},
 keywords = {circumstellar matter, infrared: stars, planetary systems: formation},
     year = 2008,
    month = feb,
   volume = 674,
      eid = {1086-1105},
    pages = {1086-1105},
      doi = {10.1086/525514},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...674.1086T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}  

@book{Unsoeld2004,
  title={Der neue Kosmos: Einf{\"u}hrung in die Astronomie und Astrophysik},
  author={A. Uns{\"o}ld and Bodo Baschek},
  isbn={9783540421771},
  url={http://books.google.de/books?id=11XXkgnJG88C},
  year={2004},
  month = sep,
  volume = 7,
  publisher={Springer}
}
   
@ARTICLE{vanBreemen2011,
   author = {{van Breemen}, J.~M. and {Min}, M. and {Chiar}, J.~E. and {Waters}, L.~B.~F.~M. and 
	{Kemper}, F. and {Boogert}, A.~C.~A. and {Cami}, J. and {Decin}, L. and 
	{Knez}, C. and {Sloan}, G.~C. and {Tielens}, A.~G.~G.~M.},
    title = "{The 9.7 and 18 {$\mu$}m silicate absorption profiles towards diffuse and molecular cloud lines-of-sight}",
  journal = {\aap},
     year = 2011,
    month = feb,
   volume = 526,
    pages = {A152},
}


@ARTICLE{vanDishoeck1998,
   author = {{van Dishoeck}, E.~F. and {Blake}, G.~A.},
    title = "{Chemical Evolution of Star-Forming Regions}",
  journal = {Annual Review of Astronomy \& Astrophysics},
     year = 1998,
   volume = 36,
    pages = {317-368},
      doi = {10.1146/annurev.astro.36.1.317},
   adsurl = {http://adsabs.harvard.edu/abs/1998ARA%26A..36..317V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanDishoeck2004,
   author = {{van Dishoeck}, E.~F.},
    title = "{ISO Spectroscopy of Gas and Dust: From Molecular Clouds to Protoplanetary Disks}",
  journal = {Annual Review of Astronomy \& Astrophysics},
   eprint = {arXiv:astro-ph/0403061},
     year = 2004,
    month = sep,
   volume = 42,
    pages = {119-167},
      doi = {10.1146/annurev.astro.42.053102.134010},
   adsurl = {http://adsabs.harvard.edu/abs/2004ARA%26A..42..119V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanLeeuwen2007,
   author = {{van Leeuwen}, F.},
    title = "{Validation of the new Hipparcos reduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.1752},
 keywords = {space vehicles: instruments, methods: data analysis, catalogs, astrometry, instrumentation: miscellaneous},
     year = 2007,
    month = nov,
   volume = 474,
    pages = {653-664},
      doi = {10.1051/0004-6361:20078357},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...474..653V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanLieshout2014,
   author = {{van Lieshout}, R. and {Dominik}, C. and {Kama}, M. and {Min}, M.
	},
    title = "{Near-infrared emission from sublimating dust in collisionally active debris disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1404.3271},
 primaryClass = "astro-ph.EP",
 keywords = {zodiacal dust, circumstellar matter},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A51},
    pages = {A51},
      doi = {10.1051/0004-6361/201322090},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..51V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Vaidya2011,
   author = {{Vaidya}, D.~B. and {Gupta}, R.},
    title = "{Infrared emission from the composite grains: effects of inclusions and porosities on the 10 and 18 {$\mu$}m features}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.1782},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, circumstellar matter},
     year = 2011,
    month = apr,
   volume = 528,
      eid = {A57},
    pages = {A57},
      doi = {10.1051/0004-6361/201014899},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...528A..57V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valenti2005,
   author = {{Valenti}, J.~A. and {Fischer}, D.~A.},
    title = "{Spectroscopic Properties of Cool Stars (SPOCS). I. 1040 F, G, and K Dwarfs from Keck, Lick, and AAT Planet Search Programs}",
  journal = {\apjs},
 keywords = {Catalogs, Stars: Abundances, Stars: Fundamental Parameters, Stars: Late-Type, Techniques: Spectroscopic},
     year = 2005,
    month = jul,
   volume = 159,
    pages = {141-166},
      doi = {10.1086/430500},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJS..159..141V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanBelle2001,
   author = {{van Belle}, G.~T. and {Ciardi}, D.~R. and {Thompson}, R.~R. and 
	{Akeson}, R.~L. and {Lada}, E.~A.},
    title = "{Altair's Oblateness and Rotation Velocity from Long-Baseline Interferometry}",
  journal = {\apj},
 keywords = {Stars: Fundamental Parameters, stars: individual (Altair), Infrared: Stars, Techniques: Interferometric},
     year = 2001,
    month = oct,
   volume = 559,
    pages = {1155-1164},
      doi = {10.1086/322340},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...559.1155V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanBelle2006,
   author = {{van Belle}, G.~T. and {Ciardi}, D.~R. and {ten Brummelaar}, T. and 
	{McAlister}, H.~A. and {Ridgway}, S.~T. and {Berger}, D.~H. and 
	{Goldfinger}, P.~J. and {Sturmann}, J. and {Sturmann}, L. and 
	{Turner}, N. and {Boden}, A.~F. and {Thompson}, R.~R. and {Coyne}, J.
	},
    title = "{First Results from the CHARA Array. III. Oblateness, Rotational Velocity, and Gravity Darkening of Alderamin}",
  journal = {\apj},
   eprint = {astro-ph/0509827},
 keywords = {Infrared: Stars, Stars: Fundamental Parameters, stars: individual (Alderamin), Techniques: Interferometric},
     year = 2006,
    month = jan,
   volume = 637,
    pages = {494-505},
      doi = {10.1086/498334},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...637..494V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vican2012,
   author = {{Vican}, L.},
    title = "{Age Determination for 346 Nearby Stars in the Herschel DEBRIS Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.1966},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: evolution, stars: rotation},
     year = 2012,
    month = jun,
   volume = 143,
      eid = {135},
    pages = {135},
      doi = {10.1088/0004-6256/143/6/135},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....143..135V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Vitense2010,
   author = {{Vitense}, C. and {Krivov}, A.~V. and {L{\"o}hne}, T.},
    title = "{The Edgeworth-Kuiper debris disk}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1006.2220},
 primaryClass = "astro-ph.EP",
 keywords = {Kuiper belt: general, methods: statistical, methods: numerical, planetary systems, circumstellar matter, infrared: planetary systems},
     year = 2010,
    month = sep,
   volume = 520,
      eid = {A32},
    pages = {A32},
      doi = {10.1051/0004-6361/201014208},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...520A..32V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Vitense2012,
   author = {{Vitense}, C. and {Krivov}, A.~V. and {Kobayashi}, H. and {L{\"o}hne}, T.
	},
    title = "{An improved model of the Edgeworth-Kuiper debris disk}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1202.2257},
 primaryClass = "astro-ph.EP",
 keywords = {methods: numerical, infrared: planetary systems, Kuiper belt: general, planet-disk interactions, interplanetary medium},
     year = 2012,
    month = apr,
   volume = 540,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201118551},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540A..30V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Voges1999,
   author = {{Voges}, W. and {Aschenbach}, B. and {Boller}, T. and {Br{\"a}uninger}, H. and 
	{Briel}, U. and {Burkert}, W. and {Dennerl}, K. and {Englhauser}, J. and 
	{Gruber}, R. and {Haberl}, F. and {Hartner}, G. and {Hasinger}, G. and 
	{K{\"u}rster}, M. and {Pfeffermann}, E. and {Pietsch}, W. and 
	{Predehl}, P. and {Rosso}, C. and {Schmitt}, J.~H.~M.~M. and 
	{Tr{\"u}mper}, J. and {Zimmermann}, H.~U.},
    title = "{The ROSAT all-sky survey bright source catalogue}",
  journal = {\aap},
   eprint = {astro-ph/9909315},
 keywords = {CATALOGS, SURVEYS, X-RAYS: GENERAL},
     year = 1999,
    month = sep,
   volume = 349,
    pages = {389-405},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...349..389V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Voshchinnikov1993,
   author = {{Voshchinnikov}, N.~V. and {Farafonov}, V.~G.},
    title = "{Optical properties of spheroidal particles}",
  journal = {Astrophysics and Space Science},
 keywords = {Optical Properties, Particle Size Distribution, Spheres, Asymptotic Properties, Electromagnetic Radiation, Interstellar Matter, Radiation Pressure, Scattering Cross Sections},
     year = 1993,
    month = jun,
   volume = 204,
    pages = {19-86},
      doi = {10.1007/BF00658095},
   adsurl = {http://adsabs.harvard.edu/abs/1993Ap%26SS.204...19V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Voshchinnikov1999,
   author = {{Voshchinnikov}, N.~V. and {Mathis}, J.~S.},
    title = "{Calculating Cross Sections of Composite Interstellar Grains}",
  journal = {\apj},
     year = 1999,
    month = nov,
   volume = 526,
    pages = {257-264},
}

@Article{Voshchinnikov2005,
   author = {{Voshchinnikov}, N.~V. and {Il'in}, V.~B. and {Henning}, T.},
    title = "{Modelling the optical properties of composite and porous interstellar grains}",
  journal = {\aap},
     year = 2005,
    month = jan,
   volume = 429,
} 

@ARTICLE{Voshchinnikov2006,
   author = {{Voshchinnikov}, N.~V. and {Il'in}, V.~B. and {Henning}, T. and 
	{Dubkova}, D.~N.},
    title = "{Dust extinction and absorption: the challenge of porous grains}",
  journal = {\aap},
   eprint = {astro-ph/0509277},
 keywords = {scattering, ISM: dust, extinction, comets: general, interplanetary medium, stars: individual: {$\zeta$} Oph, {$\sigma$} Sco, Galaxy: center},
     year = 2006,
    month = jan,
   volume = 445,
    pages = {167-177},
      doi = {10.1051/0004-6361:20053371},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..167V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Voshchinnikov2007,
   author = {{Voshchinnikov}, N.~V. and {Videen}, G. and {Henning}, T.},
    title = "{Effective medium theories for irregular fluffy structures: aggregation of small particles}",
  journal = {Applied Optics IP},
   eprint = {astro-ph/0703023},
 keywords = {Scattering, particles},
     year = 2007,
    month = jul,
   volume = 46,
    pages = {4065-4072},
      doi = {10.1364/AO.46.004065},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApOpt..46.4065V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Voshchinnikov2008,
   author = {{Voshchinnikov}, N.~V. and {Henning}, T.},
    title = "{Is the silicate emission feature only influenced by grain size?}",
  journal = {\aap},,
archivePrefix = "arXiv",
   eprint = {0803.3227},
 keywords = {line: profiles, stars: pre-main-sequence, stars: planetary systems: protoplanetary disks, stars: circumstellar matter, infrared: stars, ISM: dust, extinction},
     year = 2008,
    month = may,
   volume = 483,
    pages = {L9-L12},
      doi = {10.1051/0004-6361:200809697},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483L...9V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vrba1985,
   author = {{Vrba}, F.~J. and {Rydgren}, A.~E. and {Zak}, D.~S.},
    title = "{JHKL photometry of three Herbig-Haro jet sources and a nebulous T Tauri star}",
  journal = {Astronomical Journal},
 keywords = {Astronomical Photometry, Herbig-Haro Objects, Infrared Stars, T Tauri Stars, Interstellar Magnetic Fields, Mass Flow, Stellar Winds},
     year = 1985,
    month = oct,
   volume = 90,
    pages = {2074-2076},
      doi = {10.1086/113914},
   adsurl = {http://adsabs.harvard.edu/abs/1985AJ.....90.2074V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wada2007,
   author = {{Wada}, K. and {Tanaka}, H. and {Suyama}, T. and {Kimura}, H. and 
	{Yamamoto}, T.},
    title = "{Numerical Simulation of Dust Aggregate Collisions. I. Compression and Disruption of Two-Dimensional Aggregates}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Methods: n-Body Simulations, Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks},
     year = 2007,
    month = may,
   volume = 661,
    pages = {320-333},
      doi = {10.1086/514332},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...661..320W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wada2008,
   author = {{Wada}, K. and {Tanaka}, H. and {Suyama}, T. and {Kimura}, H. and 
	{Yamamoto}, T.},
    title = "{Numerical Simulation of Dust Aggregate Collisions. II. Compression and Disruption of Three-Dimensional Aggregates in Head-on Collisions}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Methods: n-Body Simulations, Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {1296-1308},
      doi = {10.1086/529511},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677.1296W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wada2009,
   author = {{Wada}, K. and {Tanaka}, H. and {Suyama}, T. and {Kimura}, H. and 
	{Yamamoto}, T.},
    title = "{Collisional Growth Conditions for Dust Aggregates}",
  journal = {\apj},
 keywords = {circumstellar matter, dust, extinction, methods: N-body simulations, planetary systems: formation, planetary systems: protoplanetary disks},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {1490-1501},
      doi = {10.1088/0004-637X/702/2/1490},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702.1490W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wada2011,
   author = {{Wada}, K. and {Tanaka}, H. and {Suyama}, T. and {Kimura}, H. and 
	{Yamamoto}, T.},
    title = "{The Rebound Condition of Dust Aggregates Revealed by Numerical Simulation of Their Collisions}",
  journal = {\apj},
 keywords = {dust, extinction, methods: numerical, planets and satellites: formation, protoplanetary disks},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {36},
    pages = {36},
      doi = {10.1088/0004-637X/737/1/36},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...36W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wada2013,
   author = {{Wada}, K. and {Tanaka}, H. and {Okuzumi}, S. and {Kobayashi}, H. and 
	{Suyama}, T. and {Kimura}, H. and {Yamamoto}, T.},
    title = "{Growth efficiency of dust aggregates through collisions with high mass ratios}",
  journal = {\aap},
 keywords = {planets and satellites: formation, protoplanetary disks, methods: numerical},
     year = 2013,
    month = nov,
   volume = 559,
      eid = {A62},
    pages = {A62},
      doi = {10.1051/0004-6361/201322259},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...559A..62W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walsh2012,
   author = {{Walsh}, J. and {Testi}, L.},
    title = "{First published ALMA Early Science Cycle 0 Result -  Mapping of the Fomalhaut Debris Disc}",
  journal = {The Messenger},
     year = 2012,
    month = jun,
   volume = 148,
    pages = {32-32},
   adsurl = {http://adsabs.harvard.edu/abs/2012Msngr.148...32W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{Warren1994,
   author = {{Warren}, J.~L. and {Barrett}, R.~A. and {Dodson}, A.~L. and {Watts}, A.~L. and {Zolensky}, M.~E.}, 
    title = "{Cosmic Dust Catalog 15}",
booktitle = {Houston: NASA},
     year = 1994,
}

@article{Waterman1965, 
 author={Waterman, P.~C.}, 
title={Matrix formulation of electromagnetic scattering}, 
 journal={Proceedings of the IEEE},
year={1965},
volume={53},
 number={8}, 
pages={805--812}
}

@ARTICLE{Waterman1971,
   author = {{Waterman}, P.~C.},
    title = "{Symmetry, Unitarity, and Geometry in Electromagnetic Scattering}",
  journal = {Physical Review D},
     year = 1971,
    month = feb,
   volume = 3,
    pages = {825-839},
      doi = {10.1103/PhysRevD.3.825},
   adsurl = {http://adsabs.harvard.edu/abs/1971PhRvD...3..825W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Watson2007,
   author = {{Watson}, A.~M. and {Stapelfeldt}, K.~R. and {Wood}, K. and 
	{M{\'e}nard}, F.},
    title = "{Multiwavelength Imaging of Young Stellar Object Disks: Toward an Understanding of Disk Structure and Dust Evolution}",
  journal = {Protostars and Planets V},
archivePrefix = "arXiv",
   eprint = {0707.2608},
     year = 2007,
    pages = {523-538},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..523W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Weidenschilling1993,
   author = {{Weidenschilling}, S.~J. and {Cuzzi}, J.~N.},
    title = "{Formation of planetesimals in the solar nebula}",
 keywords = {ACCRETION DISKS, FLUID DYNAMICS, PARTICLE MOTION, PLANETARY EVOLUTION, SOLAR CORONA, ASTRONOMICAL MODELS, GAS DYNAMICS, MAGNETOHYDRODYNAMIC TURBULENCE, STELLAR MASS},
booktitle = {Protostars and Planets III},
     year = 1993,
   editor = {{Levy}, E.~H. and {Lunine}, J.~I.},
    pages = {1031-1060},
   adsurl = {http://adsabs.harvard.edu/abs/1993prpl.conf.1031W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 
@BOOK{WeigertBook,
   author = {{Weigert}, A. and {Wendker}, H.~J. and {Wisotzki}, L.},
    title = "{Astronomie und Astrophysik: Ein Grundkurs.}",
booktitle = { 5. überarbeitete und erweiterte Auflage. Wiley VCH, Weinheim.},
  year = 2009,
}

@ARTICLE{Weinberger2015,
   author = {{Weinberger}, A.~J. and {Bryden}, G. and {Kennedy}, G.~M. and 
	{Roberge}, A. and {Defr{\`e}re}, D. and {Hinz}, P.~M. and {Millan-Gabet}, R. and 
	{Rieke}, G. and {Bailey}, V.~P. and {Danchi}, W.~C. and {Haniff}, C. and 
	{Mennesson}, B. and {Serabyn}, E. and {Skemer}, A.~J. and {Stapelfeldt}, K.~R. and 
	{Wyatt}, M.~C.},
    title = "{Target Selection for the LBTI Exozodi Key Science Program}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1501.01319},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, surveys, techniques: interferometric },
     year = 2015,
    month = feb,
   volume = 216,
      eid = {24},
    pages = {24},
      doi = {10.1088/0067-0049/216/2/24},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..216...24W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 

@ARTICLE{WeingartnerDraine2001,
author = {{Weingartner}, J.~C. and {Draine}, B.~T.},
    title = "{Dust Grain-Size Distributions and Extinction in the Milky Way, Large Magellanic Cloud, and Small Magellanic Cloud}",
  journal = {\apj},
   eprint = {astro-ph/0008146},
 keywords = {ISM: Dust, Extinction, ISM: Clouds},
     year = 2001,
    month = feb,
   volume = 548,
    pages = {296-309},
      doi = {10.1086/318651},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...548..296W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Westphal2014,
   author = {{Westphal}, A.~J. and {Stroud}, R.~M. and {Bechtel}, H.~A. and 
	{Brenker}, F.~E. and {Butterworth}, A.~L. and {Flynn}, G.~J. and 
	{Frank}, D.~R. and {Gainsforth}, Z. and {Hillier}, J.~K. and 
	{Postberg}, F. and {Simionovici}, A.~S. and {Sterken}, V.~J. and 
	{Nittler}, L.~R. and {Allen}, C. and {Anderson}, D. and {Ansari}, A. and 
	{Bajt}, S. and {Bastien}, R.~K. and {Bassim}, N. and {Bridges}, J. and 
	{Brownlee}, D.~E. and {Burchell}, M. and {Burghammer}, M. and 
	{Changela}, H. and {Cloetens}, P. and {Davis}, A.~M. and {Doll}, R. and 
	{Floss}, C. and {Gr{\"u}n}, E. and {Heck}, P.~R. and {Hoppe}, P. and 
	{Hudson}, B. and {Huth}, J. and {Kearsley}, A. and {King}, A.~J. and 
	{Lai}, B. and {Leitner}, J. and {Lemelle}, L. and {Leonard}, A. and 
	{Leroux}, H. and {Lettieri}, R. and {Marchant}, W. and {Ogliore}, R. and 
	{Ong}, W.~J. and {Price}, M.~C. and {Sandford}, S.~A. and {Tresseras}, J.-A.~S. and 
	{Schmitz}, S. and {Schoonjans}, T. and {Schreiber}, K. and {Silversmit}, G. and 
	{Sol{\'e}}, V.~A. and {Srama}, R. and {Stadermann}, F. and {Stephan}, T. and 
	{Stodolna}, J. and {Sutton}, S. and {Trieloff}, M. and {Tsou}, P. and 
	{Tyliszczak}, T. and {Vekemans}, B. and {Vincze}, L. and {Von Korff}, J. and 
	{Wordsworth}, N. and {Zevin}, D. and {Zolensky}, M.~E. and {aff14}
	},
    title = "{Evidence for interstellar origin of seven dust particles collected by the Stardust spacecraft}",
  journal = {Science},
     year = 2014,
    month = aug,
   volume = 345,
    pages = {786-791},
      doi = {10.1126/science.1252496},
   adsurl = {http://adsabs.harvard.edu/abs/2014Sci...345..786W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Whitney1992,
   author = {{Whitney}, B.~A. and {Hartmann}, L.},
    title = "{Model scattering envelopes of young stellar objects. I - Method and application to circumstellar disks}",
  journal = {\apj},
 keywords = {MONTE CARLO METHOD, PRE-MAIN SEQUENCE STARS, RADIATIVE TRANSFER, STAR FORMATION, T TAURI STARS, LIGHT SCATTERING, OPTICAL THICKNESS, POINT SOURCES, STELLAR ENVELOPES, STELLAR OCCULTATION},
     year = 1992,
    month = aug,
   volume = 395,
    pages = {529-539},
      doi = {10.1086/171673},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...395..529W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Whitney1993,
   author = {{Whitney}, B.~A. and {Hartmann}, L.},
    title = "{Model scattering envelopes of young stellar objects. II - Infalling envelopes}",
  journal = {\apj},
 keywords = {EARLY STARS, STELLAR ENVELOPES, STELLAR MODELS, ASTRONOMICAL MODELS, DENSITY DISTRIBUTION, INTERSTELLAR MATTER, LIGHT SCATTERING, STELLAR EVOLUTION, STELLAR WINDS},
     year = 1993,
    month = jan,
   volume = 402,
    pages = {605-622},
      doi = {10.1086/172163},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...402..605W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{White2004,
   author = {{White}, R.~J. and {Hillenbrand}, L.~A.},
    title = "{On the Evolutionary Status of Class I Stars and Herbig-Haro Energy Sources in Taurus-Auriga}",
  journal = {\apj},
   eprint = {astro-ph/0408244},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Formation, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs, Stars: Winds, Outflows},
     year = 2004,
    month = dec,
   volume = 616,
    pages = {998-1032},
      doi = {10.1086/425115},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616..998W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Whitney2004,
   author = {{Whitney}, B.~A. and {Indebetouw}, R. and {Bjorkman}, J.~E. and 
	{Wood}, K.},
    title = "{Two-Dimensional Radiative Transfer in Protostellar Envelopes. III. Effects of Stellar Temperature}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Radiative Transfer, Stars: Formation, Stars: Pre-Main-Sequence},
     year = 2004,
    month = dec,
   volume = 617,
    pages = {1177-1190},
      doi = {10.1086/425608},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...617.1177W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wichmann1998,
   author = {{Wichmann}, R. and {Bastian}, U. and {Krautter}, J. and {Jankovics}, I. and 
	{Rucinski}, S.~M.},
    title = "{HIPPARCOS observations of pre-main-sequence stars}",
  journal = {\mnras},
 keywords = {STARS: FORMATION, STARS: LATE-TYPE, STARS: PRE-MAIN-SEQUENCE},
     year = 1998,
    month = dec,
   volume = 301,
    pages = {L39},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301L..39W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wien1896,
   author = {{Wien}, W.},
    title = "{Ueber die Energievertheilung im Emissionsspectrum eines schwarzen K{\"o}rpers}",
  journal = {Annalen der Physik},
     year = 1896,
   volume = 294,
    pages = {662-669},
      doi = {10.1002/andp.18962940803},
   adsurl = {http://adsabs.harvard.edu/abs/1896AnP...294..662W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wild2006,
   author = {{Sandford}, S.~A. and {Al{\'e}on}, J. and {Alexander}, C.~M.~O.~'. and 
	{Araki}, T. and {Bajt}, S. and {Baratta}, G.~A. and {Borg}, J. and 
	{Bradley}, J.~P. and {Brownlee}, D.~E. and {Brucato}, J.~R. and 
	{Burchell}, M.~J. and {Busemann}, H. and {Butterworth}, A. and 
	{Clemett}, S.~J. and {Cody}, G. and {Colangeli}, L. and {Cooper}, G. and 
	{D'Hendecourt}, L. and {Djouadi}, Z. and {Dworkin}, J.~P. and 
	{Ferrini}, G. and {Fleckenstein}, H. and {Flynn}, G.~J. and 
	{Franchi}, I.~A. and {Fries}, M. and {Gilles}, M.~K. and {Glavin}, D.~P. and 
	{Gounelle}, M. and {Grossemy}, F. and {Jacobsen}, C. and {Keller}, L.~P. and 
	{Kilcoyne}, A.~L.~D. and {Leitner}, J. and {Matrajt}, G. and 
	{Meibom}, A. and {Mennella}, V. and {Mostefaoui}, S. and {Nittler}, L.~R. and 
	{Palumbo}, M.~E. and {Papanastassiou}, D.~A. and {Robert}, F. and 
	{Rotundi}, A. and {Snead}, C.~J. and {Spencer}, M.~K. and {Stadermann}, F.~J. and 
	{Steele}, A. and {Stephan}, T. and {Tsou}, P. and {Tyliszczak}, T. and 
	{Westphal}, A.~J. and {Wirick}, S. and {Wopenka}, B. and {Yabuta}, H. and 
	{Zare}, R.~N. and {Zolensky}, M.~E.},
    title = "{Organics Captured from Comet 81P/Wild 2 by the Stardust Spacecraft}",
  journal = {Science},
     year = 2006,
    month = dec,
   volume = 314,
    pages = {1720}
}

@ARTICLE{Williams2004,
   author = {{Williams}, J.~P. and {Najita}, J. and {Liu}, M.~C. and {Bottinelli}, S. and 
	{Carpenter}, J.~M. and {Hillenbrand}, L.~A. and {Meyer}, M.~R. and 
	{Soderblom}, D.~R.},
    title = "{Detection of Cool Dust around the G2 V Star HD 107146}",
  journal = {\apj},
     year = 2004,
    month = mar,
   volume = 604,
    pages = {414-419},
}

@ARTICLE{Wilson2008,
   author = {{Wilson}, G.~W. and {Austermann}, J.~E. and {Perera}, T.~A. and 
	{Scott}, K.~S. and {Ade}, P.~A.~R. and {Bock}, J.~J. and {Glenn}, J. and 
	{Golwala}, S.~R. and {Kim}, S. and {Kang}, Y. and {Lydon}, D. and 
	{Mauskopf}, P.~D. and {Predmore}, C.~R. and {Roberts}, C.~M. and 
	{Souccar}, K. and {Yun}, M.~S.},
    title = "{The AzTEC mm-wavelength camera}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0801.2783},
 keywords = {instrumentation: detectors , galaxies: high redshift , galaxies: starburst , submillimetre},
     year = 2008,
    month = may,
   volume = 386,
    pages = {807-818},
      doi = {10.1111/j.1365-2966.2008.12980.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..807W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Windhorst2006,
   author = {{Windhorst}, R.~A. and {Cohen}, S.~H. and {Jansen}, R.~A. and 
	{Conselice}, C. and {Yan}, H.},
    title = "{How JWST can measure first light, reionization and galaxy assembly}",
  journal = {New Astronomy Reviews},
   eprint = {astro-ph/0506253},
     year = 2006,
    month = mar,
   volume = 50,
    pages = {113-120},
      doi = {10.1016/j.newar.2005.11.018},
   adsurl = {http://adsabs.harvard.edu/abs/2006NewAR..50..113W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Witten1986,
   author = {{Witten}, T.~A. and {Cates}, M.~E.},
    title = "{Tenuous Structures from Disorderly Growth Processes}",
  journal = {Science},
     year = 1986,
    month = jun,
   volume = 232,
    pages = {1607-1612},
}

@ARTICLE{Woitas2002,
   author = {{Woitas}, J. and {Eisl{\"o}ffel}, J. and {Mundt}, R. and {Ray}, T.~P.
	},
    title = "{The Environment of FS Tauri Observed with Hubble Space Telescope Wide Field Planetary Camera 2 in Narrowband Emission Line Filters}",
  journal = {\apj},
 keywords = {ISM: Jets and Outflows, stars: individual (FS Tauri)},
     year = 2002,
    month = jan,
   volume = 564,
    pages = {834-838},
      doi = {10.1086/324274},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..834W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wolf1999,
   author = {{Wolf}, S. and {Henning}, T. and {Stecklum}, B.},
    title = "{Multidimensional self-consistent radiative transfer simulations based on the Monte-Carlo method}",
  journal = {\aap},
 keywords = {POLARIZATION, RADIATIVE TRANSFER, SCATTERING, STARS: CIRCUMSTELLAR MATTER, ISM: CLOUDS, ISM: DUST, EXTINCTION},
     year = 1999,
    month = sep,
   volume = 349,
    pages = {839-850},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...349..839W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wolf2002,
   author = {{Wolf}, S. and {Voshchinnikov}, N.~V. and {Henning}, T.},
    title = "{Multiple scattering of polarized radiation by non-spherical grains: First results}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0201549},
 keywords = {POLARIZATION, RADIATIVE TRANSFER, SCATTERING, METHODS: NUMERICAL, (STARS:) CIRCUMSTELLAR MATTER, ISM: CLOUDS},
     year = 2002,
    month = apr,
   volume = 385,
    pages = {365-376},
      doi = {10.1051/0004-6361:20020158},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...385..365W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wolf2003,
   author = {{Wolf}, S.},
    title = "{MC3D-3D continuum radiative transfer, Version 2}",
  journal = {Computer Physics Communications},
   eprint = {arXiv:astro-ph/0207374},
     year = 2003,
    month = feb,
   volume = 150,
    pages = {99-115},
      doi = {10.1016/S0010-4655(02)00675-6},
   adsurl = {http://adsabs.harvard.edu/abs/2003CoPhC.150...99W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wolf2005,
   author = {{Wolf}, S. and {Hillenbrand}, L.~A.},
    title = "{Debris disk radiative transfer simulation tool (DDS)}",
  journal = {Computer Physics Communications},
     year = 2005,
    month = oct,
   volume = 171,
    pages = {208-218}
}

@ARTICLE{Wolf2012,
   author = {{Wolf}, S. and {Malbet}, F. and {Alexander}, R. and {Berger}, J.-P. and 
	{Creech-Eakman}, M. and {Duch{\^e}ne}, G. and {Dutrey}, A. and 
	{Mordasini}, C. and {Pantin}, E. and {Pont}, F. and {Pott}, J.-U. and 
	{Tatulli}, E. and {Testi}, L.},
    title = "{Circumstellar disks and planets. Science cases for next-generation optical/infrared long-baseline interferometers}",
  journal = {The Astronomy \& Astrophysics Review},
archivePrefix = "arXiv",
   eprint = {1203.6271},
 primaryClass = "astro-ph.IM",
 keywords = {Interferometric instruments, Protoplanetary disks, Planet formation, Debris disks, Extrasolar planets},
     year = 2012,
    month = mar,
   volume = 20,
      eid = {52},
    pages = {52},
      doi = {10.1007/s00159-012-0052-1},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26ARv..20...52W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wolf2003b,
   author = {{Wolf}, S.},
    title = "{Efficient Radiative Transfer in Dust Grain Mixtures}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0209281},
 keywords = {Stars: Circumstellar Matter, Methods: Numerical, Radiative Transfer, Scattering},
     year = 2003,
    month = jan,
   volume = 582,
    pages = {859-868},
      doi = {10.1086/344710},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...582..859W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wolf2003Butterfly,
   author = {{Wolf}, S. and {Padgett}, D.~L. and {Stapelfeldt}, K.~R.},
    title = "{The Circumstellar Disk of the Butterfly Star in Taurus}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0301335},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Radiative Transfer, Scattering, Stars: Individual: Alphanumeric: IRAS 04302+2247, Stars: Pre-Main-Sequence},
     year = 2003,
    month = may,
   volume = 588,
    pages = {373-386},
      doi = {10.1086/374041},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588..373W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WolfHillenbrand2003,
   author = {{Wolf}, S. and {Hillenbrand}, L.~A.},
    title = "{Model Spectral Energy Distributions of Circumstellar Debris Disks. I. Analytic Disk Density Distributions}",
  journal = {\apj},
     year = 2003,
    month = oct,
   volume = 596,
    pages = {603-620},
}

@ARTICLE{WolfVoshchinnikov04,
   author = {{Wolf}, S. and {Voshchinnikov}, N.~V.},
    title = "{Mie scattering by ensembles of particles with very large size parameters}",
  journal = {Computer Physics Communications},
   eprint = {astro-ph/0406118},
 keywords = {Mie scattering, Scattering matrix, Efficiency factors, Cross-sections, optics, geophysics, biophysics},
     year = 2004,
    month = sep,
   volume = 162,
    pages = {113-123},
      doi = {10.1016/j.cpc.2004.06.070},
   adsurl = {http://adsabs.harvard.edu/abs/2004CoPhC.162..113W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wolff1994,
   author = {{Wolff}, M.~J. and {Clayton}, G.~C. and {Martin}, P.~G. and 
	{Schulte-Ladbeck}, R.~E.},
    title = "{Modeling composite and fluffy grains: The effects of porosity}",
  journal = {\apj},
     year = 1994,
    month = mar,
   volume = 423,
    pages = {412-425},
}


@ARTICLE{Wood1998,
   author = {{Wood}, K. and {Kenyon}, S.~J. and {Whitney}, B. and {Turnbull}, M.
	},
    title = "{Optical and Near-Infrared Model Images of the Circumstellar Environments of Classical T Tauri Stars}",
  journal = {\apj},,
 keywords = {STARS: CIRCUMSTELLAR MATTER, RADIATIVE TRANSFER, STARS: INDIVIDUAL ALPHANUMERIC: HH 30, STARS: PRE-MAIN-SEQUENCE},
     year = 1998,
    month = apr,
   volume = 497,
    pages = {404},
      doi = {10.1086/305449},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...497..404W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wood2002,
   author = {{Wood}, K. and {Wolff}, M.~J. and {Bjorkman}, J.~E. and {Whitney}, B.
	},
    title = "{The Spectral Energy Distribution of HH 30 IRS: Constraining the Circumstellar Dust Size Distribution}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0109048},
 keywords = {Accretion, Accretion Disks, ISM: Dust, Extinction, Radiative Transfer, Scattering, Stars: Individual: Alphanumeric: HH 30 IRS, Stars: Pre-Main-Sequence},
     year = 2002,
    month = jan,
   volume = 564,
    pages = {887-895},
      doi = {10.1086/324285},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...564..887W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woolf1969,
   author = {{Woolf}, N.~J. and {Ney}, E.~P.},
    title = "{Circumstellar Infrared Emission from Cool Stars}",
  journal = {\apjl},
     year = 1969,
    month = mar,
   volume = 155,
    pages = {L181},
      doi = {10.1086/180331},
   adsurl = {http://adsabs.harvard.edu/abs/1969ApJ...155L.181W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wright2010,
   author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and 
	{Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and 
	{Stanford}, S.~A. and {Cohen}, M. and {Walker}, R.~G. and {Mather}, J.~C. and 
	{Leisawitz}, D. and {Gautier}, III, T.~N. and {McLean}, I. and 
	{Benford}, D. and {Lonsdale}, C.~J. and {Blain}, A. and {Mendez}, B. and 
	{Irace}, W.~R. and {Duval}, V. and {Liu}, F. and {Royer}, D. and 
	{Heinrichsen}, I. and {Howard}, J. and {Shannon}, M. and {Kendall}, M. and 
	{Walsh}, A.~L. and {Larsen}, M. and {Cardon}, J.~G. and {Schick}, S. and 
	{Schwalm}, M. and {Abid}, M. and {Fabinsky}, B. and {Naes}, L. and 
	{Tsai}, C.-W.},
    title = "{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}",
  journal = {The Astronomical Journal},
archivePrefix = "arXiv",
   eprint = {1008.0031},
 primaryClass = "astro-ph.IM",
 keywords = {infrared: general, space vehicles, surveys},
     year = 2010,
    month = dec,
   volume = 140,
      eid = {1868},
    pages = {1868-1881},
      doi = {10.1088/0004-6256/140/6/1868},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WuWang1991,
   author = {{Wu}, Z.~S. and {Wang}, Y.~P.},
    title = "{Electromagnetic scattering for multilayered sphere: Recursive algorithms}",
  journal = {Radio Science},
     year = 1991,
    month = dec,
   volume = 26,
    pages = {1393-1401},
}

@ARTICLE{Wyatt2002,
   author = {{Wyatt}, M.~C. and {Dent}, W.~R.~F.},
    title = "{Collisional processes in extrasolar planetesimal discs - dust clumps in Fomalhaut's debris disc}",
  journal = {\mnras},
     year = 2002,
    month = aug,
   volume = 334,
    pages = {589-607},
}

@ARTICLE{Wyatt2007a,
   author = {{Wyatt}, M.~C. and {Smith}, R. and {Greaves}, J.~S. and {Beichman}, C.~A. and 
	{Bryden}, G. and {Lisse}, C.~M.},
    title = "{Transience of Hot Dust around Sun-like Stars}",
  journal = {\apj},
   eprint = {astro-ph/0610102},
 keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems: Formation},
     year = 2007,
    month = mar,
   volume = 658,
    pages = {569-583},
      doi = {10.1086/510999},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..569W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wyatt2007,
 author = {{Wyatt}, M.~C. and {Smith}, R. and {Su}, K.~Y.~L. and {Rieke}, G.~H. and 
	{Greaves}, J.~S. and {Beichman}, C.~A. and {Bryden}, G.},
    title = "{Steady State Evolution of Debris Disks around A Stars}",
  journal = {\apj},
   eprint = {astro-ph/0703608},
 keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems: Formation},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {365-382},
      doi = {10.1086/518404},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..365W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Wyatt2008,
   author = {{Wyatt}, M.~C.},
    title = "{Evolution of Debris Disks}",
  journal = {\araa},
     year = 2008,
    month = sep,
   volume = 46,
    pages = {339-383},
      doi = {10.1146/annurev.astro.45.051806.110525},
   adsurl = {http://adsabs.harvard.edu/abs/2008ARA%26A..46..339W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wyatt2012,
   author = {{Wyatt}, M.~C. and {Kennedy}, G. and {Sibthorpe}, B. and {Moro-Mart{\'{\i}}n}, A. and 
	{Lestrade}, J.-F. and {Ivison}, R.~J. and {Matthews}, B. and 
	{Udry}, S. and {Greaves}, J.~S. and {Kalas}, P. and {Lawler}, S. and 
	{Su}, K.~Y.~L. and {Rieke}, G.~H. and {Booth}, M. and {Bryden}, G. and 
	{Horner}, J. and {Kavelaars}, J.~J. and {Wilner}, D.},
    title = "{Herschel imaging of 61 Vir: implications for the prevalence of debris in low-mass planetary systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.2370},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, planet-disc interactions, circumstellar matter, planetary systems},
     year = 2012,
    month = aug,
   volume = 424,
    pages = {1206-1223},
      doi = {10.1111/j.1365-2966.2012.21298.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424.1206W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yokogawa2001,
   author = {{Yokogawa}, S. and {Kitamura}, Y. and {Momose}, M. and {Asaki}, Y. and 
	{Tamura}, M. and {Ida}, S. and {Kawabe}, R.},
    title = "{Millimeter Continuum Image of the Circumstellar Disk around the Young Star Haro 6-5B}",
  journal = {\apjl},
 keywords = {Stars: Circumstellar Matter, Stars: Individual: Name: Haro 6-5B, Stars: Pre-Main-Sequence},
     year = 2001,
    month = may,
   volume = 552,
    pages = {L59-L62},
      doi = {10.1086/320256},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...552L..59Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Yokogawa2002,
   author = {{Yokogawa}, S. and {Kitamura}, Y. and {Momose}, M. and {Kawabe}, R.
	},
    title = "{Deep $^{13}$CO(J=1--0) Imaging of the Protostar Haro 6-5B: Discovery of Rotational Motion in the Protostellar Disk}",
booktitle = {8th Asian-Pacific Regional Meeting, Volume II},
     year = 2002,
   editor = {{Ikeuchi}, S. and {Hearnshaw}, J. and {Hanawa}, T.},
    pages = {239-240},
   adsurl = {http://adsabs.harvard.edu/abs/2002aprm.conf..239Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yurkin2007,
   author = {{Yurkin}, M.~A. and {Maltsev}, V.~P. and {Hoekstra}, A.~G.},
    title = "{The discrete dipole approximation for simulation of light scattering by particles much larger than the wavelength}",
  journal = {Journal of Quantitative Spectroscopy {\&} Radiative Transfer},
     year = 2007,
    month = jul,
   volume = 106,
    pages = {546-557}
}

@ARTICLE{Yurkin2010,
   author = {{Yurkin}, M.~A. and {Min}, M. and {Hoekstra}, A.~G.},
    title = "{Application of the discrete dipole approximation to very large refractive indices: Filtered coupled dipoles revived}",
  journal = {Physical Review E},
     year = 2010,
    month = sep,
   volume = 82,
   number = 3,
    pages = {036703},
}

@ARTICLE{Zeidler2011,
   author = {{Zeidler}, S. and {Posch}, T. and {Mutschke}, H. and {Richter}, H. and 
	{Wehrhan}, O.},
    title = "{Near-infrared absorption properties of oxygen-rich stardust analogs. The influence of coloring metal ions}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.0695},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, infrared: stars, methods: laboratory},
     year = 2011,
    month = feb,
   volume = 526,
      eid = {A68},
    pages = {A68},
      doi = {10.1051/0004-6361/201015219},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A..68Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zeidler2015,
   author = {{Zeidler}, S. and {Mutschke}, H. and {Posch}, T.},
    title = "{Temperature-dependent Infrared Optical Constants of Olivine and Enstatite}",
  journal = {\apj},
 keywords = {circumstellar matter, infrared: stars, methods: laboratory: solid state, stars: AGB and post-AGB, stars: individual: IRAS 09425-6040 },
     year = 2015,
    month = jan,
   volume = 798,
      eid = {125},
    pages = {125},
      doi = {10.1088/0004-637X/798/2/125},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798..125Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhukovska2008,
   author = {{Zhukovska}, S. and {Gail}, H.-P. and {Trieloff}, M.},
    title = "{Evolution of interstellar dust and stardust in the solar neighbourhood}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0706.1155},
 keywords = {ISM: abundances, ISM: dust, extinction, galaxies: ISM, Galaxy: evolution},
     year = 2008,
    month = feb,
   volume = 479,
    pages = {453-480},
      doi = {10.1051/0004-6361:20077789},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...479..453Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zook75,
   author = {{Zook}, H.~A.},
    title = "{Hyperbolic cosmic dust - Its origin and its astrophysical significance}",
  journal = {Planetary Space Science},
     year = 1975,
    month = oct,
   volume = 23,
    pages = {1391-1397},
}

@ARTICLE{Zorec2012,
   author = {{Zorec}, J. and {Royer}, F.},
    title = "{Rotational velocities of A-type stars. IV. Evolution of rotational velocities}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1201.2052},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: rotation, stars: evolution},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A120},
    pages = {A120},
      doi = {10.1051/0004-6361/201117691},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.120Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zsom2011,
   author = {{Zsom}, A. and {Ormel}, C.~W. and {Dullemond}, C.~P. and {Henning}, T.
	},
    title = "{The outcome of protoplanetary dust growth: pebbles, boulders, or planetesimals?. III. Sedimentation driven coagulation inside the snowline}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.5198},
 primaryClass = "astro-ph.EP",
 keywords = {methods: numerical, planets and satellites: formation, protoplanetary disks},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A73},
    pages = {A73},
      doi = {10.1051/0004-6361/201116515},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A..73Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

#######################################
#######################################

@Misc{CDDCHillenbrand,
       author={Hillenbrand, L.},
     year = 2005,
	title = "Circumstellar Dust Disk Calculator (CDDC)",
       url= {http://www.astro.caltech.edu/~lah/feps/widget/dustcalc.html}
}

@Misc{DDSWolf,
   author = {{Wolf}, S. and {Hillenbrand}, L.~A.},
	title = "Debris Disk Radiative Transfer Simulator  (DDS)",
       url= {http://www1.astrophysik.uni-kiel.de/dds/}
}


@Misc{ESO_picture,
	author = {ESO, IAU},
title="{Sky \& Telescope}"
,
year={2011}
}

@Misc{Nasa_picture,
	author = {NASA JPL-Caltech, Pyle,~T.},
year={2009}
}

@Misc{Komposit_picture,
	author = {NASA JPL-Caltech, Pyle,~T.},
year={2009}
}


@Misc{ALMA_picture,
	author = {ALMA-Pressemitteilung vom 6. Nov. 2014,~(NRAO/ESO/NAOJ); Brogan,~{C.,}},
	year={, Saxton,~B. (NRAO/AUI/ NSF)}
}


@Misc{DUNES-Archiv,
	author = {DUNES-Archiv},
title="{http://www.mpia.de/DUNES/}",
year={2014}
}

http://www.mpia.de/DUNES/

@Misc{nasa,
	author = {NASA /FUSE / Lynette Cook},
title="{In the Beta Pictoris Disk}",
year={2006}
}


@Misc{NACO_User_Manual,
   author = {{NACO User Manual}},
	title = "VERY LARGE TELESCOPE NACO User Manual",
	year={2012},
       volume = {90.2},
       url= {http://www.eso.org/sci/facilities/paranal/instruments/naco/doc/VLT-MAN-ESO-14200-2761_v90.pdf}
}

@Misc{NICMOS_HandbookV1,
   author = {{NACO Handbuch}},
	title = "NICMOS Handbook Version 1.0",
	year={1996},
       month = jun,	
       volume = {1.0},
       url= {http://documents.stsci.edu/hst/nicmos/documents/handbooks/v1/ihbv10.html}
}

@Misc{VIZIER,
   author = {VizieR},
	title = "VizieR photometry viewer",
	year={ },	
       url= {http://vizier.u-strasbg.fr/vizier/sed/}
}

